Symphony in the Latent Space: Provably Integrating High-dimensional Techniques with Non-linear Machine Learning Models

This paper revisits building machine learning algorithms that involve interactions between entities, such as those between financial assets in an actively managed portfolio, or interactions between users in a social network. Our goal is to forecast the future evolution of ensembles of multivariate time series in such applications (e.g., the future return of a financial asset or the future popularity of a Twitter account). Designing ML algorithms for such systems requires addressing the challenges of high-dimensional interactions and non-linearity. Existing approaches usually adopt an ad-hoc approach to integrating high-dimensional techniques into non-linear models and recent studies have shown these approaches have questionable efficacy in time-evolving interacting systems. To this end, we propose a novel framework, which we dub as the additive influence model. Under our modeling assumption, we show that it is possible to decouple the learning of high-dimensional interactions from the learning of non-linear feature interactions. To learn the high-dimensional interactions, we leverage kernel-based techniques, with provable guarantees, to embed the entities in a low-dimensional latent space. To learn the non-linear feature-response interactions, we generalize prominent machine learning techniques, including designing a new statistically sound non-parametric method and an ensemble learning algorithm optimized for vector regressions. Extensive experiments on two common applications demonstrate that our new algorithms deliver significantly stronger forecasting power compared to standard and recently proposed methods.

==> a_exp.tex <==



==> a_move.tex <==

\iffalse
\myparab{Remarks.} \emph{(i) Performance comparison.} Fig.~\ref{fig:compare} shows the tradeoffs of multiple algorithms we studied under the decoupling principle. The algorithms ending with ``NN'' denote our proposed methods, which learn neighbors from latent positions. 
\emph{(ii) Optimized latent positions.} The estimation of $\hat K$ is closely related to the estimation of the covariance matrix of returns. 
In App.~\ref{sec:latentpos}, we % should 
discuss using risk models and news to enhance the latent position estimator. 


however, they do not have theoretical guarantees.

{\color{red} maybe move the nsf text to explain why we ues only technical factors.}


Existing ML models can be roughly categorized into univariate models and vector regression models. In a  univariate model, one produces a real-valued forecast $\hat \my_{t + 1, i} = f(\mx_{t, i})$ for the return of stock $i$ at round $t$. The features $\mx_{t, i}$ are constructed from information that is directly associated with stock $i$ \cite{wuthrich1998daily,gu2018empirical,chen2019investment,kelly2019characteristics}. In the vector regression model, we aim to learn $\my_{t + 1} = f(\mx_t)$, where $\my_{t+1}$ is a vector that represents the returns of all stocks, and $\mx_t$ consists of information related to all stocks up to (and including) round $t$.  
% (\MC{but below we say we use info ''available at the end of round t-1"}). 
Vector regression models are capable of capturing interactions between stocks, e.g., Apple's price change in the last round impacts the return of many of its upstream providers, and potential competitors. An example of a vector regression model is VAR, i.e., $\my_{t+1} = A \my_{t} + \xi_{t+1}$, where $A$ is a square matrix ~\cite{friedman2001elements,cawley2002reduced,bunea2011optimal,koltchinskii2011nuclear,huang2019shrinking,wu2019adaptive}. %This also closely relates to multi-task learning, where parameter sharing becomes a form of regularization~\cite{Ghosn1997}. 

% \MC{there is also an intermediate setting when you regress cross-sectionally $y_{t,:} = A \beta + \epsilon $, where $A$ is the feature matrix of size $d \times f$ (with f denoting the number of features). It is still cross-sectional, but still, each stock only depends on its own features, and not on features of other instruments.. We should also clarify this, and say it's now what we are after.. Or we could fit it under univariate, but say that the coefficient sharing is a form of regularization.}

In practice, univariate  models are robust against overfitting, even when the feature set size is moderately large (e.g., a few hundreds) and thus deep learning and boosted regression trees have been extensively used~\cite{han2018firm,gu2018empirical,de2018advances,feng2018deep,chen2019deep,gu2019autoencoder,chen2019investment,ding2015deep,zhang2017stock,hu2018listening,feng2019temporal,ke2019deepgbm,li2019individualized}. Note that univariate models can be trained using the coefficient sharing trick (i.e., multiple symbols share the same model)~\cite{Ghosn1997}. Here, $f(\cdot)$ uses cross-asset information, but $\mx$ does not, thus these models do not directly use linkage information (and thus do not address the task we are after). 
On the other hand, circumventing the overfitting problem for high-dimensional data stemmed from using cross-asset signals has been remarkably difficult even for linear models because one needs to carefully design and tune regularizers~\cite{bunea2011optimal,cawley2002reduced,koltchinskii2011nuclear,negahban2011estimation,wu2019adaptive,huang2019shrinking}. Limited non-linear models have been developed. Chen et al.~\cite{chen2019investment} used public funds' portfolio information to construct a latent embedding, but it does not yet use features $\mx_{t,i}$ from linked stocks. Works~\cite{wang2019alphastock,feng2019temporal} used deep learning to both estimate stocks' latent space and use features from nearby stocks in forecasting; however, they do not have theoretical guarantees. 


\subsection{Forecasting performance}
\vspace{-1mm}
Table~\ref{main_table} shows the performance of all the algorithms. Fig.~\ref{fig:fret_quantiles} shows the cumulative PnL (Profit \& Loss) under three simulations, including  ``Long-index portfolio'', ``Long-short portfolio'', and ``Weighted-Long-short portfolio.'' See  App.~\ref{performance}. Note that shorting can be done in Chinese market under very restricted conditions (e.g., entering a customized deal with a broker in Hong Kong). 
%  
We make the following overall observations. 


\bb \hspace{-1mm} \emph{1.ML techniques are effective for UMs but ineffective for CAMs.} 
We examine the performance for ML techniques on UMs, 
all of which outperform state-of-the-art CAMs. It confirms the ML techniques are ineffective for CAMs.

\bb  \emph{2.Decoupled CAMs produced under the new framework all outperform prior works.} 
We see a consistent improvement when decoupled CAMs models have better performance than prior CAMs and most UMs except for the boosting.
It confirms that our modeling framework and a decoupling principle are essential. Note that Lin-PVEL algorithm described in Section XX attains the best performance, confirming the efficacy of our heuristics. 

\bb   \emph{3. Consolidation/Ensemble aggregation.}  While comparing correlations and $t$-statistics guides our understanding of which individual model performs better, the more important overarching question, especially for practitioners, is to understand whether a new model has ``orthogonal'' prediction power compared to the other models. To this end, when we overlay a simple boosting algorithm over all the methods we examine, we produce a forecast that outperforms any single individual model on every performance metric (the last row of Table~\ref{main_table}). 
This confirms the value of building multiple CAMs. 
See App.~\ref{sec:consolidateapp}. 


\myparab{Remarks on baselines}
\bb \emph{(i) \textsc{SFM}~\cite{zhang2017stock}}. \textsc{SFM} is a recent UM model. SFM decomposes the hidden states of an LSTM network into multiple frequencies by using Discrete Fourier Transform (DFT) such that the model captures signals at different horizons. 
% 
\bb \emph{(ii)~HAN~\cite{hu2018listening}.} HAN is a recent CAM model. This work introduces a so-called hybrid attention technique that translates news into signals. 
%
\bb \emph{(iii)~ \textsc{AlphaStock}~\cite{wang2019alphastock}.}  \textsc{AlphaStock} is the most recent end-to-end CAM model, which
uses deep learning to uncover the latent positions of the stocks, and then leverages them to produce forecasts. We remove its reinforcement learning component (which translates signals into positions) and keep only the components that produce return forecasts. 

\qq{end of the exp.}



%We propose a scalable theoretically sound end-to-end pipeline and evaluation framework  for embedding stocks in a latent low-dimensional space and leveraging this representation for subsequent prediction tasks. 
%Our main contribution is three fold: 

% \MC{Do we have space for a conclusion section?} 




\newpage

\section*{Broader Impact}

Our work can potentially increase the competitiveness of quantitative investment. In general, building stronger predictive models could make adversarial impact to less-competitive investment managers and cost their jobs in some circumstances~\cite{schoning2018s}.

%\textbf{(From Neruips FAQ) Does the eight-page limit include references?} Answer: No. The page limit refers to content pages only; \textbf{additional pages containing the impact statement and references are allowed.} Acknowledgements and funding disclosure should also be included here, but only for the camera-ready submission.

\fi

==> abtract.tex <==



\begin{abstract}
%We study algorithms for embedding stocks in a low-dimensional latent space for uncovering latent lead-lag relationships between the stock returns. We propose a modeling framework under the so-called {\color{red}\emph{additive influence embedding}} assumption that enables us to decouple the estimation of the stocks' latent positions from learning the nonlinear link function between the stocks.
%To learn the latent positions, we use high-dimensional kernel-based techniques to design a provably correct algorithm.
%To learn the link function, we introduce two new algorithmic techniques, including a statistically sound non-parametric method and an ensemble learning algorithm optimized for vector regressions. 
%Extensive experiments demonstrate that the new algorithms deliver significantly stronger forecasting power compared to standard baselines and other recent state-of-the-art methods in the literature.

To solve the problem of forecasting equity returns and capturing the interactions between assets, we propose a novel framework, which we call an \emph{additive influence model.}

Under our modeling assumption, we show that it is possible to decouple the learning of high-dimensional cross-asset interactions from the learning of feature interactions.
 
To learn the cross-asset interactions, we adopt/leverage kernel-based techniques, with provable guarantees, to embed the stocks in a low-dimensional latent space. To learn the feature interactions, we generalize prominent machine learning techniques, including designing a new statistically sound non-parametric method and an ensemble learning algorithm optimized for vector regressions. 
Extensive experiments demonstrate that our new algorithms deliver significantly stronger forecasting power compared to standard and recently proposed methods. 
%estimation of the stocks' latent positions from learning the nonlinear link function between the stocks.

%We study the problem of forecasting equity returns using cross-asset pricing models. We propose a novel framework called the \emph{additive influence model} to capture the interaction between stocks. 


%{\color{red} major to prominent}
%{\color{red} disc. moved after concl.}

%\red{Is there a better word for "major" (in the abstract and throughout the paper) when we say "major ML techniques". Perhaps established/conventional/mainstream/prominent?} 

%We study algorithms for embedding stocks in a low-dimensional latent space for uncovering latent lead-lag relationships between the stock returns. On the theoretical side, we design the first prediction algorithm with provable performance guarantees under a widely used  embedding model. The algorithm first estimates the latent positions of the stocks, and then learns the nonlinear interaction function between the stocks. On the practical side, we enhance the theoretical algorithms by introducing new machine learning techniques, which include a simplified deep learning architecture and a time-efficient boosting algorithm. In our extensive experiments, the new algorithms deliver significantly stronger forecasting power compared to standard baselines and other recent state-of-the-art methods in the literature. 
\end{abstract}


==> algorithm_nips.tex <==

\section{Our learning algorithms}   
\label{sec:ourAlgos}

This section describes our algorithm, which consists of two major components: 

\myparab{1. Theoretically sound algorithms.} In Section XXX, we describe a theoretically sound algorithm to recover the latent positions. Then we describe a polynomial time algorithm to infer the function $g(\cdot)$ when $\mx_{t, i} \in \reals^{k}$ with $k = O(1)$. 

\myparab{2. New machine learning techniques.} In Section XXX, we explain how we can integrate deep learning and boosting techniques with the latent position estimation algorithm to construct optimized models. 


\subsection{Theoretically sound algorithms}
This section describes two algorithms. The first algorithm aims to estimate the latent positions of the stocks. The second algorithm aims to estimate the unknown function $g(\cdot)$. The performance of these algorithms is characterized by the following theorem. 

\begin{theorem} {\color{blue} Describe the final performance.}
\end{theorem}


\subsubsection{Algorithms for finding latent positions}

{\color{blue} ZL: the name of our model is latent stock embedding model.}

\MC{I think $n$ appears here for the first time..it should be made clear what it indexes: }

\begin{proposition} Consider running {\color{red} Algorithm XX} to learn the latent stock embedding model. 
\end{proposition}

Let $\mY \in \reals^{n \times d}$ such that $\mY_{t, i} = \my_{t, i}$ ($\mY$ emphasizes that we work with a cross-sectional  collection of data, whereas $\my_{t, i}$ emphasizes that it is a univariate random variable). Similarly, we let $\mS \in \reals^{n \times d}$ be such that $\mS_{t, i} = \ms_{t, i}$. Note that because $\mx_{t, i}$'s are independent, $\ms_{t, i}$ are also i.i.d. We have $\E[\ms_t \ms^{\transpose}_t] = \lambda I$ for some $\lambda$. Wlog, we shall assume that $\lambda = 1$. {\color{blue} ZLiu: please check that relaxing this assumption is fine. }
Let $E \in \reals^{n \times d}$ such that $E_{t, i} = \xi_{t, i}$. Finally, recall that $K \in \reals^{d\times d}$ such that $K_{i,j} = \kappa(\mz_i, \mz_j)$. 
%
%
\begin{figure}
\begin{codebox}
\Procname{$\proc{Estimate-K}(\mY, \mX)$}
\li $[V, \Sigma, V^{\transpose}] = \mathrm{svd}\left(\frac 1 n\mY^{\transpose}\mY\right)$
\li Let $\sigma_i = \Sigma_{i,i}$ 
\li \Comment {\color{red} be careful $\lambda_i$ vs $\sigma_i$.}
\li \Comment $\delta$ a tunable parameter. 
\li $i^* = \max \{\lambda_{i^*} - \lambda_{i^*+1} \geq \delta d^2\}$.
\li \Return $\hat K = \calP_{i^*}(V\Sigma^{\frac 1 2}V^{\transpose})$
\end{codebox}
\caption{Our algorithm for estimating $K$.}
\label{fig:estimatek}
\end{figure}
%
%
Having established this matrix notation, \eqref{eqn:model} now becomes 
\begin{equation}
    \mY = \mS K + E. 
\end{equation}
Our goal is to infer $K$ from only observing the cross-sectional stock returns $\mY$. Our key observation is that 
\begin{align*}
    \frac 1 n \my^{\transpose} \mY = K^{\transpose}\frac 1 n \mS^{\transpose} \mS K + \frac 1 n K^{\transpose}\mS^{\transpose}E + \frac 1 n E^{\transpose}\mS K + \frac 1 n E^{\transpose}E \approx K^{\transpose}K = K^2.  
\end{align*}
\qq{$\mY^{\transpose} \mY$? in the above equation?}
This is because $\frac 1 n \mS^{\transpose}\mS \approx I$ and $\frac 1 n \left(K^{\transpose}\mS^{\transpose}E + E^{\transpose}\mS K + E^{\transpose}E\right) \approx 0$ (one can check that the expectation is $0$; we shall also show that it concentrates quite well with high probability). 

While $\frac 1 n \mY^{\transpose}\mY \approx K^2$, it is quite non-trivial to obtain an approximation of $K$ from $\frac 1 n \mY^{\transpose}\mY$. In fact, standard matrix analysis CITE gives that

\begin{align}
\mbox{If } \|A A^{\transpose} - B B^{\transpose}\|^2_F \mbox{ is small, \quad \quad then } \|A - B W\|^2_F = O\left( \frac{\|AA^{\transpose} - BB^{\transpose}\|^2_F}{\sigma_{\min}(B)}\right)\label{eqn:gapcost}
\end{align}

{\color{red} CHECK} where $W$ is a unitary matrix. When we apply the result to our setting, we obtain an estimation of $K$ with an error in the order of $\frac{\|\frac 1 n\mY^{\transpose} \mY - K^2\|^2_F}{\sigma_{\min}(K)}$. Note that $\sigma_{\min}(K)$ can be arbitrarily small \emph{so it is difficult to obtain an approximation of $K$ even approximating $K^2$ is easy.} \MC{could be clarified better} 

We tackle this problem by leveraging three (CHECK) tools: 

\mypara{1. $K$ is near low-rank by kernel learning.} Specifically, \emph{(i)} The eigenvalues of the function $\kappa(\cdot, \cdot)$  decays exponentially when $k\kappa(\cdot, \cdot)$  \MC{??} is sufficiently smooth (e.g., $\lambda_i \leq \exp(-c i^{1/r})$ in the case of RBF; see also {\color{blue}REF}).  \emph{(ii)} The eigenvalues of $K$ converges to those of $\kappa(\cdot, \cdot)$. 

\mypara{2. Any near-low rank matrix is ``decomposible''.} We need only find an $i^*$ such that $\lambda_{i^*}(K)$ is sufficiently large (so that the additional gap cost in Eq.~\ref{eqn:gapcost} does not kill us). In addition, we need to ensure $\sum_{i > i^*}\lambda^2_i$ is $o(1)$ so that the reconstructino error is small. This is trivial when we know the parametric form of $\lambda_i$ (e.g., if $\lambda_i = \exp(-c i^{1/r})$) but it becomes more subtle when we have only an upper bound. We utilize a recent result developed for high dimensional statistics to get that $K$ can be decomposed into $\calP_{i^*}(K)$ and $K^{\bot} \triangleq K - \calP_{i^*}(K)$ such that $\lambda^{-1}_{i^*}(K) = o\left(\left\|\frac 1 n \mY^{\transpose}\mY - K\right\|\right)$ (gap does not kill us) and $\sum_{i > i^*}\lambda^2_{i^*} = o(1)$ (reconstruction error is small). 


{\color{blue} where should this block of text go?}
Let $\calP_r(A)$ be a rank-$r$ approximation of $A$ (by keeping top-$r$ singular values/vectors). By the Eckart-Young theorem  \cite{eckart1936approximation}, $\calP_r(A)$ is the rank-$r$ approximation of $A$ with the lowest Frobenius error.  Because the smallest eigenvalue of $\calP_{i^*}\left(\frac 1 n \mY^{\transpose}\mY\right)$ is $\delta$, the difference of the square roots of $\calP_{i^*}(K^{\transpose}K)$ and $\calP_{i^*}\left(\frac 1 n \mY^{\transpose}\mY\right)$ becomes manageable. 



\begin{proposition}\label{prop:yykk} Consider the problem of learning the latent position model \MC{cite a eqn maybe?}. Let $n$ be the number of observations. Let $\mY \in \reals^{n \times d}$ be that $\mY_{i, :}$ contains the $i$-th observation. Assume that $n \leq d^2$. With overwhelming probability, it holds true that 
\begin{align}
    \left\|\frac 1 n \mY^{\transpose}\mY - K^{\transpose}K\right\|_F = O\left(\frac{d^2 \log^3 n}{\sqrt n}\right).
\end{align}
\end{proposition}


{\color{blue} define ``overwhelming probability''. Also, think about how the assumption $n \leq d^2$ can be relaxed (things will look uglier).}


\begin{proof}
We can see that 

\begin{align}
    \frac 1 n \mY^{\transpose} \mY & = \frac 1 n\left(K^{\transpose}\mS^{\transpose}\mS K + K^{\transpose}\mS^{\transpose} E + E^{\transpose} \mS K + E^{\transpose}E\right) \\
    & = K^{\transpose}K + \cale_1 + \cale_2 + \cale_3 + \cale_4, 
\label{th:decompYtY}    
\end{align}
where $\cale_1  = K^{\transpose}\left(\frac{\mS^{\transpose} \mS}{n} - I\right)K$, $
    \cale_2  = \frac{K^{\transpose}\mS^{\transpose}E}{n} $, 
    $\cale_3  = \frac{E^{\transpose}\mS K}{n}$, and $\cale_4  = \frac{E^{\transpose}E}{n}$


We next show that each $\cale_i$ ($i \leq 4$) is small. 

\myparab{Bounding $\cale_1$.} 
We need the following lemma. 


{\color{red} todo: for ZZ: check the correctness of the lemma.}
\begin{lemma} Let 
$\mS \in \reals^{n \times d}$ be such that each row $\mS_{i, :}$ is an i.i.d. random vector $\|S_{i, :}\|_{\infty} \leq 1$ and 
$\E[\mS^{\transpose}_{i, :}\mS_{i, :}] = I$. We have 
\begin{equation}
    \Pr\left[\left\|\frac{\mS^{\transpose}\mS}{n} - I_{d \times d}\right\|_2 \geq \epsilon\right] \leq 2 n^2 \exp\left(-\frac{n \epsilon^2}{\log^4n}\right),
\end{equation}
where $\epsilon$ is a tunable parameter. 
\end{lemma}


Here, we shall set $\epsilon = \frac{\log^3 n}{\sqrt n}$. This implies that with high probability $\left\|\frac{\mS \mS^{\transpose}}{n} - I_{d \times d}\right\|_2 = O\left(\frac{\log^3 n}{\sqrt n}\right)$. 

On the other hand, we can see that $\|K\|^2_F = \Theta(d^2)$ and $\|K\|_F = \Theta(d)$. This implies 

\begin{equation}
    \|\cale_1\|_F = \left\|K^{\transpose}\left(\frac{\mS \mS^{\transpose}}{n} - I_{d \times d}\right)K\right\|_F \leq \left\|\frac{\mS\mS^{\transpose}}{n} - I_{d \times d}\right\|_2 \|K\|^2_F = \Theta\left(\frac{d^2 \log n}{\sqrt n}\right)
\end{equation}

\myparab{Bounding $\cale_2$ and $\cale_3$.} 
Recall that $\cale_2 = \frac{K^{\transpose}\mS^{\transpose}E}{n}$ and $\cale_3 = \frac{E^{\transpose}\mS K}{n}$. We have the following lemma. 


\begin{lemma}\label{lem:se}Let $\mS \in \reals^{n \times d}$ be such that each row $\mS_{i, :}$ is an i.i.d. random vector with $\|\mS_{i, :}\|_{\infty} \leq 1$ and $\E[\mS^{\transpose}_{i, :}\mS_{i, :}] = I$.  Let $E \in \reals^{n \times d}$ be such that $E_{i,j}$ are i.i.d. Gaussian with standard deviation $\sigma_{\xi}$. We have with overwhelming probability
\begin{equation}
    \|\mS^{\transpose} E\|^2_F \leq c_0 \sigma_{\xi}d^2 n
\end{equation}
for some constant $c_0$. 
\end{lemma}
\begin{proof}[Proof of Lemma~\ref{lem:se}] First, note that 
\begin{align*}
    \E[\|\mS^{\transpose}E_{:, i}\|^2_F \mid \mS] = \sigma^2_{\xi}\|S\|^2_F. 
\end{align*}
Therefore, we have $\E[\|\mS^{\transpose}E_{: ,i} \|^2_F] = \sigma^2_{\xi}d n$. This also implies that 
\begin{align*}
    \E[\|\mS^{\transpose}E\|^2_F] = \sum_{i \leq d}\E[\|\mS^{\transpose}E_{:,i}\|^2] = \sigma^2_{\xi}d^2n. 
\end{align*}
By a standard Chernoff bound, we have whp 
\begin{equation}
    \|\mS^{\transpose}E\|^2_F \leq c_0 \sigma^2_{\xi}d^2 n 
\end{equation}
for some constant $c_0$.
This means with high probability $\|\mS^{\transpose}E\|_F = O(d \sqrt{n})$. 
\end{proof}

{\color{red} we treat $\sigma_{xi}$ as a constant. Mabye need to fix it.}

We next use Lemma~\ref{lem:se} to bound $\cale_2$ and $\cale_3$:
\begin{equation}
    \|\cale_2 \|_F = \|\cale_3\|_F = \frac 1 n \|K^{\transpose}\mS^{\transpose}E\|_F = \frac 1 n \|K\|_2 \|\mS E\|_F. 
\end{equation}

Now we have $\|K\|_2 = O(d)$ (see {\color{blue} Lemma X in Appendix}) and $\|\mS E\|_F = O(d \sqrt n)$ whp. Therefore, with high probability 
\begin{equation*}
    \|\cale_2 \|_F = \|\cale_3 \|_F = O\left(\frac{d^2}{\sqrt n}\right).
\end{equation*}


\myparab{Bounding $\cale_4$.} With the assumption that $d = O(n)$, we have 
\begin{equation}
    \left\|\frac{E^{\transpose} E}{n}\right\|^2_F \leq \frac{\Rank(E^{\transpose}E)\|E\|^2_2}{n} = O\left(\frac{dn}{n}\right) = O(d).  
\end{equation}

Above, we used a finite sample version of semi-circle law (i.e., $\|E\|^2_2 = O(n)$ whp~\cite{rudelson2010non}). 


Summing up above and using that  $n < d^2$, we have $\left\|\frac 1 n\mY^{\transpose}\mY - K^{\transpose}K\right\|_F = O\left(\frac{d^2 \log^3 n}{\sqrt n}\right).$
\end{proof}




{\color{blue} ZLiu: this block of text will need to be polished and also converted into pseudocode.}

{\color{blue} ZLiu: (i) give a name to our model; at this moment it is ``latent stock embedding model;'' (ii) is it ``latent stock embedding'' or ''stock latent embedding''. Sounds to zliu the former.}

\begin{proposition}\label{prop:estimatek} Consider running Algorithm $\proc{Estimate-K}$ in Fig.~\ref{fig:estimatek} to learn the latent stock embedding model. Let $\epsilon = \omega \left(\frac{\log^3 n}{\sqrt n}\right)$ and $\delta^3 = \omega(\epsilon^2)$. We have $\frac 1 {d^2}\|K - \hat K\|_F =O\left(\frac{\epsilon^2}{\delta^3} + \delta^{\frac 4 5}\right)$.
\end{proposition}

{\color{blue} It looks we should set $\delta = \epsilon^{\frac{10}{19}}$.}

\myparab{Proof of Proposition~\ref{prop:estimatek}.} We now move to the proof of Proposition~\ref{prop:estimatek}. 
We shall let $A = \frac 1{d^2} K^{\transpose}K$ and $B = \frac{1}{d^2 n} \mY^{\transpose}\mY =  \frac{1}{d^2}(K^{\transpose}K + \cale)$, where $\cale = \cale_1 + \cale_2 + \cale_3 + \cale_4$ defined in \eqref{th:decompYtY}. By Lemma~\ref{prop:yykk}, we have whp $\|A - B\|_F = O\left(\frac{\log^3 n}{\sqrt n}\right)$. We shall also define 
\begin{itemize}
    \item $V^A_k$ be the first $k$ eigenvectors associated with $A$; $V^B_k$ be the first $k$ eigenvecotrs associated with $B$. Note that $A$ and $B$ are symmetric. 
    \item $\calP_A = V^A_{i^*}(V^A_{i^*})^{\transpose}$ and $\calP_B = V^B_{i^*}(V^B_{i^*})^{\transpose}$, where $i^*$ is defined in Algorithm {\color{red} XXX}. 
\end{itemize}

Next, note that for any PSD matrix $A$, the ``square root'' of it (i.e., $A^{\frac 1 2}$ such that $(A^{\frac 1 2})^{\transpose}A^{\frac 1 2} = A$) is not unique. Any two pairs of square roots differ by only a unitary matrix. We use the following (standard) definition to measure the difference between two matrices. 

\begin{definition} (Distance between two matrices) Let $X, Y \in \reals^{d_1 \times d_2}$. The distance between $X$ and $Y$ is defined as 
\begin{equation}
    \dist^2(X, Y) = \min_{W \mbox{ unitary}} \|XW - Y\|^2_F. 
\end{equation} 
\end{definition}

Next, we introduce our main building block that allows us to decompose $K$ into a low rank matrix and a negligible one. 

The result below was proved in~\cite{wu2019adaptive}. {\color{red} need to check the rigorousness of this result; also check whether the parameters are tuned correctly. }

\begin{lemma} Let $\{\lambda_i\}_{i \geq 1}$ be a sequence such that $\sum_{i \leq n}\lambda_i = 1$, $\lambda_i \leq c i^{-\omega}$ for some constant $c$ and $\omega \geq 2$. Assume also that $\lambda_1 < 1$. Define $\delta_i = \lambda_i - \lambda_{i + 1}$ for $i \geq 1$. Let $\ell_0$ be a sufficiently large number and $c_1$ and $c_2$ are two suitable constants. Let $\ell$ be any number such that $\ell \geq \ell_0$. There exists an $i^*$ such that 
\begin{equation}
    \delta_{i^*} \geq c_1 \ell^{-(\omega+1)} \quad \mbox{ and } \sum_{i \geq i^*} \lambda_i \leq c_2 / \ell^{-(\omega-1)}. 
\end{equation}
\end{lemma}

The above lemma also implies that 
\begin{equation}
    \sum_{i \geq i^*}\lambda_i = O\left(\delta^{\frac{\omega - 1}{\omega + 1}}\right) = O(\delta^{\frac 4 5}). 
\end{equation}

{\color{blue} ZLiu: to appendix.}
\begin{lemma}\label{lem:sqrt} (From~\cite{bhojanapalli2016dropping}) For any two rank-$r$ matrices $U$ and $X$, we have
\begin{align*}
    \dist^2(U, X) \leq \frac{1}{2(\sqrt 2 - 1) \sigma^2_r(X)}\|U U^{\transpose} - X X^{\transpose}\|^2_F. 
\end{align*}
\end{lemma}


{\color{blue} ZLiu: to appendix.}
\begin{lemma}\label{lem:M1M2} (From~\cite{ge2017no}) Let $M_1$ and $M_2$ be two matrices such that 
\begin{equation}
    M_1 = U_1 D_1 V^{\transpose}_1 \quad \mbox{ and } \quad  M_2 = U_2 D_2 V^{\transpose}_2. 
\end{equation}
We have 
\begin{equation}
    \|U_1 D_1 U^{\transpose}_1 - U_2 D_2 U^{\transpose}_2\|^2_F + \|V_1 D_1 V^{\transpose}_1 - V_2 D_2 V^{\transpose}_2\|^2_F \leq 2 \|M_1 - M_2\|^2_F. 
\end{equation}
\end{lemma}


{\color{red} ZLiu: need to check the correctness of the lemma.}
\begin{lemma}\label{lem:gap}
Consider running Algorithm $\proc{Estimate-K}$ in Fig.~\ref{fig:estimatek} for estimating $K$. Let $A = \frac 1 {d^2}K^{\transpose}K$ and $B = \frac 1 {d^2 n} \mY^{\transpose} \mY$. Let $\calP_A$ and $\calP_B$ be defined above. Let $\delta$ be the gap parameter specified in Algorithm XXXX. We have
\begin{equation}
    \|\calP_A - \calP_B \|_2 = \frac{\|A - B\|_2}{\delta}. 
\end{equation}
\end{lemma}
{\color{red} ZLiu to Zheng: please provide a self-contained proof for Lemma~\ref{lem:gap}. Can examine our ARRR paper or our Neruips paper.}

Let $A_{i^*} = \calP_{A}(A) (= \calP_{i^*}(A))$ and $B_{i^*} = \calP_{i^*}(B)$. Lemma~\ref{lem:gap} also gives us that 

\begin{align*}
    \|A_{i^*} - B_{i^*}\|_F = & \|\calP_A(A) - \calp_B(B)\|_F \\
    = & \|\calP_A(A) - \calP_B(A) + \calP_B(A) - \calP_B(B)\|_F \\
    \leq & \|\calP_A - \calP_B\|_2 \|A\|_F + \|A- B\|_F \\
    \leq & \Theta(\frac{\epsilon}{\delta} + \epsilon) = \Theta(\epsilon/\delta). 
\end{align*}

Now we are ready to prove Proposition~\ref{prop:estimatek}. Define 
\begin{align*}
    A^{\frac 1 2}_{i^*} = U^A_{i^*}(\Sigma^A_{i^*})^{\frac 1 2} \quad \mbox{ and } \quad  B^{\frac 1 2}_{i^*} = U^B_{i^*}(\Sigma^B_{i^*})^{\frac 1 2}
\end{align*}

By Lemma~\ref{lem:sqrt}, we have 
\begin{align*}
    \dist^2(A^{\frac 1 2}_{i^*}, B^{\frac 1 2}_{i^*}) \leq \frac{1}{2(\sqrt{2} - 1) \delta}\left(\frac{2\epsilon}{\delta} + \epsilon\right)^2 = \Theta\left(\frac{\epsilon^2}{\delta^3}\right). 
\end{align*}


This means that there exists a unitary matrix $W$ such that 
\begin{equation}
    \| U^A_{i^*}(\Sigma^A_{i^*})^{\frac 1 2}W - U^B_{i^*}(\Sigma^B_{i^*})^{\frac 1 2}\|^2_F = O\left(\frac{\epsilon^2}{\delta^3}\right). 
\end{equation}

Now by Lemma~\ref{lem:M1M2}, we have 

\begin{align*}
    \|U^A_{i^*}(\Sigma^A_{i^*})^{\frac 1 2} U^A_{i^*} - U^B_{i^*}(\Sigma^B_{i^*})^{\frac 1 2}U^B_{i^*}\|^2_F = O\left(\frac{\epsilon^2}{\delta^3}\right),  
\end{align*}
which implies $\|\frac{1}{d^2}\hat K - \frac 1{d^2}K\|_F = O\left(\frac{\epsilon^2}{\delta^3}\right)$ {\color{blue} bug: the tail is missing.}. 


{\color{blue} remark: we need another level of normalization so that eigenvalues of $A$ and $B$ are of the same scale of $\kappa$.} 

{\color{blue} this is another lemma that comes from from which world.} 

{\color{blue} move around set up of notations.}

\begin{figure}
\begin{codebox}
\Procname{$\proc{Estimate-g}(\hat K, \{\Omega_i\}_{i \leq \ell}, \mX, \mY)$}
\li \For $j \gets 1$ \To $d$
\li \Do 
$\mx_t = \mX_{t, :}$, $\my_t = \mY_{t, :}$
\li $q_i = \mathrm{Rand}(d)$.
\li $\vec C_t = \proc{Reduce-to-Regress}(\hat K_{q_i, :}, \mx_t)$
 \End
\li $\mu_1, \dots \mu_{\ell} \gets \proc(Solve-Regression)(\{\my_t, \vec C_t\}_{t \leq n})$. 
\li \Return $\mu_1, \dots \mu_{\ell} $
\end{codebox}

\begin{codebox}
\Procname{$\proc{Reduce-to-Regression}(L, \mx_t)$}
\li \Comment $L \in \reals^d$. 
\li $\vec C_{t, i} \gets 0$ for $i \in [\ell]$
\li \For $j \gets 1$ \To $d$
\li \Do 
Let $i_j$ be that $\mx_{t, j} \in \Omega_{i_j}$
\li $\vec C_{t, i_j} \gets \vec C_{t, i_j} + L_j$
 \End
\li \Return $\vec C_t$
\end{codebox}

\begin{codebox}
\Procname{$\proc{Solve-Regression}(\{\my_t, \vec C_t\}_{t \leq n})$}
\li \For $i \gets 1$ \To $\ell$
\li \Do 
\For $t\gets 1$ \To n
\li \Do
$b_i = \vec C_{t, i} > 0 ? 1: -1$
\End
\li  $\mu_i = \frac{\sum_{t \leq n}b_t \vec C_{t, i}}{\sum_{i \leq n}b_t \my_t}$
 \End
\li \Return $\{\mu_i\}_{i \leq \ell}$
\end{codebox}
\caption{Our algorithm for estimating $g(\cdot)$.}
\label{fig:estimatek}
\end{figure}


\subsubsection{Non-parametric estimation of the function $g(\cdot)$}
Recall that in our model we have $\my_{t, i} = \sum_{j \leq d} K_{j,i} g(\mx_{t,j}) + \xi_t$, where we have an estimate of $K$, know that $\mx_t$ are i.i.d. distributed, and $g(\mx_t)$ is smooth. Our goal is to estimate $g(\cdot)$. 

\myparab{Design intuition.} We first walk through our design intuition. We shall start with reviewing the simplest non-parametric technique for estimating smooth functions. Then we examine how the estimation techniques can be generalized in our setting when we assume $K$ is known. Finally, we explain the challenge of analyzing the convergence behavior in the presence of noise. 

{\color{blue} ZLiu: todo: define smooth function; does smooth imply continuous?}

{\color{red} ZLiu: be careful to check notation usage; ZLiu used some $\ell$ incorrectly.}

\mypara{Piece-wise constant approximation.} Consider a simplified problem $\my = g(\mx) + \xi$, in which 
$\mx \in [-1, 1]$ and $g(\mx)$ is smooth. We may partition $[-1, 1]$ into a total number of $\ell$ intervals such that $\Omega_i = [-1 + (i - 1) \epsilon, -1 + i \epsilon)$. We then use a constant to approximate $g(\cdot)$ for each interval, i.e., we shall let $\mu_i \approx g(\mx)$ when $\mx \in \Omega_i$ and our goal becomes to estimate $\{\mu_i\}_{i \leq \ell}$. Our estimation of $\mu_i$ is also straightforward. Let $X^{(i)}$ be the set of training data whose features fall into $\Omega_i$. We can simply estimate $\hat \mu_i = \frac{1}{|X^{(i)}|}\sum_{(t, j) \in X^{(i)}} \my_{t, j}$ {\color{blue} check notation. looks strange.} 

We make three remarks about this approach. 

\mypara{(i)} This approach uses the same assumption as near-neighbor based methods. Specifically, both reply on the assumption that $g(\mx)$ is smooth. 

\mypara{(ii)} To prove consistency/convergence result, we need to let $\ell = \omega(1)$ as $n$ (the number of samples) grows. This also resembles algorithms for neighbor-based methods. 

\mypara{(iii)} There is one minor bug in our algorithm. When we partition $[-1, 1]$ uniformly, we may have some $\Omega_i$ such that $\Pr[\mx \in \Omega_i]$ is small. In this case, it is more difficult to sample points from $\Omega_i$, causing a larger estimation variance (inaccuracy). So we should partition the support according to the probability mass for any two intervals such that $\Pr[\mx \in \Omega_i] = \Pr[\mx \in \Omega_j]$ for any $i \neq j$. 

{\color{blue} looks forget to mention: (i) we assume that the pdf for $\mx$ is known.}
We now generalize this idea to our setting. We shall partition the domain into ``cells'' $\{\Omega_i\}_{i \leq \ell}$ so that the mass of each cell is the same.\footnote{In our simplified example, we assume the support is $[-1, 1]$ so each partition is an interval; in the general setting, we assume the support is a high-dim compact set so each partition is a cell.} 

Then we use a constant $\mu_i$ to represent all $g(\mx)$ when $\mx \in \Omega_i$ like we did for the warm-up setting. The only difference is that in the simplified setting, we directly observe $(g(\mx_{t, i}) + \epsilon_{t, i}, \mx_{t, i})$, which means we directly observe an approximation of $\mu_i$ when $\mx_{t, i} \in \Omega_i$. But in our setting, we do not directly observe $\mu_i$. Instead, we observe a (noisy) linear combination of the unknowns, i.e., 
\begin{align*}
    \my_{t, i} = \sum_{j \leq d}K_{j, i}g(\mx_{t, j}) + \xi_{t, i} = \sum_{j \leq d} K_{j, i} \mu_{s_j} + \xi_{t, i}. 
\end{align*}
where $s_j$ is the index of the interval containing $\mx_{t, j}$. We can further rearrange the summation, i.e., 
\begin{align*}
\sum_{j \leq d} K_{j, i} \mu_{s_j} = \sum_{j \leq d}L_{(t, i), j}\mu_j. 
\end{align*}

Here, we define 
\begin{align*}
    L_{(t, i), j} = \sum_{k \in \calL_{t, j}}K_{k, i}, \mbox{ where } \calL_{t, j} = \{k: \mx_{t, k} \in \Omega_j\}.
\end{align*}

One can see that while the response is $\my_{t, i}$, $L_{(t, i), j}$ all depend on the same set $\calL_{t, j}$. Now our observation becomes 

\begin{equation}\label{eqn:toregression}
    \my_{t, i} = \sum_{j \leq \ell} L_{(t, i), j} \mu_j + \xi_{t, i} \mbox{ for all } t \mbox{ and } i. 
\end{equation}

%Here $L_{(t, i), j}$'s are known, $\xi_{t, i}$'s are noises, and $\mu_j$'s are unknown. This effectively reduces the problem into a linear regression problem, in which $\mu_j$'s are treated as coefficients to be estimated. 

\myparab{Solving the regression problem.} A natural way to solve the linear regression problem is to use MSE to find our estimator $\hat \mu_i$'s. We next highlight the challenges of analyzing the MSE-based estimator by considering a (simplified) special case $K_{i,j} = 1$. Now we can see that  

\mypara{(i)} Observations are not independent. Recall that when we treat the problem in Eq.~\ref{eqn:toregression} as a linear regression problem, we let $L_{(t, i),j}$'s be the features/covariates and let $\mu_i$ be the coefficients to be estimated. Now we note that when $t$ is fixed, each $\my_{t, i}$ is associated with features $L_{(t, i), j}$, which is controlled by the set $\calL_{t, j}$. This means that $L_{(t, i), j}$ are implicitly converted (through $L_{t, j}$), which also implies that the samples are not independent. 

\mypara{(ii)} Features in the same observation are correlated in a complex manner. let us now examine carefully how each of the coefficients in the same sample are correlated. Let us start with examining $L_{(t, i), 1} = \sum_{k \in \calL_{t, 1}}K_{k, i}\mu_1 = |\calL_{t, 1}|\cdot \mu_1$, where recall that $\calL_{t, 1} = \{k : \mx_{t, k} \in \Omega_1\}$. Generation of $\calL_{t, 1}$ can be interpreted as a balls-and-bins process: we sequentially go through each $k = 1, 2, \dots , d$. For each $k$, with probability $1/\ell$ that the ``$k$-th ball'' $\mx_{t, k}$ fall into $\Omega_1$. At the end, $\calL_{t, 1}$ consists of all the balls that fall into $\Omega_1$. 
This interpretation can be generalized to all other coefficients, i.e., $\my_{t, i} = \sum_{i \leq \ell}|\calL_{t, j}| \mu_j$, where $\{\calL_{t, j}\}_{j \leq \ell}$ is produced from the balls-and-bins process: we place $d$ balls into $\ell$ bins. The $j$-th coefficient $\mu_j$ corresponds to the number of balls in the $j$-th bin.

We now explain why it is ahrd to directly analyze the quality of the MSE estimator. 

\mypara{1. Only fluctuation matters.} We note that $\E[|\calL_{t, j}|] = \frac{d}{\ell}$. In addition, 
$\sum_{j \leq \ell}\E[|\calL_{t,j}|] \mu_j = 0$ (using the assumption $\E[g(\mx_{t,i})] = 0$) {\color{blue} ZLiu: need to explain how we should set up $\mu_j$.} Therefore, only the fluctuation of $|\calL_{t, j}|$ around the mean gives us useful information related to estimating $\mu_j$, i.e., the estimation problem is equivalent to 
\begin{align*}
    \my_{t, i} = \sum_{j \leq \ell}\left(|\calL_{t, j}| - \E[|\calL_{t,j}|]\right) \mu_j + \xi_{t, i}
\end{align*}

\mypara{2. The fluctuations are correlated across the features within the sample observation.} Specifically, we note that
\begin{equation}
    \sum_{j \leq \ell}\left(|\calL_{t, j}| - \E[|\calL_{t,j}|]\right) = 0
\end{equation}

\mypara{3. The features are correlated across observations.} Recall above that when $t$ is fixed, different features $L_{(t, i), j}$ are correlated for different $i$ {\color{blue} point to discussion above.} 

\mypara{4. Handling errors.} So far our discussion assumed that our knowledge of $K$ is accurate and ignore the approximation error $\mu_i - g(\mx)$ for $\mx \in \Omega_i$. 

{\color{blue} need a better wording for ignore}


Proving a concentration bound for using MSE to solve 
regressions requires us to produce a concentration result of the feature matrix. But in our feature matrix, both rows and columns are correlated (in a pretty complex manner). In addition, the feature matrix can be perturbed (due to the estimation error of $K$). Therefore, it becomes remarkably difficult to directly analyze the estimation quality. 

{\color{blue} ZLiu edit on 20200511 ends here.}

\mypara{Our intuition: reduction to a balls-and-bins process.} We next
outline our analysis. First, we build a model, in which the signal function $g(\cdot)$ is substituted by $\tilde g(\cdot)$, which indeed maps all points in the same $\Omega_i$ to a constant. In other words, in this model, we assume we obtain training data directly from the piece-wise constant function that approximates $g(\cdot)$. We shall show that a moment-based method suffices to recover all the constants. Then we move back to analyze the original process. There are two key differences between the processes we analyze and the true process. 

\mypara{(i)} We observe $g(\cdot)$ instead of $\tilde g(\cdot)$. Conceptually, we treate the difference between $g(\cdot)$ and $\tilde g(\cdot)$ as ``noise'' and shall argue that the noise does not make unmanageable impact to our estimations. 

\mypara{(ii)} We observe only $\hat K$ such that $\| \hat K - K \|^2_F\cdot \frac{1}{d^2} \leq \gamma$, where $\gamma = o(1)$, i.e., on average the entry-wise difference is small. We then argue that the error $\hat K - K$ also does not make much impact to the estimator. 



{\color{blue} legacy notations. $S^{(t,i)}_j$ in the old notation corresponds to $L_{t,j}$ in the new notations.}


{\color{red} ZL: looks there are still editing issues. This equation seems to be floating.}
Recall that 
\begin{align*}
    \my_{t, i} = K_{i, 1} g(\mx_{t, 1}) + K_{i, 2}g(\mx_{t, 2}) + \cdots + K_{i, d}g(\mx_{i, d}) + \xi_{t, i}. 
\end{align*}

We now move to execute the above idea. 

\mypara{(i) Define a discretized model.} We first define a discretized model and explain how we may design an algorithm to learn the model. 

We shall use the notation for the original model ({\color{blue} See Sec XX}). We shall let $\mu_i = \E[g(\mx_{t, i}) \mid \mx_{t, i} \in \Omega_i]$. Then we define a new function 
\begin{align*}
    \tilde g(\mx) = \mu_i, \mbox{ where } \mx \in \Omega_i.
\end{align*}

{\color{blue} give a name of the original problem.}
In the discritized stock embedding problem, we observe that 
\begin{align*}
    \my_{t, i} = \sum_{j \leq d}K_{j, i} \tilde g(\mx_{t, j}) + \xi_{t, i}. 
\end{align*}

We aim to estimate $\{\mu_i\}_{i \leq \ell}$ in this model. In what follows, we describe our algorithm to estimate $\mu_1$. 

Note that we have 
\begin{align*}
    \my_{t, i}& = \sum_{j \leq d} L_{(t, i), j} \mu_j + \xi_{t, i}\\
    & = \left(\sum_{k \in \calL_{t, 1}}K_{k, i}\right)\mu_1 + \sum_{k \notin \calL_{t, 1}} K_{k,i} \tilde g(\mx_{t, k} \mid \mx_{t, k} \notin \Omega_1) + \xi_{t, i}.
\end{align*}

We interpret the meaning of the above equation. We treat $\mx_{t, k}$ and $\calL_{t, j}$ as random variables. Then we can imagine that an observation is generated by using the following procedure. 

\begin{itemize}
    \item Step 1. Generate $\calL_{t, 1}$. This corresponds to determining the ``balls'' that need to fall into bin 1 ($\Omega_1$). 
    \item Step 2. Generate the rest of $\mx_{t, k}$ ($k \notin \calL_{t, 1}$) sequentially. Each $\mx_{t, k}$ is sampled from the conditional distribution $\mx_{t, k} \mid \mx_{t, k} \notin \Omega_1$. This explains the reason we write $\tilde g(\mx_{t, k} \mid \mx_{t, k} \notin \Omega_1)$. 
    \item Step 3. Generate $\my_{t, i}$ according to our discretized stock embedding model. 
\end{itemize}

With this interpretation in mind, we proceed to design our algorithm. 

\begin{fact} We have
\begin{align*}
    \E[g(\mx_{t, k}\mid \mx_{t,k} \notin \Omega_j] & = -\frac{\mu_j}{\ell-1} \\
    \E[\tilde g(\mx_{t, k}\mid \mx_{t,k} \notin \Omega_j] & = -\frac{\mu_j}{\ell-1} 
\end{align*}
\end{fact}
\begin{proof}
We shall prove the case for $g(\cdot)$. The case for $\tilde g(\cdot)$ can be proved in a similar manner. 

Note that by our model assumption,
\begin{equation}
    \E[\ms_{t, k}] = \E[g(\mx_{t, k})] = \mu_1 + \dots + \mu_{\ell} = 0. 
\end{equation}
On the other hand, 
\begin{align*}
    \E[g(\mx_{t,k} \mid \mx_{t, k} \notin \Omega_j] = \frac{\mu_1 + \dots + \mu_{j - 1} + \mu_{j+1}+ \dots + \mu_{\ell}}{\ell - 1} = - \frac{\mu_j}{\ell - 1}. 
\end{align*}
\end{proof}

Next we define the function 
\begin{align*}
    \tilde g_j(\mx_{t, i}) = \tilde g(\mx_{t, i}) - \E[\tilde g(\mx_{t, i}) \mid \mx_{t, i} \notin \Omega_j] = \tilde g(\mx_{t,i}) + \frac{\mu_j}{\ell - 1}. 
\end{align*}

Thus, $\tilde g(\mx_{t, i}) = \tilde g_j(\mx_{t,i}) - \frac{\mu_j}{\ell - 1} $. Therefore, we have
\begin{align}
    \my_{t,i} & = \underbrace{\left(\sum_{k \in \calL_{t, 1}} K_{i, k} - \left(\sum_{k \notin \calL_{t, 1}} K_{i,k}\right)\frac{1}{\ell - 1}\right)}_{\Pi^{(i)}_1(t)} \mu_1 + \underbrace{\sum_{k \in \calL_{t, 1}}K_{i,k} \tilde g_j (\mx_{t,i} \mid \mx_{t,i} \notin \Omega_1)}_{\Pi^{(i)}_2(t)} + \xi_{t,i} \label{eqn:fullrw}\\ & = \Pi^{(i)}_1(t) \mu_1 + \Pi^{(i)}_2(t) + \xi_{t, i} \nonumber.
\end{align}
{\color{orange} $K_{k, i}$ instead of $K_{i, k}$?}

We shall show that 
\begin{enumerate}
    \item With constant probability $|\Pi^{(i)}_1(t)| \geq \eta$ for $\eta$ to be calculated later. Also, let $b_{t, i} \in \{+1, -1\}$ be the sign of $\Pi^{(i)}_1(t)$. i.e., $b_{t, i} = 1$ if $\Pi^{(i)}_1(t) > 0$ and $b_{t, i} = -1$ otherwise. 
    \item $\E[\Pi^{(i)}_2(t) \mid \Pi^{(i)}_1(t)] = 0$. 
\end{enumerate}

We shall first briefly explain that how these two properties help us to estimate $\mu_1$. Fix an arbitrary $i$, let us compute 
\begin{align}
    \sum_{t \leq n}b_{t, i}\my_{t, i} = \left(\sum_{t \leq n}\left|\Pi^{(i)}_1(t)\right|\right)\mu_1 + \sum_{t \leq n}b_{t, i}\Pi^{(i)}_2(t) + \sum_{t\leq n}\xi_{t, i}.\label{eqn:walkovert}
\end{align}

{\color{blue} in the hand-written note, the last term $\sum_{t \leq n}\xi_{t, i}$ was accidentially not included. Need to check correctness for the analysis below.}.

The right hand side is effectively a ``drifted random walk'', in which $\sum_{t \leq n}|\Pi^{(i)}_1(t)|$ grows linearly in $\eta n$ whereas the term $\sum_{t \leq n}b_{t, i}\Pi^{(i)}_2(t)+\xi_{t, i}$ can be viewed as an unbiased random walk (each of the summands are independent and has a zero mean). Therefore,  $\sum_{t \leq n}|\Pi^{(i)}_1(t)|$ will become the dominating term as $n$ grows. This implies that $\left(\sum_{t\leq n} b_{t, i}\my_{t, i}\right)\left(\sum_{t \leq n}|\Pi^{(i)}_1(t)|\right)^{-1}$ could be a good estimator. 

We now concretely implement this idea. 

\myparab{Analysis of $\Pi^{(i)}_1(t)$.} Recall that 

\begin{align*}
    \Pi^{(i)}_1(t) = \sum_{k \in \calL_{t, 1}}K_{i, k} - \left(\sum_{k \notin \calL_{t, 1}}K_{i, k}\right)\frac{1}{\ell-1}. 
\end{align*}
We again have a random walk interpretation. But compared to (\ref{eqn:walkovert}), which corresponds to a walk over time, here the ``walk'' is over the columns of $K$. Specifically, for each $k \in [d]$, with probability $\frac{1}{\ell}$, it falls into $\calL_{t, j}$. When this happens, $\Pi^{(i)}_1(t)$ is incremented by $K_{i, k}$. With probability $1/\ell$, it does not fall into $\calL_{t,j}$. In this case, $\Pi^{(i)}_1(t)$ is decremented by $K_{i, k}/\ell$. {\color{blue} check whether we want $K_{i,k}$ or $K_{k, i}$.} We next make this random walk interpretation explicit (by coupling $\Pi^{(i)}_1(t)$ with a random walk). 

For $k \in [d]$, define a sequence of random variables 
\begin{align*}
    Z_k = \left\{
    \begin{array}{ll}
    K_{i,k} & \mbox{with probability }\frac 1 \ell.  \\
    -\frac{K_{i,k}}{\ell} & \mbox{with probability } 1-\frac 1\ell.  
    \end{array}
    \right.
\end{align*}

We can couple $\Pi^{(i)}_1(t)$ with $\{Z_i\}_{i \leq d}$ such that $\Pi^{(i)}_1(t) = \sum_{k \leq d}Z_i$. 

Let $\calF_k$ be the $\sigma$-algebra generated by $Z_1, \dots , Z_k$ (i.e., all information available up to time $k$). We can see that $\E[Z_k \mid \calF_{k - 1}] = 0$. We shall also an anti-concentration result on $\sum_{k \leq d}Z_k$. 

\begin{lemma}\label{lem:anti}Let $L_1, L_2, \dots, L_d$ be positive numbers such that $L_i = \Omega(1)$. Define a random variable 
\begin{align*}
    Z_i = \left\{
    \begin{array}{ll}
    L_i & \mbox{ with probability } \frac 1 {\ell}\\
    - \frac{L_i}{\ell} & \mbox{ with probability } 1- \frac{1}{\ell}.
    \end{array}
    \right.
\end{align*}
There exists a sufficiently small constant $c_0$ and a suitable constant $c_1$ such that 
\begin{align*}
    \Pr\left[\sum_{i \leq d}Z_i \geq \frac{c_0}{\log d}\sqrt{\frac{d}{\ell}}\right] \geq c_1
\end{align*}
\end{lemma}

\begin{proof} This is a folklore in the literature. For completeness, we provide a proof based on Littleword-Offord-Erdos. 

\begin{theorem}(Littleword-Offord-Erdos)
Let $L_1, \dots, L_d \geq 1$. Let $\xi_1, \dots \xi_n$ be independent Bernoulli $\pm 1$ unbiased random variables such taht $\Pr[\xi_i = 1] = \frac 1 2$. Let $S = \sum_{i \leq n}\xi_i L_i$. For any open interval $I$ of length 2, we have 
\begin{align}
    \Pr[S \in I] = O(n^{- \frac 1 2}). 
\end{align}
\end{theorem}

The original anti-concentration theorem requires that the random variable $\xi_i$ (or $Z_i$ in our setting) to be symmeetric, which is violated in our setting. Our goal is to reduce our problem to the original setting. 

We now show thow this can be done through ``debiasing'' the walk. 
We first define $\{B_i\}_{i \in [d]}$ such that $B_i$ is a random  binary indicator variable such $\Pr[B_i = 1] = \frac{\ell-2}{\ell}$ and $\Pr[B_i = 0] = \frac{2}{\ell}$. 

We may generate $Z_i$ by using $B_i$, i.e., when $B_i = 1$, $Z_i = -\frac{L_i}{\ell - 1}$, and when $B_i = 0$, then with $\frac 1 2$ probability that $Z_i = L_i$ and with $\frac 1 2$ probability that $Z_i = L_i$ and with $\frac 1 2$ probability that $Z_i = -\frac{L_i}{\ell- 1}$. Note that when $B_i = 0$, the probability that $Z_i$ takes one of the possible values in $\frac 1 2$ (thus is uniform).

{\color{blue} note that some assumption on $d/\ell$ is made in this paragraph. With high probability and with overwhemling probability probably should be the same.}
Next, let $\calB = \{B_i: B_i = 1\}$ and $\bar \calB = \{ B_i: B_i = 0\}$. Let also that $T = |\bar \calB|$. One can see that $\E[T] = \frac{2d}{\ell}$. In addition, because $d = \omega(\ell \log \ell)$, with overwhelming probability that $T \geq \frac{d}{\ell}$. 

We now can see that 
\begin{align*}
    \E\left[\sum_{i \in \calB}Z_i\right] = - \left(\sum_{i \leq d}L_i\right)\frac{\ell-2}{\ell(\ell-1)}
\end{align*}

In addition, $\E[Z_i \mid i \in \bar \calB] = L_i\left(1- \frac{1}{\ell - 1}\right)\frac 1 2$ for any $i \in \bar \calB$.
Next, we define a random variable to ``debias'' $Z_i$, conditioned on $i \notin \calB$, i.e., for any $i \in\bar \calB$

\begin{equation}
    \tilde Z_i = \left\{\begin{array}{ll}
L_{i} - L_i\left(1 - \frac{1}{\ell - 1}\right)\frac 1 2 & \quad \mbox{with probability $\frac 1 2$}    \\
-\frac{L_i}{\ell-1} - L_i\left(1 - \frac{1}{\ell - 1}\right)\frac 1 2 & \quad \mbox{with probability $\frac 1 2$.} 
\end{array} \right. 
\end{equation}
Note that $L_{i} - L_i\left(1 - \frac{1}{\ell - 1}\right)\frac 1 2 = 
-\frac{L_i}{\ell-1} - L_i\left(1 - \frac{1}{\ell - 1}\right)\frac 1 2 $. Next, we have 
\begin{align*}
    \sum_{i \leq d}Z_i &= \sum_{i \in \calB}\left[- \frac{L_i}{\ell-1}\right] + \sum_{i \in \bar \calB}\left(\tilde Z_i + L_i\left(1 - \frac{1}{\ell - 1}\right)\frac 1 2\right) \\
    & =  \underbrace{\left(\sum_{i \in \calB} \left(-\frac{L_i}{(\ell-1)}\right) + \sum_{i \notin \calB}  L_i\left(1 - \frac{1}{\ell - 1}\right)\frac 1 2\right)}_{\Psi_1} + \underbrace{\left(\sum_{i \notin \calB}\tilde Z_i\right)}_{\Psi_2}. 
\end{align*}

We have \emph{(i)} The sign of $\Psi_2$ is independent of the sign of $\Psi_1$.  \emph{(ii)} One of $\Pr[\Psi_1 \geq 0] \geq \frac 1 2$
 and $\Pr[\Psi_1 \leq 0] \geq \frac 1 2$ must hold. Wlog, assume that $\Pr[\Psi_1 \geq 0]\geq \frac 1 2$. By Little-Offord-Erods theorem, we have 
 $\Pr\left[|\Psi_2| \geq \frac{c_1}{\log d}\sqrt{T}\right] = \Omega(1)$.
 
Finally, we have 

\begin{align*}
    \Pr\left[\Psi_1 + \Psi_2 \geq \frac{c_1}{\log d}\sqrt{\frac{d}{\ell}}\right] & \geq \Pr[\Psi_1 \geq 0]\Pr\left[\Psi_2 \geq \frac{c_2}{\log d}\sqrt T \mid \Psi_1 \geq 0\right]\\
    & \geq \Pr[\Psi_ \geq 0]\Pr\left[\Psi_2 \geq \frac{c_1}{\log d}\sqrt{\frac{d}{\ell}} \mid \Psi_1 \geq 0\right] \\
    & = \Omega(1). 
\end{align*}

The second inequality uses $T \geq \frac{d}{\ell}$ whp. 
\end{proof}

We now move to explain our algorithm. Recall that $\my_{t, i} = \Pi^{(i)}_1(t) \mu_1 + \Pi^{(i)}_2(t) + \xi_{t, i}$ and we can see that 
\begin{align*}
    \sum_{t \leq n}b_{t, i}\my_{t, i} = \sum_{t \leq n}|\Pi^{(i)}_1(t)|\mu_1 + o(n). 
\end{align*}

So one candidate estimator is 
\begin{align*}
    \hat \mu_1 = \frac{\sum_{t \leq n}b_{t, i}\my_{t, i}}{\sum_{t \leq n}|\Pi^{(i)}_1(t)|}.
\end{align*}
A problem with this estimator is that $b_{t, i}$ (it is the sign of $\Pi^{(i)}_1(t)$) is very sensitive to perturbation when $\Pi^{(i)}(t)$ is near $0$. We also recall that $\Pi^{(i)}_1(t)$ is a function of $K$ but we have only an estimation of $K$ at best. So we need a bit of ``margin'' to improve the robustness of our algorithm. Define 

\begin{align*}
    \tilde b_{t, i} = \left\{
    \begin{array}{ll}
        1 & \mbox{ if } \Pi^{(i)}_1(t) \geq \frac{c_0}{\og d}\sqrt{\frac{d}{\ell}}  \\
        -1 & \mbox{ if } \Pi^{(i)}_1(t) \leq \frac{c_0}{\log d}\sqrt{\frac{d}{\ell}} \\
        0 & \mbox{otherwise.}
    \end{array}
    \right.
\end{align*}
{\color{blue} discussion/next iteration: do i use $\Pi^{(i)}_1(t)$ or $\hat \Pi^{(i)}_1(t)$?}

By Lemma~\ref{lem:anti} and standard concentration result, we have 
$\tilde b_{t, i}\Pi^{(i)}_1(t) \geq \frac{c_0}{\log d}\sqrt{\frac{d}{\ell}}$ with a constant probability (for a suitable $c_0$) and $\tilde b_{t, i}\Pi^{(i)}_2(t) \mid \Pi^{(i)}_1(t)$ scales in the order of $\sqrt d$ (CHECK). We shall define our estimator to be 

\begin{align*}
    \hat \mu_1 = \frac{\sum_{t \leq n}\tilde b_{t, i}\my_{t, i}}{\sum_{t \leq n}\tilde b_{t, i}\Pi^{(i)}_1(t)} = \mu_1 + \frac{\sum_{t \leq n}\tilde b_{t, i}\Pi^{(i)}_2(t)}{\sum_{t \leq n}\tilde b_{t, i}\Pi^{(i)}_1(t)} = \mu_1 + o(1).  
\end{align*}


{\color{blue} add somewhere} On the other hand, one can use standard concentration inequality to show that $\sum_{t \leq n}\tilde b_{t, i}\Pi^{(i)}_2(t) = O(\sqrt{nd})$. 
{\color{blue} end of add somewhere.}


We next move to analyze the original process, in which we have only an approximation $\hat K$ of $K$; and the observations are generated through the function $g(\cdot)$ instead of $\tilde g(\cdot)$. 

We first show how $\hat \mu$ is perturbed when $\hat K$ is used instead of $K$. Then we shall analyze the permutation from using $g(\cdot)$ instead of $\tilde g(\cdot)$. 

\myparab{Handling estimation error of $K$.} Recall that our algorthm {\color{blue} XX} gives an $\hat K$ such that $|\hat K - K|^2_F = \gamma d^2$ for $\gamma = o(1)$ whp. In addition, we can also ensure that $|\hat K - K|_{\infty} = O(1)$ because we know that $|K|_{\infty} = O(1)$ so we can set a hard threshold of $\hat K$ to ensure this happens. There are two types of estimation errors when we use $\hat K$ instead of $K$. 

\mypara{1. $\hat b_{t, i}$ is computed through $K$.} When $K$ is substituted by $\hat K$, $\tilde b_{t, i}$ can be inaccurate. We shall let $\hat b_{t, i}$ be the counterpart of $\tilde b_{t, i}$ when we use $\hat K$ instead of $K$ in Algorithm {\color{blue} XXX}. 

\mypara{2. $\Pi^{(i)}_1(t)$ and $\Pi^{(i)}_2(t)$ are also estimated through $K$.} Let $\hat \Pi^{(i)}_1(t)$ and $\hat \Pi^{(i)}_2(t)$ be the counterparts of $\Pi^{(i)}_1(t)$ and $\Pi^{(i)}_2(t)$ when we use $\hat K$ instead of $K$. 


We note that in the ideal algorithm presetned above, we fix an $i$ and collect all observations across time ($\my_{1, i}, \dots, \my_{t, i}, \dots \my_{n,i}$). There are two natural questions associated with this policy: 

{\color{blue} where is question 2?}

\mypara{Question 1. Do we need to fix $i$ in the presence of errors.} The discrepancy between $\Pi^{(i)}_1(t)$ and $\hat \Pi^{(i)}_1(t)$ (as well as between $\tilde b_{t, i}$ and $\hat b_{t, i}$) is a function of $\|K_{i, :} - \hat K_{i, :}\|^2_2$. For example, when $\|K_{i, :} - \hat K_{i, :}\|^2_2 = 0$, there is no discrepancy at all. Similarly when $\|K_{i, :} - \hat K_{i, :}\|^2_2$ is large, the discrepancy could be uncontrollable. On the other hand, we only have an ``average case'' bound between $K$ and $\hat K$ so that there is no guarantee that we can become ``lucky'' (that $\|K_{i, :} - \hat K_{i, :}\|_2$ is reasonable --- we in fact just want not that unlucky, i.e., so long as we get an average behaved $i$, we should be in good shape. But we cannot even be guaranteed to do that. We shall adopt a standard strategy to circumvent the problem, i.e., for each $t \in [n]$, we randomly sample an $i$ and our goal is that at the end the average errors produced from different $i$'s are comparable to always choose an ``average'' row (s.t. $\|K_{i, :} - \hat K_{i, :}\|^2_2 \approx \gamma d$). 

Let $q_t$ be the random row chosen at time $t$. Let $\hat \calB = \{ t \in [n]: \hat b_{t, i} \new 0\}$. Our goal is to show that: 

\begin{enumerate}
    \item $\left\|\sum_{t \in \hat \calB}\hat b_{t, i}\hat \Pi^{(q_t)}_1(t) - \sum_{t\in \hat \calB}|\Pi^{(q_t)}_1(t)| \right\|$ is small. 
    \item $\left|\sum_{t \in \hat \calB}(\hat \Pi^{(q_t)}_1(t) - \Pi^{(q_t)}_1(t)) \right|$ is small.{\color{red} check: whether there are typos?}
\end{enumerate}

\begin{lemma}\label{lem:absdiff} Consider running algorithm {\color{blue} XXX} to learn the discretized stock embedding model. Let $\hat K$ be such taht $|\hat K - K|^2_F \leq \gamma d^2$ for $\gamma = o(1)$. Let $\Pi^{(i)}_1(t)$ and $\hat \Pi^{(i)}_1(t)$ be those defined in {\color{blue} xx}. With high probability we ahve
\begin{align*}
    \sum_{t \leq n}\left|\hat \Pi^{(q_t)}_1(t) - \Pi^{(q_t)}_1(t)\right| \leq n \sqrt{\frac{\gamma d}{\ell}}\log d
\end{align*}
\end{lemma}
\begin{proof} Let $\Delta = \hat K - K \in \reals^{d \times d}$. We shall again use random walk techniques to analyze $\left|\hat \Pi^{(q_t)}_i(t) - \Pi^{(q_t)}_i(t)\right|$. Let 

\begin{align*}
    Z_i = \left\{
    \begin{array}{ll}
    \Delta_{q_t, i} &\mbox{with probability} \frac{1}{\ell}  \\
    -\frac{\Delta_{q_t, i}}{\ell - 1}     & \mbox{with probability } 1 - \frac{1}\ell. 
    \end{array}
    \right.
\end{align*}

We have $\E[Z^2_i] = O\left(\frac{\Delta^2_{q_t, i}}{\ell}\right)$, which implies that $\sqrt{\sum_{i \leq d}\E[Z^2_i]} = \sqrt{\frac{\sum_{i \leq d}\Delta^2_{q_t, i}}{\ell}}$. Now we can use Chernoff bound (let $\lambda_t$ be a tunable parameter). Specifically, one can see that 
\begin{align*}
    |\sum_{i \leq d}Z_i| = \left|\hat \Pi^{(q_t)}_i(t) - \Pi^{(q_t)}_i(t)\right|
\end{align*}

{\color{blue} check chernoff bound below.} Let $\lambda_t$ be a tunable parameter that is a function of $\sum_{i \leq d}\Delta^2_{q_t, 1}$. By using a standard Chernoff bound, we have 
\begin{align*}
    \Pr\left[\left|\sum_{i \leq d}Z_i\right|\geq \lambda_t \mid q_t\right] \leq \exp\left(- \frac{\lambda^2_t}{\frac 1{\ell}\left(\sum_{i \leq d}\Delta^2_{q_t,i}\right)+\frac{\lambda}{3}}\right), 
\end{align*}
Here, we set $\lambda_t = c_0 (\log d)\sqrt{\frac{\Delta^2(q_t)}{\ell}}$, where $\Delta^2(q_t) \triangleq \sum_{i \leq d}\Delta^2_{q_t, i}$. Now, conditioned on knowing $\{q_t\}_{t \leq n}$, we have with high probability 
\begin{align*}
    \sum_{t \leq n}\left|\hat \Pi^{(i)}_1(t) - \Pi^{(i)}_1(t)\right| \leq \sum_{t \leq n}\lambda_t = \frac{\log d}{\sqrt{\ell}}\sum_{t \leq n}\sqrt{\Delta^2(q_t)}. 
\end{align*}
Next, let us give a concentration bound for $\sum_{t \leq n}\sqrt{\Delta^2(q_t)}$. Let $v^2_i = \|K_{i, :} - \hat K_{i, K}\|^2$. We know that $\Delta^2(q_t)$ can only take values from $v_1^2, \dots , v^2_d$ with $\sum_{i \leq d}v^2_i = \|\hat K - K\|^2_F \leq \gamma d^2$. We have $\sqrt{\Delta^2(q_t)} \leq \sqrt{\gamma}d$. 

Now, using the condition that $\|\hat K - K\|^2_2 \leq \gamma d^2$, we have $\E[\sqrt{\Delta^2(q_t)}] \leq \sqrt{\gamma d}$ (using a Jensen inequality). 

We can use a Chernoff bound again and obtain 
\begin{align*}
    \Pr\left[\sum_{t \leq n}\sqrt{\Delta^2(q_t)} \geq \E\left[\sum_{t \leq n}\sqrt{\Delta^2(q_t)}\right]+\lambda\right] \leq \exp\left(-\frac{\lambda^2}{\gamma d n + \sqrt{\gamma d \lambda/3}}\right)
\end{align*}
We shall set $\lambda = \frac{\sqrt{\gamma d n}}{\log^2d}$ such that the right hand side is negligible. Now we have with high probability {\color{red} not completed here.}
\end{proof}

\myparab{Wrapping up the analysis for handling estimation error of $K$.} {\color{blue} this iteration: make sure notations and math are clear.}
To highlight the key variables' role in the analysis, we use the following abbreviations. 
\begin{itemize}
    \item $\hat b_t$ is an abbreviation for $\hat b_{t, q_t}$. 
    \item $\Pi_1(t)$ is an abbreviation for $\Pi^{(q_t)}_1(t)$. 
    \item $\Pi_2(t)$ is an abbreviation for 
    $\Pi^{(q_t)}_2(t)$. 
\end{itemize}

Recall that our estimator can be expressed as 
\begin{align*}
    \hat \mu &  = \frac{\left(\sum_{t \in \hat \calB}\hat b_t \Pi_1(t)\right) + \sum_{t \in \hat \calB}\left(\hat b_t \Pi_2(t) + \hat b_t \xi_{t,q_t}\right)}{\sum_{t \in \hat \calB}\hat b_t \hat \Pi_1(t).} \\
    & = \frac{\sum_{t \in \hat \calB}\hat b_t \Pi_1(t)}{\sum_{t \in \hat \calB}\hat \Pi_1(t)} \mu_1 + \frac{\sum_{t \in \hat \calB}\left(\hat b_t \Pi_2(t) + \hat b_t \xi_{t, q_t}\right)}{\sum_{t \in \hat \calB}\hat b_t \hat \Pi_1(t)}. 
\end{align*}

We need the following building blocks. 

\mypara{Block 1. } With high probability $|\hat \calB\| = \Omega(1)$. {\color{blue} this needs to be verified.}

\mypara{Block 2. } This is from Lemma~\ref{lem:absdiff}
\begin{align*}
\sum_{t \leq n}\left|\hat \Pi_1(t) - \Pi_1(t) \right| \leq n \sqrt{\frac{\gamma d}{\ell}}\log d. 
\end{align*}

\mypara{Block 3. } This will be a lemma we write below. 
\begin{align*}
    \left|\sum_{t \in \hat \calB} \hat b_t \Pi_1(t) - \sum_{t \in \hat \calB}|\Pi_1(t)|\right| \leq c_0 n \log^5 d \sqrt{\frac{d}{\ell}}\gamma
\end{align*}

\mypara{Block 4. } This will also be another lemma that needs to be written. 
\begin{align*}
    \sum_{t \in \hat \calB}\hat b_t \Pi_2(t) + \hat b_t \xi_{t, q_t} = O(\sqrt{nd}). 
\end{align*}

\mypara{Block 5. } With constant probability, $|\Pi_1(t)| = \frac{c_0}{\log d}\sqrt{\frac{d}{\ell}}$. This is from 
Lemma~\ref{lem:anti}. 

\mypara{Block 6.} This is part of a lemma. We need to make it a stand-alone lemma. 
Recall that $\Delta^2(q_t) = \sum_{i \leq d}\Delta^2_{q_t, i}$. We have 

\begin{align*}
    \Pr\left[\left|\hat \Pi_1(t) - \Pi_1(t)\right|\geq \lambda_t \mid q_t\right] \leq \exp\left(-\frac{\lambda^2_t}{\frac{1}{\ell}\Delta^2(q_t) + \frac{\lambda_t}{2}}\right). 
\end{align*}

We shall assume that all the building blocks are correct and analyze our estimator. Then we will prove each of the building blocks. 

First, note that 
\begin{align*}
    & \|\sum_{t \in \hat \calB} \hat b_t \hat \Pi_1(t) - \sum_{t \in \hat \calB}\hat b_t \Pi_1(t)| \\
    \leq & \sum_{t \in \hat \calB}|\hat \Pi_1(t) - \Pi_1(t)| \\
    \leq & \sum_{t \leq n}|\hat \Pi_1(t) - \Pi_1(t)|\\
    \leq & n \sqrt{\frac{\gamma d}{\ell}} \log d. 
\end{align*}

Also, we can see that 
\begin{align*}
    \left|\sum_{t \in \hat \calB}\hat b_t \Pi_1(t) - \sum_{t \in \hat \calB}|\Pi_1(t)|\right| \leq c_0 n \log^5 d \sqrt{\frac{d}{\ell}}\gamma.
\end{align*}

This implies that with high probability. 
\begin{align*}
    \left|\sum_{t \in \hat \calB}\hat b_t \hat \Pi_1(t) - \sum_{t \in \hat \calB}|\Pi_1(t)|\right| = O\left(n \log^5 d \sqrt{\frac{d}{\ell}}\sqrt{\gamma}\right)
\end{align*}
Next, we building block 1, we have 
\begin{align*}
    \sum_{t \in \hat \calB}|\Pi_1(t)| = \Omega\left(\frac{n}{\log n}\sqrt{\frac{\ell}{d}}\right)
\end{align*}

Therefore, 
\begin{align*}
    \sum_{t \in \hat \calB}\hat b_t\Pi_1(t) = (1+\tau_1) \sum_{t \in \hat \calB}|\Pi_1(t)| & \mbox{where} |\tau_1| = O\left(\log^6 n \sqrt{\epsilon}\right) \\
    \sum_{t \in \hat \calB}\hat b_t \hat \Pi_1(t) = (1+\tau_2)\sum_{t \in \hat \calB}|\Pi_1(t)|, & \mbox{where} |\tau_2| = O\left(\log^6 n \sqrt{\epsilon}\right).
\end{align*}

This implies that 
\begin{align*}
\left|    \frac{\sum_{t \in \hat \calB}\hat b_t \Pi_1(t)}{\sum_{t \in \hat \calB}\hat b_t \hat \Pi_1(t)}-1\right|  = O(\tau_1). 
\end{align*}

Now we analyze the second term. Using {\color{blue}Building block 5 and 1}, we have $\sum_{t \in \hat \calB}\hat b_t \hat \Pi_1(t) = \Omega\left(\frac{n}{\log d}\sqrt{\frac{d}{\ell}}\right)$. Now using {\color{blue} Building block 4}, we have 
$\sum_{t \in\hat \calB}\left(\hat b_t \Pi_2(t) + \hat b_t \xi_{t, q_t}\right) = O(\sqrt{nd})$, which implies 
\begin{align*}
    \frac{\sum_{t \in \hat \calB}\left(\hat b_t\Pi_2(t) + \hat b_t \xi_{t, q_t}\right)}{\sum_{t \in \hat \calB}\hat b_t \hat \Pi_1(t)} = O\left(\log d\sqrt{\frac{\ell}{n}}\right)
\end{align*}

Therefore, we can see that 
\begin{align*}
    \hat \mu_1 = (1+O(\tau))\mu_1 + O\left(\log d \sqrt{\frac{\ell}{n}}\right), 
\end{align*}
where $\tau = \log^6 n \sqrt{\gamma}$. 

{\color{red} a lot of typos above; $\epsilon$ should be changed to $\gamma$.}

\myparab{Building blocks.}

\begin{lemma} {\color{blue} Using the notation above,}
\begin{align*}
    \sum_{t \in \hat \calB}\Pi_2(t) s_t  = \sum_{t \in \hat \calB} s_t \left(\sum_{k \notin \calL_{t, 1}}K_{q_t, k}\tilde g_1(\mx_{t, k} \mid \mx_{t, k} \notin \Omega_1)\right)  = O(\sqrt{n d}). 
\end{align*}
\end{lemma}
\begin{proof} Our key observation is taht conditioned on $t \in \hat \calB$ and $\mx_{t, k} \notin \Omega_1$, $\tilde g_1(\mx_{t, k})$'s are bounded independent zero-mean random variables. In addition, we can see that $|\hat \calB| = \Omega(n)$. Therefore, a standard Chernoff bound gives that $\sum_{t \in \hat \calB}s_t \Pi_2(t) = O(\sqrt{nd})$. 
\end{proof}
\begin{lemma} {\color{blue} Using the notations above}, we have 
\begin{align*}
    \left|\sum_{t \in \hat \calB} \hat b_t \Pi_1(t) - \sum_{t \in \hat \calB}|\Pi_1(t)|\right| \leq 2n \log^5 d \sqrt{\frac{d}{\ell}}\gamma
\end{align*}
\end{lemma}

\begin{proof}Let 
\begin{align*}
    s_t = \left\{
   \begin{array}{ll}
   1 & \mbox{ if } \Pi_1(t) > 0 \\
   -1 & \mbox{ otherwise.}
   \end{array}
    \right.
\end{align*}
{\color{blue} remember to move the definition of $s_t$ out. This is needed everywhere.}
We have 
\begin{align*}
    \left\|\sum_{t \in \hat \calB} \hat b_t \Pi_1(t) - \sum_{t \in \hat \calB}|\Pi_1(t)|\right\| \leq 2 \sum_{t \in \hat \calB} |\Pi_1(t) | I(\hat b_t \neq s_t). 
\end{align*}
Note that $I(\hat b_t \neq s_t)$'s are i.i.d. random variables for different $t$'s. We next compute 


\begin{align*}
    & \Pr[I(\hat b_t \neq s_t)] \\
    \leq & \Pr[s_t = -1 \wedge \hat b_t = 1] + \Pr[s_t = 1 \wedge \hat b_t = -1] \\
    = & \Pr\left[\Pi_1(t) < 0 \wedge \hat \Pi_1(t) > \frac{c_0}{\log d}\sqrt{\frac d {\ell}}\right] + \Pr\left[\Pi_1(t) > 0 \wedge \hat \Pi_1(t) < - \frac{c_0}{\log d}\sqrt{\frac d {\ell}}\right]\\
    \leq & \Pr\left[\left|\Pi_1(t) - \hat \Pi_1(t)\right| > \frac{c_0}{\log d}\sqrt{\frac d {\ell}}\right] \\
     \leq & \Pr\left[\left(|\Pi_1(t) - \hat \Pi_1(t)| > \log d \sqrt{\frac{\Delta^2(q_t)}{\ell}}\right)\vee \left(\log d \cdot \sqrt{\frac{\Delta^2(q_t)}{\ell}}\geq \sqrt{\frac{d}{\ell}}\frac{c_0}{\log d}\right) \right] \\
     \leq & \frac{1}{n^{10}} + \Pr\left[\log d \cdot\sqrt{\frac{\Delta^2(q_t)}{\ell}}\geq \sqrt{\frac{d}{\ell}}\frac{c_0}{\log d}\right]\quad \mbox{ (by Lemma BLOCK 6)} \\
  = & \Pr\left[(\log^4 d) \Delta^2(q_t) \geq d\right] + n^{-10} . 
\end{align*}
Note that $\E[\Delta^2(q_t)] = \gamma d$. By using a Markov inequality, we have 
\begin{equation}
    \Pr\left[\log^4 d \Delta^2(q_t) > d\right] \leq \gamma \log^4 d.
\end{equation}

Using the fact that $\hat b_t$ and $s_t$ are independent across $t$, we have with high probability that 

\begin{align*}
    \left|\sum_{t \in \hat \calB} \hat b_t \Pi_1(t) - \sum_{t \in \hat \calB}|\Pi_1(t)|\right| \leq 2n \log^5 d \sqrt{\frac{d}{\ell}}\gamma
\end{align*}

\end{proof}


{\color{blue} why I dont say $\Pi^{(i)}_2(t)$ is estimated through $K$?}


\myparab{Bounding the error from discretization.} 
The error coming from the discretization is $\sqrt{d}/\ell$. So the total error is in the order of $n \sqrt{d}/\ell$. The multiplicative error seems to be in the order of $\log d \sqrt{\epsilon} + 1/\sqrt{\ell}$. 
    



\mypara{Also sum over $i$?} We have used only 1 observation for each day. This is because our analysis critically rely on that different $\Pi^{(i)}_1(t)$ and $\Pi^{(i)}_2(t)$ are independent. But here $\Pi^{(i)}_2(t)$ are correlated (fix $t$ for different $i$). While we have not excluded the possibilities that more refined analysis would allow us to use different $i$'s in the same day (although unlikely), we observe that using multiple $i$'s is unlikely to improve sampling complexity. 

Observe that if the rank of $K$ were $r$, then observations from $r$ independent rows of $K$ suffices to reconstruct all other observations {\color{blue} elaboration is needed.} TeTherefore, while there are $d$ observations every day, the effective number of observations is close to the rank of $K$. On the other hand, the rank of $K$ is low (see {\color{blue} Lemma XX an XX}). Therefore, using multiple $i$'s is unlikely to improve the performance {\color{blue} ZZ: need to implement baselines. }

The above argument is based on the assumption that we do not have noise. We shall still explain why using multiple rows is useless in the presence of noises. 


 
\myparab{Explain why we need $q(t)$.} Our estimation guarantees that $\|\hat K - K \|_F^2$ is small. But it does not guarantee that the row-wise difference is also small, e.g., tehtwe do not have non-trivial bound on $\|\hat K_{i, :} - K_{i, :}\|^2$. Thus, we need to be careful in choosing the $i$ parameter for each sample we use. There are two natural ways to circumvent the problem: 

\begin{enumerate}
    \item ``Collapse'' all the observations within the same day. 
    \item Randomly sample one 
\end{enumerate}

{\color{blue} ZLiu 20200515 edits ends here.}


\myparab{Concentration based on variance.} 
We also need a concentration result parametrized by the variance of the random variable. 

\begin{theorem}Suppose that $X_i$ are independent random variables satisfying $X_i \leq M$ for $1 \leq i \leq n$. Let $X = \sum_{i = }^n X_i$ and $\|X\| = \sqrt{\sum_{i = 1}^n \E[X^2_i]}$. Then we have 
\begin{equation}
    \Pr[X \geq \E[X] + \lambda] \leq \exp\left(-\frac{\lambda^2}{2(\|X\|^2 + M \lambda /3}\right)
\end{equation}
\end{theorem}


{\color{blue} not sure whether this block is needed.}



\subsection{Generalization}
A major implication of our theoretical result is that it is indeed possible to decouple latent position estimations from learning  $g(\cdot)$. This section first describes 
how we integrate ``main stream'' algorithms with our latent space inference algorithms.   
{\color{blue} forgot to mention that we are also tuning the transition matrix.}

\subsubsection{Deep learning}
We may use a deep learning network to represent $g(\cdot)$ (see also Fig.~\ref{fig:MLP}). Our goal is to minimize the training error
\begin{equation}
    \sum_{t, i}\left(\my_{t, i} - \sum_{j \in [d]} \hat K_{i, j} g(\mx_{t, j})\right)^2, 
\end{equation}
where $g(\cdot)$ is represented by a deep learning model. Note that $\hat K$ is produced from PROCEDURENAME and the neural net cannot change it. We examine two models. 
We examine both multi-layer perceptron models CITE and recurrent neural nets~\cite{hochreiter1997long,nelson2017stock,gao2016stock,rather2015recurrent,zhang2017stock}.

We also consider a special case, in which $g(\mx_{t, j})$ is a linear function. We shall refer to these algorithms as {\color{red} LGN (ZLiu: why it is called LGN?)}. 

\myparab{Comparisons and messages.} Our algorithms does not introduce new techniques/tricks for training DL. We \emph{simplify} recent architectures based on stock embeddings by using our stand-alone provable procedures to learn stocks' latent positions {\color{red} add figure}. We shall see in Sec. XX that our simplified architecture have better performance and reduced running time compared to prior related algorithms. CITE. {\color{red} sufficient details?}

\begin{figure*}[h!]
\centering
\includegraphics[width= .65\linewidth]{figures/MLP.pdf} 
\caption{$g(\cdot)$ is MLP}
%See Proposition~\ref{prop:closeness} and Lemma~\ref{lem:tailmain}.}
\label{fig:MLP}
\end{figure*}

 
\subsubsection{Gradient boosting algorithms}
{\color{blue} introduce notations: $b$ is the total number of base learners.}
Boosting (specifically boosted regression tree) is another important category of ML applications that is widely used in practice. Here, we generalize boosting algorithms to our settings. Recall that in a typical boosting algorithm our forecast is in the form $\sum_{i \leq b}g_i(\mx)$, in which $g_i(\cdot)$ is produced from a weak learner such as trees. The functions $g_i(\cdot)$ are trained in a sequential manner by a boosting algorithm. The key idea is to use residualized return CITE A LOT to train the model $g_i(\cdot)$. A natural way of generalizing this idea to out setting is to set $\my_{t, i} = \sum_{j \in [d]} K_{i,j}g(\mx_{t, j})$, where 
$g(\mx_{t, j}) = g_1(\mx_{t, j}) + \dots + g_b(\mx_{t,j})$.  We also use boosting algorithms to sequentially produce $g_i(\cdot)$'s. {\color{red} See Fig. XXX.} 

A key difference between the boosting algorithm here and a standard boosting algorithm is that a signal $g(\mx_{t, i})$ from any stock $i$ can impact the forecast for all stocks (see {\color{blue} the bolded flow in Fig. X}). So any minor changes in $g_j(\mx_{t, i})$ (e.g., adding a new decision node in a tree) will impact the forecast of all stocks on day $t$. This also means estimating $\my_{t, i}$ requires $d (=3,000)$ times more features. The compute and memory cost will also be significantly larger. It remains unclear how algorithms for GBRT can be generalized to handle the scale of data we face. 

Another more pronounced issue is that the forest-based models are difficult to interpret. While models based on one or two decision trees can be interpreted, boosting algorithms usually produce hundreds of trees, making interpretation impossible. 

We propose a simple, yet surprisingly effective linear base learner. We use standard algorithmic frameworks to sequentially train the learners ({\color{blue} See Fig. X}) but we use a linear model, instead of a decision tree, to represent the base learner. Our base learner chooses three variables ($\mx_{t, i_1}, \mx_{t, i_2}, \mx_{t, i_3}$) and use these variables together with their interaction terms to fit a linear model, i.e., {\color{red} notation messed up here. Should be $(\mx_{t, i})_{j_1}$}

\begin{align*}
    g_j(\mx_{t, i}) = \beta_1 \mx_{t,i_1} + \beta_2 \mx_{t, i_2} + \beta_3 \mx_{t, i_3} + \beta_4 \mx_{t, i_1} \mx_{t, i_2} + \beta_5 \mx_{t, i_1}\mx_{t, i_3} + \beta_6 \mx_{t, i_2}\mx_{t, i_3}. 
\end{align*}

The fitting procedure simply finds the best $\{\beta_i\}_{i \leq 6}$ that fits the residual return. 



\begin{figure}
\begin{codebox}
\Procname{$\proc{Boosting-Algorithm}(\mY, \mX, \eta)$}
\li \Comment $\eta$ is the learning rate. 
\li  $\mY_{\Res} \gets \mY$. 
\li \For $j \gets 1$ \To $b$
\li \Do 
$g_i \gets \proc{Linear-Fit}(\mY_{\Res}, \mX)$.

\li For all $t, j$: $(\hat \mY)_{t, j} = \sum_{k \in [d]}K_{j,k}g_i\left((\mX)_{t, k}\right)$
\li $\mY_{\Res} = \mY_{\Res} - \eta \hat \mY$. 
 \End
\li \Return $\{g_i(\cdot)\}_{i \leq b}$
\end{codebox}

\begin{codebox}
\Procname{$\proc{Linear-Fit}(\mY, \mX)$}
\li Let $\mx_{t, i} \in \reals^k$.
\li Let $\mf_{t, j} \in \reals^d$. 
\li For all $i$: $(\mf_{t,j}) = \sum_{k \in [d]}K_{k, i}(\mx_{t, k})_j$. 
\li Let $r_j = \mathrm{corrcoef}(\mf_{t, j}, \my_y)$. 
\li Let $j_1, j_2, j_3$ be the indices with the largest $r_j$. 
\li $g(\cdot) = \arg \min_{\beta_1, \dots, \beta_6}\sum_{\substack{t \leq d \\ i \in [d]}}\left(\my_{t, i} - \sum_{j \in [d]}K_{i,j}\left(\beta_1 (\mx_{t, i})_{j_1} + \dots + \beta_6(\mx_{t, i})_{j_2}\cdot (\mx_{t, i})_{j_3})\right)\right)^2$
\li \Return $g(\cdot)$
\end{codebox}

\caption{Linear boosted algorithms. {\color{red} check the dimensions of $\mX$ and $\mY$}}
\end{figure}

We next describe our learning algorithm 
and explains why our algorithm can substitute tree base learners. 

\mypara{1. Our learning procedure.} We choose the three variables that have the best explanatory power (after interacting with neighbors). See Line 4-5 in $\proc{Linear-Fit}$. Then we add interaction terms to the linear model. 

\mypara{2. Why linear model works.} It works for four reasons: \emph{(i)} Shallow trees (those with depth 3 or smaller) suffices for equity models. But when the trees' depth is only 2 or 3, the model can only extract interactions between 2 and 3 features. \emph{(ii)} Interaction terms are economically meaningful. The features we construct are economically meaningful so most interactions are still meaningful. We observe that direct interactions (e.g., $(\mx_{t, i})_{j_1}(\mx_{t, i})_{j_2}$) suffice to approximate the interactions produced from trees. \emph{(iii)} Approximate the greedy decision: trees are learned by using a greedy heuristics (i.e., to determine the splitting node, the algorithm seeks to find the splitting variables that maximizes the reduction in $r^2$. Here, our decision rule also has this greedy fashion, i.e., we choose the variables by only considering their first-order forecasting power. \emph{(iv)} Our linear model significantly speeds up {\color{blue} xxxxx}. 

{\color{blue} mention somewhere that our generalization can handle high-dimensional features.}

{\color{red} there are some indexing/notational issues above.}


\subsection{Robust latent estimation.}
mention static and dynamic models. 

{\color{red} to be moved around.}
\myparab{Barra Equity Model.}
Recall that we aim to construct $K^{(1)}$ from Barra China Equity Model (hereafter, Barra model)~\cite{orr2012supplementary}. 
The model uses 10 real valued factors and 1 categorical variable  to characterize a stock. The real valued factors include beta, momentum, size, earnings yield, residual volatility, growth, book-to-price, leverage, liquidity, and non-linear size. The categorical variable represents which industrial sector the stock is in. Roughly speaking, Barra factor model asserts that when two stocks have similar Barra factors, their behaviors are highly correlated. {\color{blue} need an extended version to discuss Barra factors.} 
See {\color{red} Table XX} for a description of the statistics. We use the real valued factors (also referred to as ``firm-level characteristics'') to construct $K^{(1)}$. We do not use sector information. 

Specifically, we let $F_{t, i} \in \reals^{10}$ be the factor exposure of the $i$-th stock on day $t$. We may construct $K^{(1)}_t$ using two standard methods. 

\begin{itemize}
    \item \emph{Inner product.} $(K^{(1)}_t)_{i,j} = \langle F_{t, i}, F_{t, j}\rangle$. 
    \item \emph{Distance.} $(K^{(1)}_t)_{i,j} = \exp(- \lambda |F_{t, i} - F_{t, j}|^2)$. {\color{blue} ZLiu: check the statement is correct. }
\end{itemize}

{\color{blue} some notational issues: $K^{(1)}_t$ refers to the first piece of distance matrix at time $t$. }

{\color{blue} Qiong, please check the correctness of the statement.}

{\color{red} todo: build a table to explain the factors. Also, check again whether we use $K^{(1)}_t$ or $K^{(1)}$.}

\myparab{News Data.} 
We observe also that when two or more stocks are mentioned in the same piece of news, they are more likely to be related /similar. Thus, we may build our second hint matrix $\mK_2$ as the occurrance matrix in the news dataset. Specifically, {\color{blue} describe how we construct the news.} Note here, our way to use news dataset deviates from standard news-based models for predicting stocks CITE. Most news-based models aim to  extract sentiments and events that could directly impact one or more related stocks' price. Here, we do not attempt to build links between events and fluctuation of stocks. Instead, we use news datasets to identify similarities between stocks, when two stocks are co-mentioned often, they are more likely to be similar. This is orthogonal to how the news itself impact the movements of stock prices. {\color{blue} Maybe some massage; text glued from different versions. }

We construct $K^{(2)}_t$ from news and $K^{(2)}_t$ consists of two steps. First, we construct $\tilde K^{(2)}_t \in \reals^{d \times d}$ such that  $(\tilde K^{(2)}_t)_{i,j}$ represents the number of news articles that mention both stock $i$ and stock $j$ between day $t - 59$ and day $t$ (i.e., we maintain a sliding window of 60 days). We then construct $K^{(2)}_t$ by taking a moving average of $\tilde K^{(2)}_t$ with a half-life being a hyper-parameter to be tuned. 

Our news are from a major Chinese news portal Sina. Specifically, we crawled all the financial news between 2013 and 2018 from Sina. We have collected a total number of 2.6 million articles. Each article can mention one or multiple stocks.  {\color{red} todo: some basic statistics of the news; like average number of news every day; every number of stocks that are mentioned by news every day?} 

The timestamps of news published online are usually unreliable (the dates are reliable but the hour or minute information is usually inaccurate). We use news signal on the next trading day or later to avoid looking ahead issues.

{\color{blue} question for Qiong: did we check that $K^{(2)}_t$ is a distance matrix? Other questions ZLiu asked in wechat: \emph{(i)} What is the half-life of the EMA? Any justification of using this half-life? \emph{(ii)} did we do anything to normalize $K^{(2)}_t$?  \emph{(iii)} Why do we do moving average (sliding window) and then EMA again? Can we just do one? }

\myparab{Construction of $K_t$.} Recall that we shall let $K_t$ be constructed from $K^{(1)}_t$ (produced from Barra data) and $K^{(2)}$. We shall examine the following consolidation algorithm. 

\mypara{Faithful implementation of {\color{blue} Algorithm XX.}} We first produce a faithful implementation of our algorithm discussed in Sec. XXX. {\color{red} I highly doubt whether this is a faithful implementation.} Specifically, we shall let $K_t = \exp(\beta K^{(1)}_t + (1-\beta) K^{(2)}_t)$. 

\mypara{Additional heuristics.} We may employ additional heuristics to tune $\beta$, including 
\begin{enumerate}
    \item Fine-tuning with deep learning blackbox. As discussed in the forthcoming sections, we shall use deep learning to learn the function $g(\cdot)$. When we use deep learning
    %We may continue to update the $\beta$ parameter 
    \item Hard-thresholding: for each row, we shall keep the $k$ largest entries. This is equivalent to assuming that the price of stock $i$ is only impacted by its $k$ nearest neighbors. 
    \item Row-wise normalization: we can also re-normalize $K$ so that each row sums to $1$. 
\end{enumerate}

{\color{blue} These are the questions for Qiong:
\begin{itemize}
    \item Q1. Is the matrix for news positive definite?
    \item Q2. Why exponentiation is needed? 
    \item Q3. Why there is no hyperparameter in the exponentiation. 
    \item Q4. Why do we set a hard threshold on number of neighors to use. 
    \item Q5. Why do we want a normalization (so that the sum of weights is 1).
    \item Q6. why dont we exponentiate barra matrix and news matrix and then do the linear combination later? 
    \item Q7. your model probably implies any stocks are positively correlated. 
    \item Q8. after you take exponentiation, your matrix is not even symmetric (and not positive definite)?
    \item Q9. can we still have the notion of latent position? In the original model, we assume $K_{i,j} = f(|\mz_i - \mz_j|)$, where $f(\cdot)$ is a radial basis function. If we use Qiong's algorithm, can we still have latent positions?
    \item Q10. if we do not use deep learning, we will fix $\beta$ and not update it? 
\end{itemize}

}




==> cover_letter.tex <==

\section{Cover letter}

The title is 
\subsection{The main reasons for rejection}

\subsection{Changes to addresses the reviews' comments}



\newpage
\qq{add the citations and clear the typos}


\section{Reviews and responses from AAAI 2021(weak reject, accept, weak accept)}

\myparab{R1.1} \textit{UNCONVINCING EXPERIMENTS:  1) short test period, 2) not include a full economic cycle, and 3) only using Chinese Market. }

Economic cycles have a substantial impact only on very low frequency models (multiple months of forecasting horizon) and unhedged/raw returns [1,2]. Here, we examine mid-frequency market neutral return (next 5 days) so these strategies are robust against long term economic cycles. * In other words, we assess the strength of our forecasts only against the idiosyncratic future return of each stock, and are completely agnostic to overall movements of the market; this is an important aspect to stress and we should make this clear from the outset. Furthermore, the t-statistics we report provide strong evidence for the statistical significance of our forecasts, for the 3-year period considered. 
Compared to state-of-the-art works ([3] 10 months, [4] 9 months, [5] one year) which employ testing periods of at most one year in a single market, our experimental setup has significantly extended the testing period to three years. App.G  discussed reasons for using Chinese data. We thank the reviewer for the suggestion; we will pursue the examination of multiple markets in upcoming future work.


\myparab{R1.2} \textit{2. PRESENTATION: $n$ in Line 197, $s$ in Line 254 (can a single number contain so much information?).}

Thank you for pointing this out. $n$ is the number of observations (Line 281 $\&$ 295), and will move the definition forward. $s$ is the latent/unobserved signal defined in the Line 254 $\&$ 271 and indeed should “contain much information” under our model definition. One of the goals of our algorithm is to recover an effective $s_{t,i}$ of $s_i$’s that have strong predictive power (See details on Sec.2)

\myparab{R1.3} \textit{FEATURES IN [-1,1]?}

Standard normalization and winsorization are used for each feature and fit the range into [-1,1].

\myparab{R1.4} \textit{INTERPRETATION OF THE PROPOSED LINEAR MODEL.}

Thank you for the suggestion. We presented our effort for interpreting the proposed linear model in App. F (specifically Table 7 $\&$ 8), and will move forward a portion of the discussion to the main paper.

\myparab{R1.5}  \textit{ILLUSTRATE HEAT MAP OF LEARNED $K_{i,j}$.}

We have included a t-SNE visualization of $K$ in Fig.13 in App.F.7. Thank you for the good suggestion. In addition to the t-SNE, we will surely add an illustrative heatmap.

\myparab{R1.6}.  \textit{THOUSAND COMMA INCONSISTENCY}

Thank you for pointing this out, and we have fixed it.

\myparab{R1.7}. \textit{FALSE POSITIVE OF PREVIOUS MODELS}

Confirming the (in)efficacy of existing approaches is a major contribution. We extensively tested our hypothesis in the experiments and also provided source code for replication purposes. 
A major reason for their inefficacy is the curse of dimensionality, e.g., the number of interactions to be estimated is significantly larger than the number of observations (see also Line 59-85, 135-137, and 224 - 227 for detailed discussions).

\myparab{R1.8}. \textit{ASSUMPTION ON LINE 132.}

The model assumptions are explained in Sec. 2 (Line 267-282). App. A also discusses why the assumptions are reasonable/mild.

\myparab{R1.9}. \textit{ABLATION STUDY (LINE 156)}
The boosting algorithm consists of two components: (a) change the original tree learners to linear learners, (b) use neighbor information.
We examined the impacts of removing one or two components in Table 2: (i) removing both (a) $\&$ (b): this reduces to the standard GBRT, which is one of the baselines. (ii) removing only (b): this is another baseline named poor man Lin-PVEL. 


\myparab{R1.10 } \textit{CITATIONS $\&$ DISCUSSIONS}

See the discussion in Line 1190-1192 for Jegadeesh and Titman 1993, and Fama and French 1996. Line 793 and 794 for Ming et al. 2014; Line 76-77 for Wu et al 2019. Thanks for the suggestion, we will add more discussion about these citations.

\myparab{R1.11}  \textit{ADD CITATIONS ON LINE 46 $\&$ 59}

For prior UMs and CAMs, we discuss more citations in the related work paragraph (Line 214-239).

\myparab{R1.12} \textit{ADD CITATION ON LINE 72 (citations use embedding $\&$ how to use the embeddings?)}
Thank you for the suggestion, citations that use embedding appear in 138-140 and will be moved forward. How embeddings are used are discussed in Line 1120-1125 in the App. F.4.


\myparab{R5.1} \textit{SURVEY $\&$ INNOVATION (REASON TO REJECT)}

Our proposed methods (e.g., how high-dim/kernel methods, boosting, non-parametric, and deep learning should be integrated/interacted under our proposed “decoupling principle”) have substantial differences compared to existing works. 
We are conscious that our paper combines a wide range of ingredients which could give the appearance of a survey (for this reason, we aimed at deferring background material to the appendix). We also believe that our comprehensive experimental setup and comparison with different methods also contributes to this impression; however, as illustrated by results in Table 2, our proposed pipeline significantly outperforms existing methods (3 new state-of-the-art very recent CAM models and 8 other baselines) across each of the four metrics considered (for two stock universes), over a period of time which is three times bigger than any of the current state-of-the-art methods used in their respective experiments.  
We will improve the paper structure to highlight these technical contributions in the final version.


\myparab{R5.2} \textit{MODEL AVERAGING, UNBALANCED DATA OR THOSE THAT HAVE CONFOUNDERS.}

We thank the reviewer for the insightful comment. Standard methods are used to average the models and process data. For example, we use a t-statistics based method (App.D.3) to average the models (effectively resembles Bayesian averaging). Investigation of more elaborated averaging/data processing schemes (e.g., leveraging correlations between different models’ forecasts) is indeed an important future work. We remark that the simple averaging scheme we used already leads to a consolidated forecast that outperforms each individual one, thus making the point we wanted to convey.

\myparab{R5.3}. \textit{LEARNED EMBEDDING, PCA VISUALIZATION, GBRT PICK UP METRICS. }

App. F.7 presents a qualitative examination of our embedding model, including a t-SNE visualization (similar to PCA visualization). We observe that the boosting algorithm with learned embedding delivers a stronger forecast compared to the original one (approx. 10% improvement shown in Table 2), which is a sign that it picks up the metrics. We will add a table explaining how the feature importance changes after using the learned embedding. 

\myparab{R5.4}. \textit{TEXT/ESG SIGNALS/SOCIAL IMPACT FOR LINE 38-40.}

Thank you for pointing this out. Price dependent features (Line 38-40) are used only as an example and will be clarified in the final version. App. G gives an overview of models using different features (including text etc) and explains why this work focuses on technical features. 

\myparab{R5.5}.\textit{ HYPOTHESIS TESTING, BAYESIAN INTERPRETATION FOR LASSO.}

Thanks for the reminder. We will add a discussion on how lasso-based hypothesis testing can be used in equity market forecasting [6].

\myparab{R5.6}. ADD REF. TO LINE 145-160 (e.g., empirical asset pricing via machine learning, or 
can machine learn finance.)

We will add the suggested refs in Line 145-160. Empirical pricing was cited elsewhere (Line 217). 

\iffalse
[1] De Prado, M. L. Advances in financial machine learning. 2018.
[2] Zhou, X., & Jain, S.  Active Equity Management.  2014.
[3] Hu, Z., Liu, W., Bian, J., Liu, X., & Liu, T. Y. Listening to chaotic whispers: A deep learning framework for news-oriented stock trend prediction. WSDM. 2018.
[4] Li, Z., Yang, D., Zhao, L., Bian, J., Qin, T., & Liu, T. Y.  Individualized indicator for all: Stock-wise technical indicator optimization with stock embedding. KDD. 2019.
[5] Zhang, L., Aggarwal, C., & Qi, G. J. Stock price prediction via discovering multi-frequency trading patterns. KDD. 2017.
[6] Javanmard, A., & Montanari, A. Confidence intervals and hypothesis testing for high-dimensional regression. JMLR, 2014
\fi

 
 
 
 

 
 
 
 


\section{Reviews from NeurlIPS 2020}

\myparab{Review 1; a reject}

There are a few assumptions/claims in the model and theory that I find unnatural:

1. The main part of the stock return forecast is essentially a kernel weighted sum of signals from neighboring stocks. For Gaussian or inverse multi-quadratic kernels (as assumed in the theory), the kernel weight is always positive. Therefore, the contribution of a stock, $s_{t, j}$, has to be of the same sign to all other stocks. I find this property unrealistic, since in reality, for example, a stock's return can positively impact the return of one stock and negatively impact that of another.


2. The theory assumes that $s_{t, j}'s$ and $\xi_{t, i}$' are both iid. According to Equation (1), this makes the returns stock returns $y_{t, i}$ iid across both t and i (if I understand correctly, K is non-random). For daily stock returns (as is used in the trading simulation), this is unrealistic.

3. Line 136: could the authors elaborate on why $E^T E / n$ is asymptotically smaller than $K^2$?

4. The paper claims embedding stocks in a low-dimensional latent space as a main advantage of the proposed methodology. However, the methodology doesn't actually estimate any embeddings. Only a kernel matrix between the latent positions is used. It's unclear how the latent positions compare in dimension to the observed features.

5. Regarding the experiments, I find the comparison between the proposed methods and ones without neighbors ("w/o" in Table 1) unfair. If I understand correctly, the "w/o" methods directly estimates the stock return by the g function. According to the definition of g (Line 110), it only has access to the information of the self stock. It's entirely possible that these ML models could outperform the neighbor-based method if allowed to exploit cross-sectional information.


\textbf{Writing}
The intuition behind the proposed algorithms is well explained. On the other hand, I find the main paper less self- contained. Many details necessary for understanding the work is put in the supplementary materials (e.g., distributional assumptions, forecasting and trading simulation setup, factor definitions, definitions of the various models compared in the experiment). The experimental results could also be strengthened by providing more interpretations. For example, in Section 4.4, while the latent positions are not driven by sectors, what relations between the stocks do the clusters capture?

\iffalse
\textbf{typos}

Typos and minor comments:
- Line 69: "$||x - z||$" should be "$||x - x'||$".

- Line 151: remove subscript "$F$".

- Line 183: missing "$y_{t, i}$" in the numerator. 

- The font size in Table 4 is too small.
\fi


\myparab{Reviewer 2, weak accept}
I'm in general skeptical to papers related to financial market predictions due to the fact that there are no standard benchmarks and the empirical results can be manipulated on a fixed limited data set (only daily price / volume in a few years are pretty small). So my comments on weaknesses are also in the evaluation.

1. The author need to change the title to a very precise description of the techniques because embeddings are too broad. The content in this paper is definitely not covering all these topics. For example, BERT on financial news can generate embedding.


2. The evaluation on Chinese market is not convincing to me. Limit the claims of the algorithms to Chinese markets. - "Using the US market is not a better option for comparison purpose". Using the US market is definitely a better option because US market has longer history and is a more competing market. Also the no-same-day-sell rule makes huge difference. Half of the previous research not using it is a a reason that we should not make the evaluation better and more convincing.
- "there is no evidence that an effective strategy in one market is not effective in the other market". This is not true. An effective high frequency strategy in US market won't even work in the Chinese market because you cannot receive price update at millisecond level and the rules forbid you to trade so frequently.
And the best way to verify this is to simply evaluate both and show readers the conclusion. This conclusion would be very valuable.


3. When choose 5-day return as label, what if the price is positive on the 5th day but it drops significantly on the 3rd day and the position has to be cleared due to stop-loss setup? Is it still good to treat it as positive label? My point is that the label needs to consider the trajectory of price movement.


4. What about survival bias?

5. Only TA features are used. Would it change conclusions if fundamental features are
included?

6. The evaluation time window is not long enough to show the algorithm is still working in abnormal environments.

7. It uses "the efficient market hypothesis" on line 117 to defend an assumption. By EMH, my understanding is that all information has been included in current market and the current price is fair. Then without new information coming in, how can you predict the return in future?
I am totally fine if the author just claim that EMH is wrong. Don't use it to defend a work predicting returns.


\myparab{Reviewer 3 reject}

1. I did not see much technical contribution in this paper. They employ kernel learning/neural network for stock embedding/prediction. The techniques they are employing seem to be very standard and lack novelty. The decoupling of latent position learning and link function also looks straightforward.

2. The writing of paper could be improved. I found the current presentation of this paper a bit hard to follow.

3. Something that needs more explanation: why restrict $s_{t,i}$ to {-1, 1} instead of real values (as in most embedding methods).


\myparab{Reviewer 4, weak reject}

1. In this paper, the authors proposed to use $f(g(x_t))$ to predict $y_t$ where $f$ is a nonlinear function. The authors assume that $\{x_t\}$ is given. Then y can be estimated by many statistic models, such as semi-parametric single index models. The paper lacks comparison with existing works that use $f(g(x))$ format to predict $y$, where f is nonlinear and g is a smooth function with constrains.


2. Also, for time series, a more realistic assumption is that $y_t = f_1(x_t) + f_2(y_{t-1})$ where the previous stock return also affects the current stock return. This time dependency is what makes high-dimensional time series become interesting. Without this time dependency, the theory and algorithms have no difference with predicting $\{y_i\}_{i=1}^n $ based on $\{x_i\}_{i=1}^n$ under the iid assumption.




==> exp_nips.tex <==


\section{Evaluation}\label{evluation}



%{\color{red} please give a pointer to the appendix.}

\myparab{Experimental setup.}
We use 10 years of equity data from the Chinese market to evaluate our algorithms and focus on predicting the next 5-day returns, in which the last three years are out-of-sample. The test period is substantially longer than those in recent works~\cite{zhang2017stock,hu2018listening,li2019individualized}.   
We constructed 337 standard technical factors to serve as a feature database for all models (App.~\ref{sec:fac}). 
%We exclusively use technical factors in App.~\ref{sec:fac} as features. 
We consider two universes: (i) \emph{Universe 800} can be construed as an equivalence to the S$\&$P 500 in the US, and consists of 800 stocks, and (ii) \emph{Full universe} consists of all stocks except for the very illiquid ones.  Visualizations are shown in App.~\ref{performance}.

% The average ``size'' (in either market capital or trading volume) in \emph{Universe 800} is larger than the average size of the \emph{Full universe}. Synthetic data studies are also presented in App.~\ref{sec:synthetic}. Synthetic data studies and



We next explain our metrics and argue why they are different from those for standard ML problems (see App.~\ref{robustevaluation}) 
% 
$\bullet$ \emph{(i) Correlation vs MSE.} While the MSE is a standard metric for regression problems, correlations are better suited  metrics for our setting~\cite{zhou2014active}. %
% 
$\bullet$~\emph{(ii) Significance testing.} 
The use of  $t$-statistics estimators~\cite{newey1986simple} can account for the serial and cross-sectional correlations (App.~\ref{robustevaluation})
%
$\bullet$~\emph{(iii) Stock capacity/liquidity considerations.}  Predicting illiquid stocks is less valuable compared to predicting liquid ones because they cannot be used to build large portfolios. We use a standard approach to weight correlations (w\_corr) and $t$-statistics by a function of historical \textit{notional (dollar) traded volume} to reflect the capacity of the signals. 
%$\bullet$~\emph{(iii) Latent position visualization.} We visualize our learned latent positions in App.~\ref{visualization} \qq{not sure where we mention the visualization.}

%Uniform evaluation platforms are unavailable to the academic community, and thus it has been impossible to perform a fair comparison among equity forecast models. To this end, we open source our evaluation framework together with important baselines. 
%{\color{blue} Qiong: please move that to appendix and add details, e.g., Felix' bootstrapping algorithm.}


%We tackle this community-wide problem by \emph{(i)} explain how a signal should be rigorously tested, which is different from other standard ML problems, \emph{(ii)} open source our testing framework, and \emph{(iii)} replicate recent works CITE so that the community can use/study them. 


%\vspace{-0.6cm}

\vspace{-1mm}
\myparab{New CAMs from our model.}
We estimate $K$ and $g(\cdot)$ separately. To estimate $K$, we use both the algorithm discussed in Sec.~\ref{k_est} and other refinements discussed in App.~\ref{add_K}. To estimate $g(\cdot)$, we use SGD-based algorithms (MLP, LSTM, and linear), nparam-gEST, and \Linpvel. 
%See Fig.~\ref{fig:compare} for the comparison.

%We follow the decoupling principle and effectively decompose the problem into two parts: $K$ estimation and $g$ estimation.  In the $K$ estimation, Opt.denotes the optimal results where the $K$ is estimated by mathematical sound Alg.~\ref{fig:estimatek}. Moreover, we also examine other data-driven ways (DD) to construct $K$. See App.~\ref{construct_K} for more details. In the $g$ estimation, we implement the non-parametric learning method ($g$-EST), algorithms based on stochastic gradient descent (MLP, LSTM), Lin-PVEL in projected vector ensemble learning, and linear model(including ridge and lasso).

\vspace{-1mm}
\myparab{Baselines.} 
%{\color{red} please move around the text so that it is consistent with earlier part of the paper.} 
\emph{(i) The UMs} include linear, MLP, LSTM, GBRT, and SFM~\cite{zhang2017stock}. We also implement a ``poor man's version'' of both {\Linpvel} and nparam-gEST for UM, which assumes that influences from other stocks are 0;   \emph{(ii) The CAMs} include a standard linear VAR ~\cite{negahban2011estimation}, ARRR~\cite{wu2019adaptive}, AlphaStock~\cite{wang2019alphastock}, and HAN~\cite{hu2018listening}. 

\vspace{-1mm}

\myparab{Results.} See Table~\ref{main_table} for the results and Fig.~\ref{fig:fret_quantiles} for the simulated Profit \& Loss (PnL). App.~\ref{sec:app_exp} describes additional details and experiments. The experiments confirm that \mbox{\bb \emph{(i)} generic} ML techniques are effective for UMs but ineffective for CAMs;  \bb \emph{(ii)} CAMs produced out of our model consistently outperform prior works. In addition, our {\Linpvel} model has the best performance;  \bb \emph{(iii)} By using a simple consolidation algorithm, the aggregated signal outperforms all individual ones. Our new models pick up signals that are orthogonal to existing ones because we rely on a new mechanism to use stock and feature interactions. 
\vspace{-2mm}
\begin{figure}[ht!]
% \captionsetup[subfigure]{aboveskip=-4pt,belowskip=-1pt}
\centering
\includegraphics[width=0.48\textwidth]{figures/main_pnl.pdf}
\vspace{-2mm}
\captionsetup{width=1.0\linewidth}
\captionsetup{font=small}
\caption{Cumulative PnL (Profit and Loss) curves of the top quintile portfolio from \textit{Full universe} (i.e., on any given day, we consider a portfolio with only the top 20\% strongest predictions in magnitude, against future \textit{market excess returns}). See App.~\ref{performance}} %for more results.}
\vspace{-5mm}
\label{fig:fret_quantiles} 
\end{figure}
\vspace{-1mm}
%\qq{It % latter aspect
%confirms the value of building multiple CAMs (App.~\ref{sec:consolidateapp}) and \red{aggregating their forecasts} is crucial for portfolio managers.} 

%AlphaStock cannot return profits since 2010, which is consistent with our experiments.
%\myparab{Discussion about prior evaluations.} SFM (\cite{zhang2017stock}) is open-sourced, and other studies reported  similar performance of SFM. SFM, HAN, and AlphaStock did not compute $t$-statistics. HAN's PnL is positive, but its signal is not significant. AlphaStock cannot beat the market and  generates negative PnL returns since 2010. 
%stopped returning profits since 2010
%stopped returning profits since 2010. 


\iffalse
{\color{red} please provide an explanation. please be extremely careful in explaining opt and dd (need to connect back to the decoupling principle section). then please re-format the table: first UMs, then existing CAMs, then our CAMs. Then highlight existing CAMs are all worse than UMs; Ours are all better than existing CAMs. Ours are better than most UMs except for the boosting. }

%\myparab{Then re-write observations. we do not need to have with neighbor without neighbor for this version. }

% {\color{red} please add pointers when you find suitable.}

\hspace{-2mm}  
\bb  \emph{(i)~Linear (including Ridge \& LASSO)}. We build a linear model and train the model using all the stock data. 
% 
\bb \emph{(ii)~Deep~learning.} We use the entire stock data to train a model
$\my_{t, i} = g(\mx_{t, i}) + \xi_{t,i}$, 
where $g(\cdot)$ is a  non-linear function represented by MLP or LSTM. 
%
\bb  \emph{(iii)}~Vector~regression (\textsc{VR}). We use the model $\my_t = M \mx_t + \xi_t$, where $\my_t$ is a vector of returns and $\mx_t$ a vector of past returns. We use nuclear norm~\cite{negahban2011estimation} as regularizer.
% 
\bb \emph{(iv) \textsc{SFM}~\cite{zhang2017stock}}. \textsc{SFM} decomposes the hidden states of an LSTM network into multiple frequencies by using Discrete Fourier Transform (DFT) such that the model captures signals at different horizons. SFM is open sourced and other studies reported similar performance of SFM~\cite{chen2019investment}; 
% 
\bb \emph{(v)~HAN~\cite{hu2018listening}.} This work introduces a so-called hybrid attention technique that translates news into signals. The key statistics between our replication and HAN (reported in their papers) are consistent.
%
\bb \emph{(vi)~ \textsc{AlphaStock}~\cite{wang2019alphastock}.} \textsc{AlphaStock} uses deep learning to uncover the latent positions of the stocks, and then leverages them to produce forecasts. We remove its reinforcement learning component (which translates signals into positions) and keep only the components that produce return forecasts. %{\color{red} do we still have vector linear?}
\textsc{AlphaStock} cannot beat the market (generate negative return) since 2010, which is consistent with our experiments;

%\myparab{Vector linear regression.} We use the model $\my_t = M \mx_t + \xi_t$, where $\my_t \in\reals^d$ is a vector of returns and $\mx$ is a vector of features. $M$ is a learnable matrix and we use nuclear norm to regulate $M$ CITE. 


\subsection{Forecasting performance}
\vspace{-1mm}
Table~\ref{main_table} shows the performance of all the algorithms. Fig.~\ref{fig:fret_quantiles} shows the cumulative PnL (Profit \& Loss) under three simulations, including  ``Long-index portfolio'', ``Long-short portfolio'', and ``Weighted-Long-short portfolio.'' See  App.~\ref{performance}. Note that shorting can be done in Chinese market under very restricted conditions (e.g., entering a customized deal with a broker in Hong Kong). 
%  
We make the following overall observations. 
%
\bb \hspace{-1mm} \emph{1. Improvement using neighbors.} We see a uniform improvement when a linear or ML model uses neighborhood information. This confirms that the neighbor-based method is a generic technique that can improve many existing ML models. 
% 
\bb  \emph{2. Efficacy of {\Linpvel}.} {\Linpvel} algorithm described in Section \ref{sec:generalization} attains the best performance,  confirming the efficacy of our heuristics. Note that \textbf{the best model} (Boosting Opt or DD) \textbf{is a linear model} (with interaction terms) that outperforms all the non-linear ones.   
%
\bb  \emph{3. Design of deep learning architecture.} Deep learning can be beneficial. For example, MLP+NN method is better than \textsc{FlipSign} and standard linear algorithms. However, over-engineered architectures, such as LSTM, \textsc{AlphaStock}~\cite{wang2019alphastock}, lead only to degraded performance. 
%
\bb   \emph{4. Consolidation/Ensemble aggregation.}  While comparing correlations and $t$-statistics guides our understanding of which individual model performs better, the more important overarching question, especially for practitioners, is to understand whether a new model has ``orthogonal'' prediction power compared to the other models. To this end, when we overlay a simple boosting algorithm over all the methods we examine, we produce a forecast that outperforms any single individual model on every performance metric (the last row of Table~\ref{main_table}). See App.~\ref{sec:consolidateapp}. %\MC{shall we refer to the correlation analysis in the appendix? (if we still plan on adding it)}
\fi

% \vspace{-2mm}

%\myparab{Remark on baselines.} While all recent ML results (SFM, \textsc{AlphaStock}, and HAN) do not seem to be competitive, \emph{(i)} SFM is open sourced and other studies reported similar performance of SFM~\cite{chen2019investment}; \emph{(ii)} \textsc{AlphaStock} cannot beat the market (generate negative return) since 2010, which is consistent with our experiments; and \emph{(iii)} the key statistics between our replication and HAN (reported in their papers) are consistent. %\qq{might be we should give some credit to SFM, since they are open-sourced. For SFM,  we used their original implementation.}
%{\color{red} add a sentence to link back the importance of the evaluation framework.}

%{\color{red}The signals used in HAN were not significant (low t-statistics) and could have been captured under our framework. TOO AGGRESSIVE?}\qq{might be too aggressive, their features are all from news and the other baselines use factors.}
%we remark that it is unlikely we had a wrong implementation. 


%Some of the neighbors found by us are quite impressive. 





%\myparab{Training and testing.} We use standard ``sliding window'' method to train and test our model {\color{red} See Appendix XX for details.}

\iffalse
\myparab{Prior works.}
\mypara{(i) Lack of significant tests.} A few works {\color{blue}XX} studies a testing period for one year or less and do not compute the significance level. 
\mypara{(ii) Look ahead.} When data from the testing set is leaked to training, a  look-ahead happens.   For example, 
\cite{zhang2017stock,mikolov2013fefficient} used testing data to normalize features and responses. 
\mypara{(ii) Labels.} Many prior works (from CS) {\color{blue} cite} casts the problem as a classification problem, which is less standard in empirical asset pricing CITE. Some works use prices as response. But price time series are not stationary. Predicting non-stationary process is remarkably challenging, if not inappropriate. 
\fi




==> experiment_setup.tex <==
\section{Experiment setup}
We use the Chinese stock market dataset that consists of approximately 3600 stocks between 2013 and 2018. We focus on predicting the \emph{next 5-day returns}.  We examine two  universes in this market: (i) \emph{Universe 1} is equivalent to S$\&$P 500 and consists of 800 stocks, and (ii) \emph{Full universe} consists of all stocks except for illiquid ones.

\subsection{Learning $D$ with hint from news and Barra datasets}
\myparab{Barra factor loading}
We use 10 classical barra factors including yield, earnings growth, volatility, liquidity, momentum, size, price-earnings ratio, leverage, and growth.
We collect the risk exposures on these factors for the full universe.
Assume $b_{i,t}$ and $b_{j,t}$ are the two exposure vectors for stock $s_i$ and $s_j$ on date $t$ and the exposure vectors dimension is 10.
We update the barra matrix in daily granularity. We use the dot product $d_{i,j,t} = b_{i,t}b_{j,t}^{\transpose}$ to measure the similarity between two stocks.  At date $t$, the barra similarity matrix is $M_{bar,t} \in \reals^{n\times n}$, where $n$ is the number of stocks. Then we use $d_{i,j,t}$ to construct the barra similarity matrix $M_{bar,t}$

\myparab{News loading}
We crawled all the financial news between 2013 and 2018 from a major Chinese news website Sina\footnote{https://finance.sina.com.cn}. It has a total number of 2.6 million articles. Each article can refer to one or multiple stocks. The timestamps of news published online are usually unreliable (the dates are reliable but the hour or minute information is usually inaccurate). We use news signal on the next trading day or later to avoid looking ahead issues.
Assume $M_{news,t} \in \reals^{n\times n}$ is the similarity matrix on date $t$ and $n$ is the number of stock.  Each entry in $M_{news,t}$ represents the number of training news articles that mention both $s_i$ and $s_j$ on date $t$. Since the news co-occurrence matrix is relatively sparse, we update the daily news co-occurrence matrix using exponential moving average. 

%We construct the daily co-occurrence matrix $M_{news,t} \in \reals^{n\times n}$ from our news dataset, where $n$ is the number of stocks and $t$ is the date. Each entry in $M_{news,t}$ represents the number of training news articles that mention both $s_i$ and $s_j$ on date $t$.
\qq{Do we mention the EMA on news? we need to explain why we use the EMA, too sparse}
\begin{equation}
M_{news,t} = \left\{\begin{matrix}
 M_{news,1} & t = 1\\ 
\alpha M_{news,t} + (1-\alpha)  M_{news,t-1} ) & t>1
\end{matrix}\right.
\end{equation}{}
where $\alpha = \frac{2}{1+w}$ and $w$ is the window size and $w$ is a hyper parameter. 

\myparab{Linear interpolation}
At date $t$, the similarity matrix $M_t$ is 
\begin{equation}
  M_t =  \beta M_{bar,t} + (1- \beta)M_{news,t}
\end{equation}{}
where $\beta$ is a learnable parameter.

\myparab{Dynamic kNN}
Motivated by the dynamic intrinsic stock properties, we use the daily similarity/distance matrix to reveal the stock current state based on their neighbors technical indicators. 
More formally, we compute the top-$k$ stocks for stock $s_i$ at time $t$.
\qq{Might be I should add a figure}

\qq{update in 0422, I remove the softmax functions, and use M directly}

\begin{equation}
  w_{i,j,t} =  \frac{exp(M_{i,j,t})}{\sum_1^k exp(M_{i,j,t})}
  \text{\qq{It looks like attention}}
\end{equation}{}


{\color{blue} These are the questions for Qiong:
\begin{itemize}
    \item Q1. Is the matrix for news positive definite?
    \item Q2. Why exponentiation is needed? 
    \item Q3. Why there is no hyperparameter in the exponentiation. 
    \item Q4. Why do we set a hard threshold on number of neighors to use. 
    \item Q5. Why do we want a normalization (so that the sum of weights is 1).
    \item Q6. why dont we exponentiate barra matrix and news matrix and then do the linear combination later? 
    \item Q7. your model probably implies any stocks are positively correlated. 
    \item Q8. after you take exponentiation, your matrix is not even symmetric (and not positive definite)?
    \item Q9. can we still have the notion of latent position? In the original model, we assume $K_{i,j} = f(|\mz_i - \mz_j|)$, where $f(\cdot)$ is a radial basis function. If we use Qiong's algorithm, can we still have latent positions?
    \item Q10. if we do not use deep learning, we will fix $\beta$ and not update it? (for the linear models, I will update the $\beta$ in the training phase)
\end{itemize} 
}

\myparab{Weight normalization}
We re-scale the neighbors factors by the $ w_{i,j,t}$ and use the weighted sum as the representation for neighbors.

\begin{equation}
  F_{i,t} = \sum_{j =1}^{k} M_{i,j,t} \cdot I_{j,t}
\end{equation}{}
where $I_{j,t}$ is the technical indicator for stock $j$ on date $t$.

\myparab{MLP}
A straight-forward way is to combine the representations of stock neighbors together with its own indicator with linear interpolation. Formally,

\begin{equation}
\begin{array}{l}
    \hat{y}_{i,t+1} = MLP( S_i) \\
    S_i = \theta F_{i,t} + (1- \theta) I_{i,t}
\end{array}
\end{equation}

where $\theta$ is a hyper-parameter and MLP represents the multilayer perceptron.


\qq{We also tried a direct concatenate for  $[F_{i,t} , I_{i,t}]$, but seems the linear equation works better}

\myparab{Sequence modeling}
In the MLP model, we made the assumption that the market state will be consistent in two consecutive days. It is natural to leverage the historical neighbor relationships and indicators to make the future stock forecast. LSTM is widely used in stock forecasting \qq{CITE} to capture the historical stock states and our forecast is 

\qq{Do we add the details of LSTM equations?}

\begin{equation}
     \hat{y}_{i,t+1} = LSTM(\overrightarrow{S_i}_{<t})
\end{equation}{}

%\input{knn_setup}




==> factor_universe.tex <==
\newpage
\section{Factor list}\label{sec:fac}

In this section, we provide a table to explain the technical factors we build. The last column shows the number of features for one factor category since we can build several factors for different time scales.

\setlength{\tabcolsep}{3mm}
\renewcommand{\arraystretch}{1.5}{
\begin{longtable}{p{0.6cm}p{2.5cm}p{7.5cm}p{2cm}}
\toprule
 Index &  Factor Name &                                                                                                                                                                                        Factor Description &  \# of Factors \\
\midrule
\endhead
\midrule
\multicolumn{4}{r}{{Continued on next page}} \\
\midrule
\endfoot

\bottomrule
\endlastfoot
 1 &  AD~\cite{colby1988encyclopedia} &  Accumulation/Distribution is a cumulative indicator that uses price and volume to assess whether an equity is cumulative or distributed. &  3 \\
 2 &  MACD~\cite{colby1988encyclopedia} &  Moving Average Convergence Divergence (MACD) is a trend-following momentum indicator that shows the relationship between two moving averages of an equity's price.  &  9 \\
 3 &  RSI~\cite{colby1988encyclopedia} &  Relative strength index is a momentum indicator to measure the magnitude of one equity's recent price changes. &  3 \\
 4 &  SRMI~\cite{colby1988encyclopedia} & Shifted relative momentum index. &  4 \\
 5 &  VRSI~\cite{colby1988encyclopedia} &  VRSI is an indicator similar to RSI, but it measures volume rather than price. &  5 \\
 6 &  Amihud~\cite{amihud2002illiquidity} &  Amihud illiquidity measure is mainly used to calculate the level of illiquidity of a stock. &  6 \\
 7 &  Volume Std &  Standard deviation of volume. &  2 \\
 8 &  CR  &  Cumulative return &  3 \\
 9 &  ER~\cite{colby1988encyclopedia} &  Elder-Ray indicator defines bull and bear power by 13 days exponential moving average of highest and lowest price. &  1 \\
 10 &  DDI~\cite{colby1988encyclopedia} &  The DDI indicator measures the relative relationship of one stock's highest and lowest prices. &  3 \\
 11 &  BBI~\cite{colby1988encyclopedia} &  BBI measures the difference between the moving averages of stock indices closing prices in different periods. &  3 \\
 12 &  EoM~\cite{colby1988encyclopedia} &  Exponential moving average of BBI indicator. &  2 \\
 13 &  KDJ~\cite{colby1988encyclopedia} &  KDJ indicator is a technical indicator used to analyze and predict changes in stock trends and price patterns in a traded asset.  &  3 \\
 14 &  Hurst~\cite{hurst1965long} &  The Hurst indicator is used to do chaotic fractal analysis for the capital market. It reflects the result of a long series of interconnected events. &  3 \\
 15 &  Klinger~\cite{colby1988encyclopedia} &  Klinger’s volume swing indicator determines the long-term capital flow trend while maintaining sensitivity to short-term capital flows, so it can be used to predict short-term price inflection points. &  2 \\
 16 &  LQ~\cite{fama1993common} &  An indicator to measure one equity's liquidity for a time period. &  8 \\
 17 &  MF~\cite{colby1988encyclopedia} &  Money flow. &  2 \\
 18 &  Close regression~\cite{colby1988encyclopedia} &  Linear regression on one equity’s close prices. &  2 \\
 19 &  High regression~\cite{colby1988encyclopedia} &  Linear regression on one stock’s highest prices. &  2 \\
 20 &  Low regression~\cite{colby1988encyclopedia} &  Linear regression on one stock’s lowest prices. &  2 \\
 21 &  Volume regression~\cite{colby1988encyclopedia} &  Linear regression on one stock’s trading volume. &  2 \\
 22 &  MFI~\cite{colby1988encyclopedia} &  The MFI indicator combines price and quantity and includes it in the scope of comprehensive consideration. &  6 \\
 23 &  ROC~\cite{colby1988encyclopedia} &  A momentum oscillator that measures the percent change in price from one period to the next. &  5 \\
 24 &  SRMI~\cite{colby1988encyclopedia} &  SRMI indicator revised momentum indicator based on the relation of closing prices of the day and the previous trading day. &  3 \\
 25 &  TEMA~\cite{colby1988encyclopedia} &  Triple exponential moving average on closing prices. &  3 \\
 26 &  TRIX~\cite{colby1988encyclopedia} &  Smoothed TEMA indicator. &  3 \\
 27 &  ULCER~\cite{colby1988encyclopedia} &  ULCER indicator measures the relationship between the highest price and closing price of a stock over a period of time. &  3 \\
 28 &  Volume Std~\cite{fama1993common} &  Standard deviation of trading volume over a period of time. &  3 \\
 29 &  Price Std~\cite{fama1993common} &  Standard deviation of closing prices over a period of time. &  3 \\
 30 &  Volume Mean~\cite{fama1993common} &  Average of trading volume over a period of time. &  3 \\
 31 &  Price Mean~\cite{fama1993common} &  Average of closing prices over a period of time. &  3 \\
 32 &  ASI~\cite{colby1988encyclopedia} &  The cumulative volatility index uses the stock's opening price, closing price, highest price, and lowest price to measure long-term trends. &  3 \\
 33 &  EMV~\cite{colby1988encyclopedia} &  Ease of Movement is an oscillator to measure the ‘ease’ of stock moving. &  3 \\
 34 &  ATR~\cite{colby1988encyclopedia} &  The Average True Range is the average of the price range over the past n periods. &  3 \\
 35 &  CO~\cite{colby1988encyclopedia} &  The CO indicator measures the difference between the index moving averages of stock AD indicators in different periods. &  1 \\
 36 &  CV~\cite{colby1988encyclopedia} &  CV measures the difference between the exponential moving averages of stock price ranges in different periods. &  1 \\
 37 &  CMO~\cite{colby1988encyclopedia} &  The Chande momentum oscillator is a price volume oscillator which is closely related to RSI indicator. &  2 \\
 38 &  Ccurve~\cite{colby1988encyclopedia} &  Exponential moving average of past 7 and 14days’ return. &  1 \\
 39 &  DMI~\cite{colby1988encyclopedia} &  The DMI indicator provides a basis for judging trends by analyzing changes in the balance of power between buyers and sellers during the rise and fall of stock prices. &  13 \\
 40 &  VROC~\cite{colby1988encyclopedia} &  Volume change rate indicator measures the range of changes in trading volume at a certain moment. &  3 \\
 41 &  M2C~\cite{colby1988encyclopedia} &  M2C indicator measures the relationship between stocks’ closing price and its exponential moving average. &  4 \\
 42 &  OBV~\cite{colby1988encyclopedia} &  On-Balance Volume speculates on stock price trends by counting the `number of trends' in volume changes. &  2 \\
 43 &  PSY~\cite{colby1988encyclopedia} &  PSY is an indicator to count the number of rising days over a period of time. &  4 \\
 44 &  PVT~\cite{colby1988encyclopedia} &  Price Volume Trend not only measured the price-volume trend relative to the previous day but also measures the relative price-volume trend N days ago. &  2 \\
 45 &  RVI~\cite{colby1988encyclopedia} &  RVI is used to predict the direction of volatility, which predicts the strength of prices by calculating volatility rather than changes in prices. &  6 \\
 46 &  StochRSI~\cite{colby1988encyclopedia} &  StochRSI is an oscillator indicator to measure the RSI indicator. &  3 \\
 47 &  VOSC~\cite{colby1988encyclopedia} &  The volume moving average indicator measures the running trend of the volume and determines the direction of the trend change. &  2 \\
 48 &  VEMA~\cite{colby1988encyclopedia} &  Exponential moving average of trading volume over a period of time. &  2 \\
 49 &  RSV~\cite{colby1988encyclopedia} &  Stochastic value for each period. &  5 \\
 50 &  WR~\cite{colby1988encyclopedia} &  Williams overbought/oversold index. &  5 \\
 51 &  VR~\cite{colby1988encyclopedia} & A measure that helps investors follow the volatility of a stock's price. &  3 \\
 52 &  VCR~\cite{colby1988encyclopedia} &  Volume cumulative return. &  3 \\
 53 &  EMA~\cite{colby1988encyclopedia} &  Exponential moving average. &  1 \\
 54 &  Momentum Std~\cite{fama1993common} &  Standard deviation of trading momentum over a period of time. &  3 \\
 55 &  Momentum Mean~\cite{fama1993common} &  Average of trading momentum over a period of time. &  3 \\
 56 &  101 ALPHA~\cite{kakushadze2016101} &  101 ALPHA is published recently which includes a collection of 101 technical indicators. We choose 77 factors from them. &  77 \\
 57 &  MF Series 1~\cite{leontief1993money} &  Money flow indicators series one. This group compares the volume-weighted average prices of trading orders in different groups (extra large, large, medium, and small). &  12 \\
 58 &  MF Series 2~\cite{leontief1993money} &  Money flow indicators series two. This group compares the trading volume among different group of buy and57 sell orders (extra large, large, middle,small). &  36 \\
 59 &  MF Series 3~\cite{leontief1993money} &  Money flow indicators series three. This group compares the volume of buy and sell orders over different periods (extra large, large, middle,small). &  30 \\\hline
  &  Summary &   &  337 \\
\end{longtable}
}
\newpage

==> figures/a_evaluation.tex <==







==> framework.tex <==





==> frequent_questions.tex <==

\section{FAQ}\label{sec:faq}
\myparab{Why focus on technical features but fundamental features are not included?}

Prediction models can be categorized into the following four groups based on the  technical and non-technical features used by the model.
\emph{Group 1. Technical models.} Technical models rely on technical factors to predict stock returns. A technical feature is constructed from information related to trading activities, such as a stock’s historical price/trading volume, the evolution of the bid-ask spreads, or the number of transactions worth 1 million dollars or more on the last trading day. A non-technical feature could be the revenues of the underlying company (see models in group 2 discussed below), news about the company, or postings on the social networks of its major shareholders.  \emph{Group 2. Fundamental models.} Fundamental models rely on statistics related to a company's financial status, such as revenues, research expenses, and price-earning ratios. These technical factors, also called fundamental factors, can characterize a company's long-term behavior, such as whether its products will stay competitive in the next few years. Fundamental factors are usually extremely sparse. For example, quarterly revenue information provides four datapoints points for one stock each year~\cite{das1998earnings,pritamani2001return,kelly2019characteristics}. 
\emph{Group 3. Macro models.} Macro models rely on  macroeconomic conditions' of the nation which a company calls home, or is registered to conduct business. For example, if a nation subsidizes renewable energy, an electric vehicle company may benefit from a rise in its stock price.
\emph{Group 4. Event models.} Event models capture  price fluctuation due to the release/announcement of new information to the market. For example, replacing the CEO can cause a positive price fluctuation, whereas breaking news about merger and acquisition can drive down the acquiring company’s stock price. 

\mypara{Not using fundamental and macro factors.} These two types of factors are usually not used for building machine learning models forecasting 5-day returns. \emph{(i)}  
fundamental and macro factors have long-term  (multiple months) impact to stock prices so they are not suitable for forecasting 5-day returns. \emph{(ii)} Simple linear regressions are widely used for fundamental and macro models partly because of data sparsity. 

%Not all models rely on machine learning techniques. For example, simple linear regressions are widely used for fundamental and macro models partly because of data sparsity. 

%Since our work focuses on the use of ML techniques for technical and event models, beginning with some notations below, we discuss the modeling, system, and educational challenges related to the use of FML. 


\iffalse
\emph{Technical features.}  The technical features are constructed from information related to trading activities, such as a stock’s historical price/trading volume, the evolution of the bid-ask spreads, or the number of transactions worth 1 million dollars or more on the last trading day.

\emph{Fundamental models.} Fundamental models rely on statistics related to a company's financial status, such as revenues, research expense, and price-earning ratios. These technical factors, also called fundamental factors, can characterize a company's long-term behavior, such as whether its products will stay competitive in the next few years. However, fundamental factors are usually extremely sparse. For example, quarterly revenue information provides four datapoints points for a stock each year~\cite{das1998earnings,pritamani2001return,kelly2019characteristics}.
\fi


\myparab{Why do you perform experiments only on the China market?} 
\emph{(i)} The US and Chinese markets are the two largest equity markets by trading volume~\cite{liu2019size}, and the
Chinese market has attracted increasing attentions.
\emph{(ii)} Among important recent results, many were evaluated soly in the Chinese market
(e.g., ~\cite{wang2019alphastock,feng2019temporal,chen2019investment,wu2019adaptive,gu2019autoencoder,ding2015deep,zhang2017stock,hu2018listening}). 
%Using the US market is not a better option for comparison purposes, 
%\emph{(iii)} there is no evidence that an effective strategy in one market is not effective in the other market for models forecasting 5 to 10 days returns. Note that this is not true for intraday/high-frequency trading or models that have very low turnover, and 
\emph{(iii)} The license cost for China market data is significantly lower than that of the US market. 
%So at least half of the algorithms need to be tested in a different market from what they were originally designed for, 
%Regardless of the choice of the markets. 
%\emph{(iii)} There seems to have no evidence that an effective strategy in one market becomes completely ineffective in a second market. \emph{(iv)} The license cost for Chinese market data is significantly lower than that of US markets.  

\myparab{Why not making money, instead of publishing?}
Empirical asset pricing is a long and established area~\cite{gu2020empirical,jegadeesh1993returns,fama1996multifactor,fama1993common,colby1988encyclopedia}, in which the predictability of equity returns is extensively studied. The reasons we share our research results are similar to those of researchers in the same field. Some of our considerations include: 
\begin{itemize}
    \item \emph{Signal is only a part of a large system.}
    Building a profitable system requires substantially more optimization and engineering efforts 
    than merely discovering the signals~\cite{feng2019taming}. In other words, while identifying ``alpha'' signals is an important part of a trading system, other parts (such as data acquisition and execution) also play an important role in building a reliable and profitable trading system.
    \item \emph{Execution quality.} Hundreds of stocks need to be traded every day. While building this trading system (using standard brokers such as Interactive Broker or its equivalence in China) is feasible, it involves a highly non-trivial amount of engineering work. An effective and robust execution system without incurring large slippage cost is itself a highly nontrivial component and is beyond the scope of this paper. %In addition, the slippage assumption made in this paper can only be done by institutes with strong engineering support. 
    \item \emph{Fees and robustness} Although our strategy is stable and has a high Sharpe, we note that we did not account for the the transaction cost and slippage, which are nontrivial since the holding period is only 5-days.
    %is insufficient for risk-averse individual investors. 
    We estimate that after accounting for the transaction cost and slippage, with approximately 5\% to 10\% probability that an individual may still experience a loss in any specific year. 
    This may not be acceptable for extremely risk averse investors.
    Hence, to obtain a robust industry level strategy, many components of our strategy need to be optimized.  
    %whereas it is fine for institutions because in part institutions are often much less risk-averse so that they can afford to lose (a small amount of) money for a year or two~\cite{mslf}. 
    %{\color{red} maybe cite the performance of some open funds by GSAM or Morgan Stanley?} 
    %(ii) portfolio managers usually construct a portfolio based on multiple strategies so that the portfolio becomes truly robust. While each individual portfolio could be potentially valuable, only combining more than one portfolio can result in robust.
   % \qq{we already have the consolidation part}
    %{\color{red} we need to verify that we are not making contradictory statements, i.e., our strategy is a strong one but it is insufficiently strong to become a ``stand-alone'' portfolio. 
    %} \qq{need to update, our sharp is 10 now}
    %\item \emph{``Slow'' strategies.}
\end{itemize}



%\emph{Signal is only a part of a large system.}Building a profitable system requires substantially more resources than discovering the signals.

%In other words, while identifying ``alpha'' signals is an important part of a trading system, other parts (such as data acquisition) also play an important role in building a reliable and profitable trading system.

%\mypara{Academic values of asset pricing research.}Finally, we also re-iterate a few reasons besides its applied value. 
%\mypara{Decays and industrial collaboration.}








==> impact.tex <==

\iffalse
\section*{Broader Impact: Ethical Considerations}
Our work can potentially increase the competitiveness of quantitative investment. In general, building stronger predictive models could make adversarial impact to less-competitive investment managers and cost their jobs in some circumstances~\cite{schoning2018s}.

{\scriptsize
\noindent \textbf{(From Neruips FAQ) Does the eight-page limit include references?} Answer: No. The page limit refers to content pages only; \textbf{additional pages containing the impact statement and references are allowed.} Acknowledgements and funding disclosure should also be included here, but only for the camera-ready submission.
}
\fi
\section*{Broader Impact: Ethical Considerations}
Our work can potentially increase the competitiveness of quantitative investment. In general, building stronger predictive models could make adversarial impact to less-competitive investment managers and cost their jobs in some circumstances~\cite{schoning2018s}.
%Compared to examples in the suggested reading~\ref{schoning2018s}, 

==> intro_nips_2021.tex <==


\section{Introduction}
Consider the problem of simultaneously forecasting returns of a large collection of stocks in the equity market. We aim to build models that reveal the underlying  ``dependencies'' between stocks.  e.g., positive news on Apple Inc.'s sales could impact prices of Apple's component providers~\cite{hertzel2008inter,wu2014supply,lu2017impact}.  Designing such models has been remarkably difficult because one needs to circumvent two challenges that require often incompatible solutions.  
\textbf{\emph{1. High dimensionality}}, which refers to problems with more parameters than observations, leading to overfitting issues. For example, in a portfolio of 3,000 stocks, the total number of potential links between pairs of stocks is $3,000 \times 3,000 \approx 10^7$, but we often have only 2,500 data points (e.g., 10 years of daily data). To design a high-dimensional algorithm, one usually needs to mathematically understand the root cause of the overfitting, and design regularization techniques to alleviate such issues. Most algorithms in this category are linear and have theoretical guarantees.
\textbf{\emph{2. Nonlinearity.}} Features and responses (stocks' returns) usually have non-linear interactions. Machine learning ``black boxes'' such as deep learning (DL) or gradient boosted algorithms are the most effective in extracting non-linear signals, but they often do not come with theoretical guarantees.

%\qq{Might be we can put the challenges together and existing works together? Then explain existing works only solve one of these two challenges.}


Integrating solutions for these challenges has been a frustrating endeavor for the community of both academics and practitioners. For example, we experimented using mainstream machine learning black boxes to learn high-dimensional problems, and found ourselves in ``the worst of both worlds'' where the algorithm cannot learn non-linear signals and has overfitting problems. %{\color{blue} insert a fig.} 
%\qq{I am not sure whether we need to add this paragraph}


Such challenges were recently recognized~\cite{wang2019alphastock,feng2019temporal,chen2019investment,wu2019adaptive}, leading to the introduction of latent embedding models. The central idea is to project the stocks into points in a low-dimensional space so that similar stocks are closer in the embedding. Because point interactions are more restrictive in the latent space, they have the potential to address the overfitting issues~\cite{wang2019alphastock}. However, these lines of work do not offer any theoretical guarantees, and are often not robust in practice.  
%\qq{This part delivers the same message with the sentences after Nonliearity.}

%We revisit the stock embedding model, with the goal of designing a suite of \textbf{statistically sound} and  \textbf{practically effective} algorithms optimized for a natural latent model that has been used extensively. 


We revisit the stock embedding problem, and discover that we shall \emph{not} find a ``one hammer for all'' solution. 
Instead, under mild assumptions, the learning architecture needs to be decoupled into two components. The first component estimates stocks' latent positions, which can be solved \emph{provably} by using high-dimensional statistics techniques. The second component uses latent information to forecast returns, which can be implemented by either theoretically sound non-parametric methods when the feature size is small, or machine learning techniques optimized to use latent position information. 
Our experiments also confirm that the decoupling principle is essential because the algorithms that do not follow this principle perform significantly worse. 
%{\color{red} add a sentence on the ``negative results''.}

Our algorithmic framework results in a unification of two approaches for forecasting equity returns. Compared to deep learning and ensemble methods~\cite{gu2020empirical}, our solution insulates the component with the greatest overfitting risk and ``out-sources'' it to high-dimensional algorithms; compared to factor-based models~\cite{stock2002forecasting,stock2005implications}, our decoupling principle enables these models to utilize recent powerful ML techniques while still maintaining low overfitting and interpretable properties. 

%To give a holistic view of our approach, an analogy can be made with the factor analysis methodology, a fundamental tool in economics/financial econometrics for the last half a century. Factor models are statistical models aimed at capturing complex interactions though a small number of causal factors, which simultaneously addresses the issues of dimensionality reduction of models to render more feasible the estimation process, and also to uncover the latent causes that drive the data. Such examples include macroeconomic factors, fundamental factors, or statistical factors (which altogether facilitate the process of interpreting the results), which are then typically leveraged for subsequent analysis/prediction via linear models. The dichotomy between standard ML techniques and our proposed pipeline which decouples the process of learning the latent embedding from that of learning the link/interaction function of the quantity of interest and the latent factors, can be indeed construed as an instance of the above paradigm that has dominated the econometrics literature for the last several decades. In a nutshell, our proposed pipeline further pushes the boundary in this direction, by essentially  incorporating a nonlinearity component into both stages of the pipeline, while preserving scalability to the high-dimensional setting, and improving the prediction power and interpretability of the model (?).

% (too long need to compress this more into a few sentences... )

% (another example of a classical similar 2-stage approach is the closely related principal component regression)

% (need to find some good references.. maybe financial econometrics, though nips reviewers might not appreciate this.. probably many think econometrics is a waste of time/resources in 2020 :) )

%We highlight the three main contributions of our work:
In summary, we made three main contributions:
\textbf{C1. Theory.} We develop the first algorithm that can provably estimate the stocks' latent positions and provide theoretical guarantees. Our novel analysis leverages a diverse set of tools from kernel learning, non-parametric methods, and random walks. \qq{only mentioned the theoretical guarantees for component 1.} \textbf{C2. Practice.} We improve the performance of these theoretical results by introducing a decoupling principle and new machine learning techniques. This includes simplified deep learning architectures with enhanced forecasting power, and a new time-efficient boosting algorithm. \textbf{C3. Community.} Given that our results are highly empirical, a rigorous evaluation platform is needed, which is not available to the machine learning and finance community to present date. We develop the first open-source rigorous evaluation framework and explain major pitfalls in evaluating forecasts.

%{\color{red} todo: 
%\begin{itemize}
%    \item From MC: cite MC's %paper on news sentiment propagation.  MC: ok will update\end{itemize}}
%This paper makes contributions at three fronts. 



==> notation.tex <==


\section*{Notations}
\begin{itemize}
    \item $d$: the number of stocks. 
    \item $n$: the number of observations (the number of training days). 
    \item $\ms_{i,t}$: the (unobserved) factor associated with stock $i$ at time $t$. 
    \item $\mx_{i, t}$: the observed features associated with stock $i$ at time $t$. 
    \item $k$: the number of features. 
    \item $r$: the dimension of the latent space. 
    \item $\ell$: the number of hint matrices. 
\end{itemize}

{\color{blue} paper structure}

\begin{itemize}
    \item Page 1 to 2 intro. 
    \item Page 3 model. 
    \item page 4 our algorithm. 
    \item page 5 evaluation framework
    \item page 7 and 8 evaluation. 
\end{itemize}

{\color{blue} Full paper (without space constraint)}

\begin{itemize}
    \item Page 1 to 2 intro. 
    \item Page 3 to 4: model. 
    \item Page 5 to 6.5: Overview of our approach (main provable result and how we can design a two-staged algorithm).  
    \item Page 6.5: to page 14: analysis. 
    \item page 15 to page 18: all of our algorithms. 
    \item Page 18 to 19: Our system framework; why rigorous simulation is necessary. 
    \item page 20: Introduction of experiments. 
    \item Page 21 to 22: description of baselines. 
    \item Page 23 to 29 evaluation. 
    \item Page 30: conclusion. 
    \item Page 30 to 35: appendix: more math. 
\end{itemize}

==> outline.tex <==


\section*{Notations}
\begin{itemize}
    \item $d$: the number of stocks. 
    \item $n$: the number of observations (the number of training days). 
    \item $\ms_{i,t}$: the (unobserved) factor associated with stock $i$ at time $t$. 
    \item $\mx_{i, t}$: the observed features assocated with stock $i$ at time $t$. 
    \item $k$: the number of features. 
    \item $r$: the dimension of the latent space. 
    \item $\ell$: the number of hint matrices. 
    \item $f_{\mu_z}(\cdot)$ the pdf of $\mz$'s. 
\end{itemize}

{\color{blue} paper structure}

\begin{itemize}
    \item Page 1 to 2 intro. 
    \item Page 3 model. 
    \item page 4 our algorithm. 
    \item page 5 evaluation framework
    \item page 7 and 8 evaluation. 
\end{itemize}

{\color{blue} Full paper (without space constraint)}

\begin{itemize}
    \item Page 1 to 2 intro. 
    \item Page 3 to 4: model. 
    \item Page 5 to 6.5: Overview of our approach (main provable result and how we can design a two-staged algorithm).  
    \item Page 6.5: to page 14: analysis. 
    \item page 15 to page 18: all of our algorithms. 
    \item Page 18 to 19: Our system framework; why rigorous simulation is necessary. 
    \item page 20: Introduction of experiments. 
    \item Page 21 to 22: description of baselines. 
    \item Page 23 to 29 evaluation. 
    \item Page 30: conclusion. 
    \item Page 30 to 35: appendix: more math. 
\end{itemize}

\newpage

==> residual.tex <==


{\color{red} 
\section{some residual}}



{\color{red} ZL's question: are we able to write down many results for different cases? }

{\color{blue} some self-notes for ZLiu: need to make sure that we still have theoretically groundd-results if some of the assumptions are violated.}



\begin{equation}
    \mr_{t} = M \mr_{t - 1} + \epsilon_t, 
\end{equation}
where $M \in \reals^{n \times n}$. In practice, $n \approx 3000$ (e.g., in the US market), whereas the number of observations is also around 3,000 (i.e., 10 years of data). The number of learnable parameters in $M$ is 
$3,000 \times 3,000 = 10$ million. Therefore, we cannot even properly fit a linear model without carefully regularizing it. 



\myparab{The power of non-linearity.} On the other hand, it has been repeatedly demonstrated that when manually crafted features are fed into a non-linear model, we are able to produce significantly more powerful forecasts than linear ones. 

Thus, our goal is to build non-linear cross sectional models with sound theoretical guarantee. {\color{red} Be careful to check notation consistencies.} Specifically, we aim to bulid the following model
\begin{equation}
    \my_t = D f(\mx_t), 
\end{equation}
where 
\begin{itemize}
    \item $n$ is the number of stocks. 
    \item $\my_t \in \reals^n$
    \item $\mx_t \in \reals^{n \times d}$, where 
    $(\mx_t)_i$ represents the features associated with the $i$-th stock on day $t$.
    \item $f: \reals^{n \times d}\rightarrow \reals^n$ is a (possibly non-linear) function that transforms features into signals. 
    \item $D$ is the matrix handling the interactions between signals. 
\end{itemize}

{\color{blue} some clarification on the notations:} We assume that $\ms_t = f(\mx_{i, t}) \in \reals^n$. 

\myparab{Latent structure.} We examine imposing latent structure for the matrix $D \in \reals^{n \times n}$. Specifically, we assume that each stock $i$ is associated with a latent variable $\mz_i$. We further assume that $D_{i,j} = \kappa(\|\mz_i - \mz_j\|)$, where $\kappa$ is a universal kernel function {\color{blue} check the definition of universal; from the jhu paper} that is monotonicalyl decreasing. Examples of these functions include: 
\begin{enumerate}
    \item Graussian kernel function $\kappa(\mx, \my) = \exp\left( - \frac{\|\mx - \my\|^2}{\sigma^2}\right)$, where $\mx, \my \in [0, 1]^{c}$. {\color{red} check: which letter to use for the dimension of the latent space.}
    \item Polynomial kernel 
    \begin{equation}
    \kappa(\mx, \my) = \frac{\epsilon}{\|\my - \mx \|^2 + 1}        
    \end{equation}
    {\color{red} check the details of this; use nips 2017.} 
    \item {\color{red} Fill in other examples.}
\end{enumerate}

\myparab{Theoretical guarantee.} We make the following assumptions. 

\mypara{A1.} $d = 1$, i.e., $\mx_t \in \reals^n$. Each component $\mx_{t_i}$ is i.i.d. distributed. 

\mypara{A2.} $f(\mx_t)$ is a component-wise function, i.e., $f(\mx_t) = (f(\mx_{t, 1}), f(\mx_{t, 2}), \dots, f(\mx_t, n)$. 
{need to clear up notations}


\mypara{A3.} Let $\ms_{t, i} = f(\mx_{t, i})$. From A2, we can see that $\{\mz_{t, i}\}_{i \leq n}$ are i.i.d. We further assume that $\E[\ms_{t, i}] = 0$ and $\Var[\ms_{t, i}] = 1$. Let us also explain the justification for this assumption. \emph{(i)} $\E[\ms_{t, i}] = 0$: this is because by efficient market hypothesis, $\E[\my_t] = 0$. This implies $e[\mz_t] = 0$. Otherwise, the expectation of the return would be non-zero. \emph{(ii)} $\Var[\mz_{t, i}] = 1$ is a standard normalization assumption {\color{blue} check this very carefully.} 

\myparab{Our algorithm.} Our major contribution is the design of an algorithm that decouples the task of estimating the latent space from the task of of learning the non-linear function. We first prove that the latent space can be reliably discovered by using a small number of samples. Then we show that once we have sufficiently accurate estimate on the nodes' latent positions, we can use simple moment-based method to produce estimate of $f(\cdot)$. This method has provable generalization guarantee. 

This approach is only a specialization of an algorithm under the framework we offer. In this framework, we decouple the problem of estimating the latent space from the problem of learning non-linear functions. Additional algorithms can be designed to solve each of the insulated problems. 

\myparab{1. Solving the latent space embedding problem.} We also derive other possible approaches to solve the latent space embedding problem. For example, $D$ can be evolving so we may not have sufficient data to track $D$. But on the other hand, we may apply domain knowledge and assume that 
\begin{align}
    D_t = \beta_1 D^{(1)}_t + \beta_2 D^{(2)}_t. 
\end{align}

{\color{blue} This paragraph is rough; we need a second iteration.} 

We assume that $D_t$, $D^{(1)}_t$, and $D^{(2)}_t$ are evolving but $\beta_1$ and $\beta_2$ are constants, which do not change over time. So our main objective here is to estimate $\beta_1$ and $\beta_2$. 

\myparab{2. Learning the non-linear interactions.} We may use other building blocks (such as deep learning) to extract non-linear features. 

\myparab{Additional assumptions.} We assume that the stocks are uniformly distributed on the latent space $[-1, 1]^r$ {\color{blue} check: the latent dimension should be $r$ instead of $c$.} This assumption can be relaxed; but we probably still need the distribution to be smooth almost anywhere. Our analysis also assumes that we use a Gaussian kernel. Again, this assumption can be relaxed. 

{\color{red} if we use $n$ to represent the number 
of stocks, we should use $T$ to represent the number of observations.} 
Now we can express the interaction among latent positions, features, and responses using the following equation: 
\begin{equation}
    \mY = \mS D + E, 
\end{equation}
where $\mS \in \reals^{T \times n}$ is the matrix stacking together all the signals and $\mY \in \reals^{T \times n}$ is the matrix that stacks together all the responses. Observe that 
\begin{equation}
    \frac 1 n \mY^{\transpose} \mY = D^{\transpose}\left(\frac 1 n \mS^{\transpose}\mS\right) D + \frac 1 n \mZ^{\transpose} E. 
\end{equation}

\myparab{Known building blocks.} Let $U_D S_D U^{\transpose}_D$ be a low rank approximation of $D $ (with a suitable choice of the rank). Also let $\epsilon$ and $\delta$ be the parameter we use for our ICML submission. Using standard results from kernel learning, we have (copied from our nips paper). 

\begin{lemma} 
\begin{equation}
\| U_D S^{\frac 1 2}_D W - \Phi_d(\mZ)\|_F \leq 2 \sqrt 2 \frac{\sqrt{(\log \epsilon)^{-1}}}{\delta}.
\end{equation}
\end{lemma}

\myparab{Some scaling things.} The scale of $D$: we have $\|U_D S^{\frac 1 2}_D\|^2_F = d$. Intuitively, each row in $U_D S^{\frac 1 2}_D$ corresponds to a feature map for one point (stock). The $\ell_2$-norm for each feature map is a constant. Therefore the square of Frobenius norm scales linearly with the number of stocks. 

The decay of eigenvalues: $\lambda_i(\kappa) \leq \sqrt K C'\exp(-C i^{\frac 1 r})$ ($K$ is an upper bound on the kernel function). This comes from the reference ``approximation beats concentration? an approximation view on inference with smooth radial kernel''. Now there is a scaling effect (together with some statistical errors). We have

\begin{equation}
    \lambda_i(D) \approx n \lambda_i(\kappa). 
\end{equation}

\mypara{Use standard building block to do dimension reduction.} Let $\varepsilon$ be the estimation error. We need to set up $\delta$ such that the gap is larger than $\varepsilon$. Then we can know the tail is a function of $\delta$. 

\myparab{Comptuation of $\varepsilon$. }
Let $\lambda^*_1, \lambda^*_2, \dots, \lambda^*_{\calh}$ be the eigenvalues associated with the kernel function $\kappa$ and the probability measure $\mu$. {\color{blue} need to define probability measure.} For simplicity, we shall assume that $\mu$ is a uniform distribution on $[0, 1]^r$. We have 

\begin{equation}
    \lambda_i(\kappa_{\mu}) \leq \sqrt{K} C' \exp(-Ci^{\frac 1 r}). 
\end{equation}

Now let's revisit the equation $\mY = \mS D + E$. Recall that we have 
\begin{align*}
    \mY^{\transpose}\mY & = (\mS D + E)^{\transpose}(\mS D + E) \\
    & = D^{\transpose}\mS^{\transpose}\mS D + D^{\transpose} \mS^{\transpose} E + E^{\transpose} \S D + E^{\transpose} E. 
\end{align*}

{\color{blue} be careful; we cannot assume that $\mS$ are standard Gaussian; so we need to find more general concentration bounds.}

Now we also need to do normalization. \begin{align*}
    \frac 1 n \mY^{\transpose}\mY = D^{\transpose}D + D^{\transpose}\left(I - \frac 1 n \mS^{\transpose}\mS\right)D + \frac 1 n D^{\transpose} \mS^{\transpose}E + \frac 1 n E^{\transpose} \mS D + \frac{\mS^{\transpose}\mS}{n}. 
\end{align*}

\mypara{The scale of $D$ and $D^{\transpose}D = D^2$ (because $D$ is symmetric.} We know that $\lambda_i(D/n)$ converges to $\lambda^*_i$ for $D$ as $n$ grows. Therefore, $\lambda_i(D) = n \lambda^*_i$ {\color{blue} the text looks quite repetitive.} $\|D\|^2_F = \Theta(n^2)$ {\color{red} this seems to be the correct one; the earlier one seems wrong.} We can also see that $\|D^{\transpose}D\|^2_F = \Theta(n^4)$. Next, we can also see that {\color{blue} be careful; there are some subtle issues; see our icml submission.} 
\begin{equation}
    \left\|I - \frac{\mS^{\transpose}\mS}{n}\right\|_2 = \Theta\left(\sqrt{\frac{n}{T}}\right)
\end{equation}

For the spectral norm of $\mS^{\transpose} E/ n$, we know that each entry is of order $\Theta\left(\frac{1}{T}\right)$. 

{\color{red} need to be careful about why the dimension reduction is needed.}  Now this is what we get so far: the ground-truth that we want to estimate is $\frac 1{n^2}D D^{\transpose}$. The observed data is \begin{equation}
    \frac 1 {n^2} DD^{\transpose} + \cale, 
\end{equation}
where $\|\cale\|_F \leq \varepsilon = O\left(\sqrt{\frac n T} + \sqrt {\frac{\sigma^2_{\epsilon}}{Tn}}\right).$

Let $\frac{1}{n^2}DD^{\transpose} + \cale = U\Sigma U^{\transpose}$. The left hand side is symmetric because we get it from $\mY^{\transpose}\mY$ {\color{red} check it.} Let $\frac{1}{n^2}D D^{\transpose} = U^*\Sigma^* (U^*)^{\transpose}$. So 
$U^* (\Sigma^*)^{\frac 1 4}$ is what we want. We aim to show that $U^* (\Sigma^*)^{\frac 1 4}R \approx U\Sigma^{\frac 1 4}$. {\color{blue} maybe we already assumed that they are low rank. Check.} 

Let $A = \frac 1{n^2}D D^{\transpose}$ and $B = \frac 1{n^2} D D^{\transpose} + \cale$. Let $A_k$ be the rank-$k$ approximation of $A$ and $B_k$ be the rank-$k$ approximation of $B$. {\color{blue} ZL's random thoughts: the argument still looks highly complex. Maybe we should highlight the difference between this analysis and the one in nips 2017.} We have 
\begin{equation}
    \|A_k - B_k\|_F \leq \varepsilon + \frac{\varepsilon^2}{\delta^2}. 
\end{equation}
Let 
\begin{align*}
A^{\frac 1 2}_k &  = U^*_k (\Sigma^*_k)^{\frac 1 2}(U^*_k)^{\transpose} \\
B^{\frac 1 2}_k & = U_k \Sigma^{\frac 1 2}_k (U_k)^{\transpose}. 
\end{align*}

We have (result from nips 2017) {\color{blue} remember to check whether the inequality below is F-norm or 2-norm:}: 
\begin{equation}
    \left\|U^*_k (\Sigma^*_k)^{\frac 1 2}W - U_k \Sigma^{\frac 1 2}_k\right\|_F \leq \frac{\varepsilon^2}{\delta^2}. 
\end{equation}

Let $M_1 = U^*_k (\Sigma^*_k)^{\frac 1 2}W$ and $M_2 = U_k \Sigma^{\frac 1 2}_k$. Let also the SVD of $M_1$ and $M_2$ be 

\begin{align*}
    M_1 & = U_1 D_1 V^{\transpose}_1 \\
    M_2 & = U_2 D_2 V^{\transpose}_2.
\end{align*}

{\color{red} be careful; there are some overload of $D_i$.}
A lemma in ``no spurious local minima: a unified geometric analysis'' says: 
\begin{equation}\label{eqn:diff}
    \|U_1 D_1 U^{\transpose}_1 - U_2 D_2 U^{\transpose}_2\|^2_F + \|V_1 D_1 V^{\transpose}_1 - V_2 D_2 V^{\transpose}_2\|^2_F \leq 2 \|M_1 - M_2\|^2_F. 
\end{equation}
{\color{red} there is a dependency on $k$, i.e., the dimension to keep; need to check that whether we can relax the dependency; or maybe the dependency is not relevant. }

(\ref{eqn:diff}) implies that 
\begin{equation}
    \|U_1 D_1 U^{\transpose}_1 - U_2 D_2 U^{\transpose}_2 \|_F \leq 2 \|M_1 - M_2\|_F \leq \sqrt 2 \kappa \frac{\varepsilon^2}{\delta^2}. 
\end{equation}

This means 
\begin{equation}
    \|U^*_k (\Sigma^*_k)^{\frac 1 2}(U^*_k)^{\transpose} - U_k\Sigma^{\frac 1 2}_k U^{\transpose}_k \|_F \leq \frac{2k^2 \varepsilon^2}{\delta^2}. 
\end{equation}

Now apply the square root result again 
{\color{blue} we need to tweak the result from the universal consistent paper.} 
\begin{align*}
    \|X W - Y\| \leq \|X \|\|(T^{\transpose}T)^{\frac 1 2} - I\|_F + \|R\|_F \|Y\|\|(Y^{\transpose}Y)^{-1}\|.
\end{align*}
Note that 
\begin{equation}
    \|(T^{\transpose}T)^{\frac 1 2}- I\|_F \leq \|T^{\transpose} T - I\|_F \leq \frac{\|R\|_F}{\delta}. 
\end{equation}
Also, we have 
\begin{equation}
    \frac{\|X\|\|R\|_F}{\delta} + \frac{\|R\|_F\|Y\|}{\delta} = \|R\|_F\frac{\|X\| + \|Y\|}{\delta}. 
\end{equation}
So we have a modified lemma. 








. 


{\color{red} need to check the wording here.}

{\color{blue} ZL: need to give a name to these algorithms.}



\section{Notations}
\begin{itemize}
    \item $d$: the number of stocks. 
    \item $n$: the number of observations (the number of training days). 
    \item $\ms_{i,t}$: the (unobserved) factor associated with stock $i$ at time $t$. 
    \item $\mx_{i, t}$: the observed features assocated with stock $i$ at time $t$. 
    \item $k$: the number of features. 
    \item $r$: the dimension of the latent space. 
    \item $\ell$: the number of hint matrices. 
\end{itemize}


{\color{red} todo: need to find out all related papers; otherwise, it will be wasting time.}

{\color{red} notational issues: $\varepsilon$ or $\epsilon$?}

{\color{blue} some clarification of notations: $\mx$ are the features, $\ms$ are the signals, $\my$ are the responses.} 



{\color{blue} other additional remarks: 
\begin{itemize}
    \item We shall pitch that as a contribution to both building a platform (or building a benchmark) and designing an algorithm that captures the non-linear interactions between stocks.
\end{itemize}

}


\subsubsection{Deep learning}


{\color{red} Qiong is also testing the performance of GRU}

\begin{table}[ht!]
\centering
  \caption{The neighbors for each center stock  }
   \includegraphics[width=0.8\linewidth]{figures/cluster_table.pdf}
\end{table}



potential serial dependencies of the return series {\color{blue} be careful; this sentence could be problematic.}. We examine LSTM, with a standard way to feed the features into LSTM~\cite{hochreiter1997long}
    {\color{blue} is this a standard reference for LSTM?} We
    do not report results from other RNN because their performances are similar. 
    
    The Long Short Term Memory(LSTM) based price prediction mode is one of the state-of-the-art baselines. This model is proposed by~\cite{nelson2017stock} and operates on the sequential indicators, which enables it to capture the long-term dependency of stock prices at different moments. {\color{blue} Question for Qiong: why we don't use other RNN? Maybe just the performance are similar? Do we need to describe LSTM at this level of details?}
    




%\begin{figure*}[ht!]
%\includegraphics[width= 0.8\linewidth]{figures/synthetic/mse_vs_low_rank_level_2000.png}
%\label{fig:mse_vs_low_rank_level_2000}
%\end{figure*}

\myparab{TODO list}
\begin{itemize}
    \item check on different functions (how to visualize? leave as a question)
    \item May need to prepare a table for all results
    \item May need to run each experiment 5 times to get average.
\end{itemize}
{\color{blue} todo: explain that it is not about competition; it is about understanding whether we can consolidate everything. todo: add synthetic data. 
}

\myparab{Table 1. Improvement at the factor level.} This table examines the factors that can be improved by considering the neighbors. 

Plot four pictures in a graph (draw data driven, barra inner product, barra l2, barra + news); but we will use only 1 at the end. 
\begin{itemize}
    \item Scatters of in-sample $r^2$ vs out-of-sample $r^2$. 800; 3000; partition methods and linear (maybe will only use partition at the end. 
    \item Two curves showing some kind of variance-bias tradeoff by choosing the number of partitions. Maybe for each $k$, plot bar charts of the factors (median plus quantiles).
\end{itemize}

{\color{red} todo for Zheng}
Produce one table to summarize the results. 




{\color{red} experiment section can end here. }

\newpage \newpage


\myparab{Table 2. Overall performance for 800 and 3000.} No need to break down by years; 

One table for 800 and one table for 3000. 
Table should include the following columns: 
\begin{itemize}
    \item $r^2$: weighted, unweighted. 
    \item $t$-statistics: weighted, unweighted,
    \item against raw return and residualized returns (including Mihai's residualized return, if have time).  
    \item Long short sim: uniform weighted and sadv weighted, return, Sharpe,  
    \item Long only sim: uniform weighted and sadv weighted, return, Sharpe, 
\end{itemize}


\begin{figure}
\begin{codebox}
\Procname{$\proc{Boosting-Algorithm}(\mY, \mX, \eta)$}
\li \Comment $\eta$ is the learning rate. 
\li  $\mY_{\Res} \gets \mY$. 
\li \For $j \gets 1$ \To $b$
\li \Do 
$g_i \gets \proc{Linear-Fit}(\mY_{\Res}, \mX)$.

\li For all $t, j$: $(\hat \mY)_{t, j} = \sum_{k \in [d]}K_{j,k}g_i\left((\mX)_{t, k}\right)$
\li $\mY_{\Res} = \mY_{\Res} - \eta \hat \mY$. 
 \End
\li \Return $\{g_i(\cdot)\}_{i \leq b}$
\end{codebox}

\begin{codebox}
\Procname{$\proc{Linear-Fit}(\mY, \mX)$}
\li Let $\mx_{t, i} \in \reals^k$.
\li Let $\mf_{t, j} \in \reals^d$. 
\li For all $i$: $(\mf_{t,j}) = \sum_{k \in [d]}K_{k, i}(\mx_{t, k})_j$. 
\li Let $r_j = \mathrm{corrcoef}(\mf_{t, j}, \my_y)$. 
\li Let $j_1, j_2, j_3$ be the indices with the largest $r_j$. 
\li $g(\cdot) = \arg \min_{\beta_1, \dots, \beta_6}\sum_{\substack{t \leq d \\ i \in [d]}}\left(\my_{t, i} - \sum_{j \in [d]}K_{i,j}\left(\beta_1 (\mx_{t, i})_{j_1} + \dots + \beta_6(\mx_{t, i})_{j_2}\cdot (\mx_{t, i})_{j_3})\right)\right)^2$
\li \Return $g(\cdot)$
\end{codebox}

\caption{Linear boosted algorithms. {\color{red} check the dimensions of $\mX$ and $\mY$} {\color{orange} This is the original version.}}
\end{figure}

\begin{figure}
\begin{codebox}
\Procname{$\proc{Boosting-Algorithm}(\mY, \mX, \eta)$}
\li \Comment $\eta$ is the learning rate. 
\li  $\mY_{\Res} \gets \mY$. 
\li \For $k \gets 1$ \To $b$
\li \Do 
$g_k \gets \proc{Linear-Fit}(\mY_{\Res}, \mX)$.

\li For all $t$: $(\hat \mY)_{t, k} = \sum_{t \in [n]}K_{t}g_k\left((\mX)_{t}\right)$
\li $\mY_{\Res} = \mY_{\Res} - \eta \hat \mY$. 
 \End
\li \Return $\{g_k(\cdot)\}_{k \leq b}$
\end{codebox}

\begin{codebox}
\Procname{$\proc{Linear-Fit}(\mY, \mX)$}
\li Let $\mx_{t, i} \in \reals^k$.
\li Let $\mf_{t, i} \in \reals^k$. 
\li For all $i$: $(\mf_{t,i}) = \sum_{j \in [d]}K_{i, j}\mx_{t, j}$. 
\li Let $r_i = \sum_{t \leq n}\mathrm{Corrcoef}(\mf_{t, i}, \my_{t,i})$. 
\li Let $j_1, j_2, j_3$ be the indices with the largest $r_j$. 
\li $g(\cdot) = \arg \min_{\beta_1, \dots, \beta_6}\sum_{\substack{t \leq n \\ i \in [d]}}\left(\my_{t, i} - \sum_{j \in [d]}K_{i,j}\left(\beta_1 (\mx_{t, i})_{j_1} + \dots + \beta_6(\mx_{t, i})_{j_2}\cdot (\mx_{t, i})_{j_3})\right)\right)^2$
\li \Return $g(\cdot)$
\end{codebox}

\caption{Linear boosted algorithms. {\color{red} check the dimensions of $\mX$ and $\mY$} {\color{orange} I moved the original version to `residual' part.}}
\end{figure}

 {\color{red} explain the table?} One can see that our simple rule is effective in identifying factors that can benefit from using neighbor information.  On average the improvement of the forecasting power (in correlation) is {\color{red}XXX} for the original algorithm and is {\color{red} xxx} for the robust algorithm. When we consolidate all the forecasts into 1 (using a standard method resembling exp3 algorithm {\color{red} cite}), the improvement is {\color{red} xx} for the original algorithm and {\color{red} xx} for the optimized algorithm. {\color{red} Note: 1. make sure text and figure are consistent. 2. give name to the model and give name to the algorithms.}

{\color{red} comments from Mihai}


{\color{red} some text moved from other places.}



At the theoretical front, we introduce a natural latent space model for non-linear signals \MC{here do we mean features or signals? I guess we should clarify this earlier on, I thought by signal we mean our final forecast, and if so perhaps it makes less sense to have ''nonlinear signals"}, and designs a statistically sound time-efficient algorithm to extract the latent positions. Our model assumes that 
\begin{align}
\my_{t, i} = \sum_{j}\kappa(\|\mz_i - \mz_j\|)\ms_{t, j} + \xi_{t, i}, 
\end{align}
where $\xi_{t, i}$ is a zero-mean noise \MC{Gaussian or?}. In other words, stock $i$'s return on day $t$ is a weighted sum of $\ms_{t,j}$, where the weights depend on the distance between $\mz_i$ and the other latent variables $\mz_j$'s. In addition, we assume $\ms_{t, i} = g(\mx_{i,t})$, i.e., the unknown factor $\ms_{t, i}$ is a function of the observable features $\mx_{i, t}$. It is important to stress that we do not have any a-priori knowledge of  $g(\cdot)$, $\mz_i$'s or $\kappa(\cdot)$. 


{\color{blue} more text residuals.}
{\color{blue} move around?}
In this work, we develop a theoretically sound latent-space model that outperform all the recent baselines. Roughly speaking, we aim to develop learning algorithms for the model 
\begin{align*}
\my_{t, i} = \sum_{j}\kappa(|\mz_i - \mz_j|)g(\mx_{t, j}) + \xi_{t,i},
\end{align*}
where $\my_{t, i}$ is the return of stock $i$ on day $t$, $\mz_i$ is the latent position of stock $i$, $\kappa(|\mz_i - \mz_j|)$ is an (unknown) radial-basis function that measures the strength of interactions between stock $i$ and $j$, $\mx_{t, i}$ is the features/characteristics of stock $i$ on day $t$,  $g(\mx_{t, i}) \in\reals$ is another unknown function that translates signal in the latent space, and $\xi_{t, i}$ is a noise. Our goal is to \emph{simultaneously} learn the latent positions $\mz_i$ and the possibly non-linear function $g(\mx_{t,j})$ with minimum sample complexity. 


\MC{people typically forecast close-to-close (that's where also the main liquidity event is). Do we only focus on open-to-open at this point, or 5-day open-to-open?} {\color{blue} I see. We do 5-day open-to-open. We do not have intraday data; does it still make sense to do close-to-close forecast (I feel this will do us harm).}  \MC{To clarify, the news used, do they only arrive outside of market hours? I mean, if all the news come out after yesterday's close until (but before) today open, then indeed it makes most sense to "init" the trades at the open and thus forecast starting at the open. But if the news arrive also intraday (including yesterday intraday (since they would not be used in yesterday's forecasts)) then I don't think we would necessarily be worse off, if we init at the close. } 

\begin{algorithm}[t!]
    \caption{Our algorithm for estimating $g(\cdot)$ }\label{fig:estimateg}
    \hspace*{\algorithmicindent} \textbf{Input} $\mX$, $\mY$, $\hat K$, $\{\Omega_i\}_{i \leq \ell}$\\
    \hspace*{\algorithmicindent} \textbf{Output}  $\{\mu_i\}_{i \leq \ell}$
    \begin{algorithmic}[1]
    \Procedure{$\proc{Estimate-g}$}{$\hat K, \{\Omega_i\}_{i \leq \ell}, \mX, \mY$}
    \ForAll{$t \gets \text{1 to n}$}
    \State $\mx_t = \mX_{t, :}$, $\my_t = \mY_{t, :}$
    \State $\vec C_t = \proc{Reduce-to-Regress}(\hat K, \mx_t)$
    \EndFor
    \State $\mu_1, \dots \mu_{\ell} \gets$ $\proc{Solve-Regression}$ $(\{\my_t, \vec C_t\}_{t \leq n})$
    \State \Return $\mu_1, \dots \mu_{\ell}$
    \EndProcedure
    
    \Procedure{$\proc{Reduce-to-Regression}$}{$q_t, \{\my_{t, j}, \mx_{t, j}\}_{j \leq d}, \{\Omega_j\}_{j \leq \ell})$} \\
    \Comment Reduce observation $\my_{t, q_t}$ to an observation in the regression problem for $\mu_j$'s.
    \State Let $\hat L_{(t, q_t), j} = 0$ 
    \ForAll{$k \gets 1$ \To $d$}
    \State Find $\Omega_j$ such that $\mx_{t, k} \in \Omega_j$
    \State $\hat L_{(t, q_t), j} +=\hat  K_{q_t, k}$
    \EndFor
    \State \Return $\{\mu_i\}_{i \leq \ell}$
    \EndProcedure
    
    \Procedure{$\proc{Solve-Regression}$}{$q_t, \{\my_{t, j}, \mx_{t, j}\}_{j \leq d}, \{\Omega_j\}_{j \leq \ell})$}
    \ForAll{$t \gets 1$ \To $n$}
    \State $\Pi^{(q_t)}_1(t) \triangleq \sum_{k \in \calL_{t, 1}}\hat K_{i, t} -\left( \sum_{k \notin \calL_{t, 1}}\hat K_{i, k} \right)\frac{1}{\ell - 1}.$
    \State $
    \tilde b_{t, q_t} = \left\{\begin{array}{ll}
    1 & \mbox{ if } \Pi^{(q_t)}_1(t) \geq \frac{c}{\log d}\sqrt{\frac{d}{\ell}} \\
    -1 & \mbox{ if } \Pi^{(q_t)}_1(t) <- \frac{c}{\log d}\sqrt{\frac{d}{\ell}} \\
    0 & \mbox{otherwise}.
    \end{array}
    \right.$
    \State $\hat L_{(t, q_t), j} += \hat K_{q_t, k}$
    \EndFor 
    \State \Return{$\mu_1 = \frac{\sum_{t \leq n}\tilde b_{t, q_t}\my_{t, q_t}}{\sum_{t \leq n}\tilde b_{t, q_t}\Pi^{(q_t)}_1(t)}$}
    \EndProcedure
\end{algorithmic}
\end{algorithm}



\begin{algorithm}[t!]
    \caption{Our algorithm for Linear Boosting. {\color{orange} moved from text}}\label{fig:linearboost1}
    \hspace*{\algorithmicindent} \textbf{Input} $\mX$, $\mY$, $\hat K$, $\eta$\\
    \hspace*{\algorithmicindent} \textbf{Output}  $\{g_k(\cdot)\}_{k \leq b}$
    \begin{algorithmic}[1]
    \Procedure{$\proc{Boosting-Algorithm}$}{$\mY$, $\mX$, $\hat K$, $\eta$}
    \State $\mY_{\Res} \gets \mY$. 
    \Comment $\eta$ is the learning rate.
    \ForAll{$k \gets 1$ \To $b$}
    \State $g_k \gets \proc{Linear-Fit}(\mY_{\Res}, \mX)$.
    \State $(\hat \mY)_{k} \gets \hat K g_{k}(\mX)$.
    \State $\mY_{\Res} \gets \mY_{\Res} - \eta (\hat \mY)_{k}$. 
    \EndFor
    \State \Return $\{g_k(\cdot)\}_{k \leq b}$
    \EndProcedure
    \Procedure{$\proc{Linear-Fit}$}{$\mY$, $\mX$, $\hat K$}
    \Comment Let $\mx_{t, i},\mf_{t, i} \in \reals^k$.
    \ForAll{$i \gets 1$ \To $n$}
    \State $\mf_{t,i} = \sum_{j \in [d]}\hat K_{i, j}\mx_{t, j}$.
    \EndFor
    \ForAll{$j\gets 1$ \To $k$}
    \State $r_j = \sum_{t \leq n}\mathrm{Corrcoef}(\left(\mf_{t, :}\right)_{j}, \my_{t,:})$.
    \EndFor
    \State Let $j_1, j_2, j_3$ be the indices with the largest $r_j$. 
    \State $g(\cdot) = \arg \min_{\beta_1, \dots, \beta_6}\sum_{\substack{t \leq n \\ i \in [d]}}\left(\my_{t, i} - \sum_{j \in [d]}\hat K_{i,j}\left(\beta_1 (\mx_{t, i})_{j_1} + \dots + \beta_6(\mx_{t, i})_{j_2}\cdot (\mx_{t, i})_{j_3})\right)\right)^2$.
    \State \Return $g(\cdot)$
    \EndProcedure
\end{algorithmic}
\end{algorithm}

\begin{algorithm}[t!]
    \caption{Our algorithm for estimating $g(\cdot)$ {\color{orange} moved from text} }\label{fig:estimateg1}
    \hspace*{\algorithmicindent} \textbf{Input} $\mX$, $\mY$, $\hat K$, $\{\Omega_i\}_{i \leq \ell}$\\
    \hspace*{\algorithmicindent} \textbf{Output}  $\{\mu_j\}_{j \leq \ell}$
    \begin{algorithmic}[1]
    \Procedure{$\proc{Estimate-g}$}{$\hat K, \{\Omega_j\}_{j \leq \ell}, \mX, \mY$}
    \ForAll{$t \gets \text{1 to n}$}
    \State $\mx_t = \mX_{t, :}$, $\my_t = \mY_{t, :}$, and $q_t \gets Rand(d)$
    \State $\hat L_t = \proc{Reduce-to-Regression}(\hat K, \mx_t, \{\Omega_j\}_{j \leq \ell}, q_t)$
    \EndFor
    \State $\mu_1, \dots \mu_{\ell} \gets$ $\proc{Solve-Regression}$ $(\{\my_t, \hat L_t\}_{t \leq n})$
    \State \Return $\mu_1, \dots \mu_{\ell}$
    \EndProcedure
    
    \Procedure{$\proc{Reduce-to-Regression}$}{$\hat K, \mx_t, \{\Omega_j\}_{j \leq \ell}), q_t$} 
    %\Comment Reduce original problem into the regression problem for $\mu_j$'s.
    \State Let $\hat L_{(t, q_t), j} = 0$ 
    \ForAll{$k \gets 1$ \To $d$}
    \State Find $\Omega_j$ such that $\mx_{t, k} \in \Omega_j$
    \State $\hat L_{(t, q_t), j} +=\hat  K_{q_t, k}$
    \EndFor
    \State \Return $\hat L_t$
    \EndProcedure
    
    \Procedure{$\proc{Solve-Regression}$}{$(\{\my_t, \hat L_t\}_{t \leq n})$}
    \ForAll{$t \gets 1$ \To $n$}
    \State $\Pi^{(q_t)}_1(t) \triangleq \sum_{j \in \calL_{t, 1}}\hat L_{(t,q_t), j} -\frac{1}{\ell - 1}\left( \sum_{j \notin \calL_{t, 1}}\hat L_{(t,q_t), j} \right).$
    \State $
    \tilde b_{t, q_t} = \left\{\begin{array}{ll}
    1 & \mbox{ if } \Pi^{(q_t)}_1(t) \geq \frac{c}{\log d}\sqrt{\frac{d}{\ell}} \\
    -1 & \mbox{ if } \Pi^{(q_t)}_1(t) <- \frac{c}{\log d}\sqrt{\frac{d}{\ell}} \\
    0 & \mbox{otherwise}.
    \end{array}
    \right.$
    \EndFor 
    \State \Return{$\mu_1 = \frac{\sum_{t \leq n}\tilde b_{t, q_t}\my_{t, q_t}}{\sum_{t \leq n}\tilde b_{t, q_t}\Pi^{(q_t)}_1(t)}$}
    \EndProcedure
\end{algorithmic}
\end{algorithm}
\begin{algorithm}[t!]
    \caption{Our algorithm for estimating $K$ {\color{orange} moved from text}}\label{fig:estimatek1}
    \hspace*{\algorithmicindent} \textbf{Input} $\mX, \mY$\\
    \hspace*{\algorithmicindent} \textbf{Output} $\hat K$
    \begin{algorithmic}[1]
    \State $[V, \Sigma, V^{\transpose}] = \mathrm{svd}\left(\frac 1 n\mY^{\transpose}\mY\right)$
    \State Let $\sigma_i = \Sigma_{i,i}$ 
    \State  $i^* = \max \{\lambda_{i^*} - \lambda_{i^*+1} \geq \delta d^2\}$.\Comment{$\delta$ a tunable parameter}
    \State \Return $\hat K = \calP_{i^*}(V\Sigma^{\frac 1 2}V^{\transpose})$
    \end{algorithmic}
\end{algorithm}

While non-parametric methods can handle constant size features and have high interpretability, we may use deep learning models to learn $g(\cdot)$. The deep learning models are capable 
of handling a large number of features at the cost of having reduced interpreability and performance guarantee. We shall aim to learn the function $g(\cdot)$ via minimizing the MSE
\begin{equation}
    \min_{g(\cdot)} \sum_{t \leq n}\|\my_t - K g(\mx_t)\|^2_2. 
\end{equation}
We shall consider the following deep learning architecture: 
\begin{itemize}
    \item \emph{Multi-layer perceptrons.} This model uses multi-layer perceptrons to represent $g(\cdot)$.  Multi-layer perceptrons are neural networks that consist of multiple fully connected layers. {\color{red} See Fig. X}. {\color{blue}  Question for Qiong: maybe describe the hyper-parameters? }
    
    \item \emph{Recurrent neural nets (LSTM).}  We also examine using recurrent neural nets to extract potential serial dependencies of the return series {\color{blue} be careful; this sentence could be problematic.}. We examine LSTM, with a standard way to feed the features into LSTM~\cite{hochreiter1997long}
    {\color{blue} is this a standard reference for LSTM?} We
    do not report results from other RNN because their performances are similar. 
    
    The Long Short Term Memory(LSTM) based price prediction mode is one of the state-of-the-art baselines. This model is proposed by~\cite{nelson2017stock} and operates on the sequential indicators, which enables it to capture the long-term dependency of stock prices at different moments. {\color{blue} Question for Qiong: why we don't use other RNN? Maybe just the performance are similar? Do we need to describe LSTM at this level of details?}
    
    \qq{It is natural to use LSTM on the sequential market states for prediction since
    LSTM has been widely used in conduct sequential prediction\cite{nelson2017stock,gao2016stock,rather2015recurrent,zhang2017stock}. 
    LSTM is a type of recurrent neural network CITE. The advantage of LSTM over vanilla RNN is that it allows memory cells to store and access information over long periods
    and able to avoid the vanishing and exploding gradient problems. Moreover, LSTM usually achieves competitive performance compared to other RNN  variants. CITE
    } 
\end{itemize}

This section introduces the implementation details about partition method.
We use the Chinese equity market data from the start of year 2013 to the end of year 2018. Since this is a time series dataset, we creates sliding windows from the input data. The size of the training window is 3 years and the size of the test window is the following 1 year. We set a gap of 21 trading days (1 month) between the training window and test window to avoid look ahead issue. For the next training - test fold, the training and the test windows are shifted to 1 year later. In summary, we have year 2016, 2017 and 2018 as our test years. We test our model in two different universe of stocks, one is 800 and one is 3000.{ \color{orange} Need to specify what are these universes.} 

We prepare a set of 337 factors as the input feature $X$ for all stocks in our universe daily. Then we carefully perform a daily normalization technique to each factor to transform the distribution of factor to gaussian distribution. We set next 5 days return as the response of our model. For evaluation metrics, we use average and t-statistic on daily correlation. Besides, to avoid our model mostly rely on low liquidity equities in market, we also compute the average and t-statistic on liquidity weighted daily correlation, where the weight is set as the last 21 days turnover. 

For partition algorithm, we apply a forecasting model based on each factor first for model simplicity. In total we have 337 forecasts from all factors. Then we combined all the forecasting power together by using a t-statistic weighted summation on all forecasts from factors. {\color{orange} This part is pretty rough that I need to polish it carefully. I can not use too many words to specify this part. But I need to make this part clear and understandable.} In detail, we have one forecast for one factor model $[\my_{t,i}]_{q}=\sum_{j\leq d}{K_{j,i}g([\mx_{t,i}]_{q})}$ {\color{orange} Kind of running out of usable notation.}, here $q$ is an integer to denote the index of factor while $q\in [1,k]$, $k$ is the number of our features. We do a weighted sum on all feature forecast $[\my_{t,i}]_{q}$ by the weight of t-statistic of in sample daily correlation. Finally we have one combined forecast for each stock daily. However, not all factors can have a better performance after adding distance.{ \color{orange} I need to think very carefully about how to avoid attacking on this sentence. This looks vulnerable now.} We perform a `pre-checking' process in the training stage. Since each factor can have two forecasts $[\my_{t,i}]_{q, with distance}$ and $[\my_{t,i}]_{q, without distance}$, one from adding distance and the other from non-distance version. We can check the in sample daily correlation difference between two models. We will use the one with a better in sample performance.{ \color{orange} need to be more clear here.} In summary, we will have two sets of factor forecasts $S_1 = \{[\my_{t,i}]_{q, with distance}, where (corr([\my_{t,i}]_{q, with distance}) - corr([\my_{t,i}]_{q, without distance}) > 8e^{-3}) \& (corr([\my_{t,i}]_{q, without distance}) > -8e^{-3})\}$ and $S_2 = \{[\my_{t,i}]_{q, without distance}, rest of factors\}$. Finally we combine these two sets together to calculate for the final combined forecast. { \color{orange} Maybe we can put this part in appendix? kind of too messy. I don't think about a good way to do it clear now.}

For linear boosting algorithm, we deployed a similar feature selection way. First we select the part of factors that can be improved with neighbor.{\color{orange}give more details here.} Then we build a linear boosting model with neighbor on this part of factors. To utilizing all the forecasting power of our factors, we also build another linear boosting model based on the rest of features. Finally we combined these two models weighted by the t-stat of in sample daily correlation

\myparab{Comparisons and messages.} Our algorithms does not introduce new techniques/tricks for training DL. We \emph{simplify} recent architectures based on stock embeddings by using our stand-alone provable procedures to learn stocks' latent positions {\color{red} add figure}. We shall see in Sec. XX that our simplified architecture have better performance and reduced running time compared to prior related algorithms. CITE. {\color{red} sufficient details?}
{\color{blue} move around.}


There are two key differences between this model and the cross-sectional linear models: \emph{(i)} the learnable parameter forms a matrix. Information from stock $i$ can be used as a signal to forecast return of stock $j$. In AR1, for example, the past return of stock $i$ is a covariate of the future return of stock $j$. \emph{(ii)} The size of learnable parameters becomes significantly larger. Using the AR1 example again, when the number $d$ of stocks is $3,000$, the size of $M$ is $3k \times 3k \approx 1$ million. In these cases, regularizations are needed to secure out-of-sample forecasting power. 
\begin{table}[ht!]
\small
\begin{adjustbox}{width=0.8\columnwidth,center}
\centering
\begin{tabular}{|l|l|l|l|l|l|l|l|l|l|l|l|}
\hline
\multicolumn{2}{|l|}{\multirow{2}{*}{Models}} & \multicolumn{4}{l|}{raw return}   & \multicolumn{4}{l|}{adjust return} & \multicolumn{2}{l|}{Profit} \\ \cline{3-12} 
\multicolumn{2}{|l|}{}     & corr   & w\_corr & t-stat & w\_t-stat & corr   & w\_corr & t-stat  & w\_t-stat & pnl    & sharp  \\ \hline
\multirow{3}{*}{Boosting}  & Optimized neighbor        & 0.0764 & 0.0936  & 6.7939 & 6.3362    & 0.0676 & 0.0883  & 8.4587  & 7.2296    & 0.3833 &	8.4073 \\ \cline{2-12} 
                           & Neighbor with data driven & 0.0692 & 0.0874  & 6.3141 & 5.8140    & 0.0665 & 0.0879  & 8.5304  & 7.2582    & 0.3519 &  7.7530 \\ \cline{2-12} 
                           & No neighbor               & 0.0674 & 0.0866  & 6.0947 & 5.7312    & 0.0649 & 0.0872  & 8.3500  & 7.1282    & 0.3405 &  7.3344 \\ \hline
\multirow{3}{*}{Partition} & Best results              & 0.0446 & 0.0320  & 3.2961 & 1.5753    & 0.0361 & 0.0335  & 3.7171  & 2.3454    & 0.1981 &  3.8347 \\ \cline{2-12} 
                           & Neighbor with data driven & 0.0445 & 0.0307  & 3.2781 & 1.5399    & 0.0360 & 0.0340  & 3.6550  & 2.3571    & 0.1988 &  3.8511\\ \cline{2-12} 
                           & No neighbor               & 0.0432 & 0.0309  & 3.1505 & 1.4912    & 0.0229 & 0.0336  & 2.4520  & 2.8195    & 0.1883 &  3.5370\\ \hline
\multirow{3}{*}{MLP}       & Best results              & 0.0550 & 0.0567  & 6.4782 & 5.0172    & 0.0450 & 0.0540  & 7.0786  & 6.0621    & 0.2682 & 5.6809 \\ \cline{2-12} 
                           & Neighbor with data driven & 0.0540 & 0.0562  & 6.4396 & 4.9953    & 0.0437 & 0.0525  & 6.5941  & 5.7666    & 0.2591 & 5.4195 \\ \cline{2-12} 
                           & No neighbor               & 0.0507 & 0.505   & 6.0234 & 4.4966    & 0.0424 & 0.0459  & 6.6923  & 5.1343    & 0.2556 &	5.3963\\ \hline
\multirow{3}{*}{LSTM}      & Best results              & 0.0286 & 0.0347  & 3.4517 & 3.0261    & 0.0250 & 0.0406  & 3.7566  & 4.5594    & 0.1415 &3.6961  \\ \cline{2-12} 
                           & Neighbor with data driven &  0.0231&	0.0352	&2.6108	&2.9779    & 0.0196		&0.033	&	2.9315	&	3.4961 &0.0903 & 2.1206   \\ \cline{2-12} 
                           & No neighbor               & 0.0178 & 0.0200  & 2.2136 & 1.8077    &0.0172 & 	0.0300 & 	2.5049	 & 3.1426   & 0.0812&	2.2245       \\ \hline
\multirow{3}{*}{Linear(Q)}   & Best results   & 0.0449 & 0.0517 & 4.8020 & 4.5514 & 0.0359  & 0.0407 & 5.3930 & 4.4816 & 0.2224	& 4.3217       \\ \cline{2-12} 
                           & Lasso                     & 0.0106 & 0.0192  & 1.6471 & 2.3030    & 0.0107 & 0.0153  & 2.0325  & 2.0107    & 0.0733&	1.7489 \\ \cline{2-12} 
                           & Ridge                     & 0.0247	& 0.0246 &2.3553 &1.9628  &0.0305&	0.0377	&4.486	&4.2442 & 0.1186	&1.9513\\ \hline
\multicolumn{2}{|l|}{ML: GBRT}                         & 0.0516 & 0.0591  & 7.5739 & 5.6310    & 0.0652 & 0.0666  & 10.0494 & 5.7849    & 0.2543 & 9.1759  \\ \hline
\multicolumn{2}{|l|}{DL: SFM}                          & 0.0027 & 0.0032  & 0.4688 & 0.405     & 0.0059 & 0.0024  & 1.2083  & 0.3488    &   0.0750&	1.8050	      \\ \hline
\multicolumn{2}{|l|}{DL: Alpha}                        & 0.0085 & 0.0063 & 2.1045 & 1.2516   & 0.0114 & 0.0115  & 0.7202  & 0.6734    & 0.0420	 & 1.7622       \\ \hline
\multicolumn{2}{|l|}{DL: HAN}                          & 0.0028 & -0.0037 & 0.6901 & -0.6084   & 0.0045 & 0.0005  & 1.4521  & 0.1179    &   0.0043 &	0.1651       \\ \hline
\multicolumn{2}{|l|}{Consolidate: Neighbor}            & 0.0775 & 0.0950  & 6.8687 & 6.4108    & 0.0681 & 0.0886  & 8.4995  & 7.2485    &   0.3855     &   8.3218     \\ \hline
\end{tabular}
\end{adjustbox}
\caption{The table in the main part,800}
\end{table}


\begin{table}[ht!]
\small
\begin{adjustbox}{width=0.8\columnwidth,center}
\centering
\begin{tabular}{ll|l|l|l|l|l|l|l|l|l|l}
\hline
\multicolumn{2}{l}{\multirow{2}{*}{Models}}                                 & \multicolumn{4}{l|}{raw return}       & \multicolumn{4}{l|}{adjust return}     & \multicolumn{2}{l|}{Profit} \\ \cline{3-12} 
\multicolumn{2}{l}{}                            & corr   & w\_corr & t-stat & w\_t-stat & corr   & w\_corr & t-stat  & w\_t-stat & pnl          & sharp        \\ \hline
\multicolumn{1}{l|}{\multirow{3}{*}{Boosting}}  & Optimized neighbor        & 0.0944 & 0.1009  & 8.2607 & 6.4435    & 0.0820 & 0.0951  & 10.2551 & 8.4881    & 0.5261       & 10.9728      \\ \cline{2-12} 
\multicolumn{1}{l|}{}                           & Neighbor with data driven & 0.0934 & 0.1000  & 9.0551 & 6.9076    & 0.0817 & 0.0954  & 10.2386 & 8.5358    & 0.5181       & 11.8055      \\ \cline{2-12} 
\multicolumn{1}{l|}{}                           & No neighbor               & 0.0827 & 0.0884  & 7.4297 & 5.6659    & 0.0766 & 0.0898  & 9.1907  & 7.7917    & 0.4565       & 9.7692       \\ \hline
\multicolumn{1}{l|}{\multirow{3}{*}{Partition}} & Best results              & 0.0618 & 0.0553  & 5.7327 & 3.5212    & 0.0339 & 0.0437  & 4.4609  & 3.9459    & 0.3386       & 7.5921       \\ \cline{2-12} 
\multicolumn{1}{l|}{}                           & Neighbor with data driven & 0.0603 & 0.0507  & 5.0648 & 3.0551    & 0.0333 & 0.0430  & 4.4181  & 3.9586    & 0.3330       & 7.0454       \\ \cline{2-12} 
\multicolumn{1}{l|}{}                           & No neighbor               & 0.0584 & 0.0509  & 5.0098 & 3.0844    & 0.0332 & 0.0427  & 4.3958  & 3.9260    & 0.3070       & 6.5996       \\ \hline
\multicolumn{1}{l|}{\multirow{3}{*}{MLP}}       & Best results              & 0.0738 & 0.0692  & 9.2034 & 6.4151    & 0.0576 & 0.0615  & 9.9377  & 7.7624   & 0.4202 & 9.4349             \\ \cline{2-12} 
\multicolumn{1}{l|}{}                           & Neighbor with data driven & 0.0671 & 0.0640  & 8.9526 & 6.1564    & 0.0560 & 0.0588  & 9.5861  & 7.5261    &  0.3493 & 8.1658               \\ \cline{2-12} 
\multicolumn{1}{l|}{}                           & No neighbor               & 0.0606 & 0.0467  & 8.2857 & 4.4555    & 0.0510 & 0.0546  & 8.9825  & 7.1801    &  0.2782 & 6.3847             \\ \hline
\multicolumn{1}{l|}{\multirow{3}{*}{LSTM}}      & Best results               & 0.0473 & 0.0491 & 6.3615 & 4.2385 & 0.0431 & 0.0554 & 7.4720 & 7.2205 & 0.2487 & 7.1084     \\ \cline{2-12} 
\multicolumn{1}{l|}{}                           & Neighbor with data driven & 0.0415 & 0.0429 & 6.0979 & 4.0582 & 0.0429 & 0.0526 & 8.8588 & 7.3113 & 0.2012 & 5.6228         \\ \cline{2-12} 
\multicolumn{1}{l|}{}                           & No neighbor                & 0.0352 & 0.0297 & 4.0602 & 2.3619 & 0.0401 & 0.049  & 7.3926 & 6.6228 & 0.175  & 4.334             \\ \hline
\multicolumn{1}{l|}{\multirow{3}{*}{Linear(Q)}} & Best results              & 0.0548 & 0.0560  & 6.3589 & 4.9856    & 0.0451 & 0.0562  & 6.6027  & 6.5757    &   0.3218 & 6.478                \\ \cline{2-12} 
\multicolumn{1}{l|}{}                           & Lasso                     & 0.0290 & 0.0251  & 4.4711 & 2.6010    & 0.0289 & 0.0333  & 6.400   & 5.2190    &  0.1888 & 4.7914              \\ \cline{2-12} 
\multicolumn{1}{l|}{}                           & Ridge                     & 0.0358 & 0.0406  & 4.5172 & 3.6941    & 0.0363 & 0.0428  & 5.3988  & 5.2386    &         0.1839 & 3.98              \\ \hline
\multicolumn{2}{l|}{ML: GBRT}                                               & 0.0673 & 0.0747  & 9.3379 & 7.8931    & 0.0862 & 0.0922  & 15.7695 & 10.4105   & 0.3858       & 4.4517       \\ \hline
\multicolumn{2}{l|}{DL: Alpha}                                              & 0.0147 & 0.0051  & 1.2683 & 0.3892    & 0.0121 & 0.0037  & 1.1642  & 0.3187    & 0.0169       & 0.5464       \\ \hline
\multicolumn{2}{l|}{DL: SFM}                                            & 0.0027 &  0.0032 &  0.4688 &     0.4050    & 0.0059 & 0.0024 & 1.2083  & 0.3488    & 0.0045 &  0.1065      \\ \hline
\multicolumn{2}{l|}{DL: HAN}                                                & 0.0015 & 0.0118  & 0.4236 & 2.1548    & 0.0012 & 0.0084  & 0.3936  & 1.7602    &   0.0016	&0.0473           \\ \hline
\multicolumn{2}{l|}{Consolidate: Neighbor}                                  & 0.0958 & 0.1025  & 8.5703 & 6.6487   & 0.0819 & 0.0959  & 10.2067 & 8.5112    &  0.5346    &   11.3046           \\ \hline
\end{tabular}
\end{adjustbox}
\caption{The table in the main part,3000}
\end{table}


\begin{table}[ht!]
\begin{adjustbox}{width=0.8\columnwidth,center}
\begin{tabular}{|l|l|l|l|l|l|l|l|l|l|l|l|l|l|}
\hline
Method &
   &
  2016\_corr &
  2016\_w\_corr &
  2016\_t-stat &
  2016\_w\_t-stat &
  2017\_corr &
  2017\_w\_corr &
  2017\_t-stat &
  2017\_w\_t-stat &
  2018\_corr &
  2018\_w\_corr &
  2018\_t-stat &
  2018\_w\_t-stat \\ \hline
  
  
GBL    & Optimized    &     0.1102 &       0.1105 &      12.7957 &         9.4390 &     0.0723 &       0.0844 &       8.9903 &         7.3310 &     0.0634 &       0.0905 &       8.9792 &         8.6941   \\\hline
GBL    & Data      &   0.1107 &       0.1113 &      12.9251 &         9.5677 &     0.0719 &       0.0836 &       8.9219 &         7.2237 &     0.0624 &       0.0914 &       8.8689 &         8.8160 \\\hline
GBL & No neighbor &     0.1042 &       0.1036 &      11.6317 &         8.6149 &     0.0675 &       0.0772 &       8.0083 &         6.5935 &     0.0582 &       0.0887 &       7.9321 &         8.1666 \\\hline
Partition & Optimized &       0.0683 &       0.0680 &       6.7174 &         5.3683 &     0.0143 &       0.0217 &       2.2734 &         1.9366 &     0.0191 &       0.0412 &       4.3920 &         4.5327 \\\hline
Partition & Data &    0.0683 &       0.0682 &       6.7453 &         5.3980 &     0.0139 &       0.0215 &       2.2403 &         1.9252 &     0.0177 &       0.0393 &       4.2686 &         4.5527 \\\hline
Partition & No neighbor &      0.0681 &       0.0679 &       6.7199 &         5.3754 &     0.0138 &       0.0212 &       2.2105 &         1.8894 &     0.0177 &       0.0390 &       4.2569 &         4.5133 \\\hline
  
MLP    & Optimized   & 0.0789 & 0.0776 & 6.8391 & 5.8248 & 0.0408 & 0.0453 & 4.4891 & 3.2911 & 0.0531 & 0.0616 & 9.6439 & 5.5921 \\ \hline
MLP    & Data        & 0.0730 & 0.0728 & 6.2636 & 5.4889 & 0.0441 & 0.0458 & 4.7645 & 3.3034 & 0.0508 & 0.0579 & 8.0554 & 5.2430 \\ \hline
MLP    & No neighbor & 0.0724 & 0.0696 & 6.1909 & 5.2321 & 0.0397 & 0.0448 & 4.4849 & 3.2059 & 0.0408 & 0.0493 & 8.6270 & 5.4372 \\ \hline
LSTM   & Optimized   & 0.0568 & 0.0570 & 4.9664 & 4.0557 & 0.0478 & 0.0584 & 5.3133 & 4.7910 & 0.0245 & 0.0510 & 3.9122 & 4.3118 \\ \hline
LSTM   & Data        & 0.0441 & 0.0479 & 6.0089 & 4.8630 & 0.0497 & 0.0527 & 5.6341 & 4.2197 & 0.0350 & 0.0570 & 4.6902 & 4.4317 \\ \hline
LSTM   & No neighbor & 0.0536 & 0.0535 & 4.9642 & 4.0641 & 0.0505 & 0.0588 & 5.9703 & 4.4946 & 0.0161 & 0.0347 & 3.5111 & 3.6958 \\ \hline
GBRT & No neighbor & 0.1103 &       0.1115 &      20.1555 &        13.2341 &     0.0821 &       0.0811 &      14.6572 &         9.4954 &     0.0662 &       0.0839 &      12.4958 &         8.5020  \\ \hline
Linear & Optimized   & 0.0668 & 0.0673 & 5.3072 & 4.6795 & 0.0308 & 0.0313 & 2.8023 & 2.1256 & 0.0378 & 0.0702 & 4.3575 & 5.8719 \\ \hline
Lasso  & No neighbor & 0.0344 & 0.0369 & 4.6964 & 4.0490 & 0.0360 & 0.0373 & 3.7746 & 2.6650 & 0.0162 & 0.0258 & 4.7343 & 3.6365 \\ \hline
Ridge  & No neighbor & 0.0664 & 0.0675 & 5.2647 & 4.6993 & 0.0400 & 0.0413 & 3.5950 & 2.7889 & 0.0025 & 0.0194 & 0.5023 & 2.1586 \\ \hline
SFM  &  & 0.039 & 0.0412 & 4.0343 & 3.2286 & 0.0054 & 0.0101 & 0.6339 & 0.9499 & 0.0104 & 0.0201 & 1.4257 & 1.822\\\hline
Alpha &  & 0.0106 &       0.0091 &       2.2448 &         1.7491 &     0.0119 &       0.0079 &       3.8844 &         2.1731 &    -0.0037 &      -0.0008 &      -1.3122 &        -0.2159  \\ \hline
\end{tabular}
\end{adjustbox}
\caption{3000, adj by year}
\end{table}




\begin{table}[ht!]
\begin{adjustbox}{width=0.8\columnwidth,center}
\begin{tabular}{|l|l|l|l|l|l|l|l|l|l|l|l|l|l|}
\hline
Method &
   &
  2016\_corr &
  2016\_w\_corr &
  2016\_t-stat &
  2016\_w\_t-stat &
  2017\_corr &
  2017\_w\_corr &
  2017\_t-stat &
  2017\_w\_t-stat &
  2018\_corr &
  2018\_w\_corr &
  2018\_t-stat &
  2018\_w\_t-stat \\ \hline




GBL    & Optimized    &     0.0909 &       0.1045 &      12.0192 &         8.8934 &     0.0529 &       0.0707 &       6.1165 &         5.2288 &     0.0590 &       0.0896 &       7.2402 &         7.5667 \\\hline
GBL    & Data      &    0.0903 &       0.1042 &      12.2675 &         9.0455 &     0.0490 &       0.0684 &       5.6019 &         4.8668 &     0.0602 &       0.0910 &       7.7218 &         7.8623  \\\hline
GBL & No neighbor &     0.0903 &       0.1043 &      12.2679 &         9.0450 &     0.0537 &       0.0710 &       6.3276 &         5.1011 &     0.0507 &       0.0864 &       6.4546 &         7.2384 \\\hline
Partition & Optimized &      0.0537 &       0.0435 &       5.1136 &         2.7487 &     0.0129 &       0.0186 &       1.4095 &         1.4000 &     0.0417 &       0.0384 &       4.6283 &         2.8875 \\\hline
Partition & Data &   0.0534 &       0.0439 &       5.0507 &         2.7682 &     0.0123 &       0.0168 &       1.3011 &         1.2607 &     0.0422 &       0.0414 &       4.6131 &         3.0424  \\\hline
Partition & No neighbor &       0.0498 &       0.0536 &       4.5738 &         3.8038 &     0.0096 &       0.0213 &       1.0684 &         1.7055 &     0.0093 &       0.0258 &       1.7139 &         2.9493  \\\hline

MLP    & Optimized   & 0.0686 & 0.0674 & 6.3348 & 4.5279 & 0.0218  & 0.0315  & 2.1049  & 2.0044  & 0.0466  & 0.0600 & 5.7584  & 4.6373 \\ \hline
MLP    & Data        & 0.0653 & 0.0667 & 5.4364 & 4.3428 & 0.0239  & 0.0302  & 2.2594  & 1.8829  & 0.0418  & 0.0607 & 4.8780  & 4.6655 \\ \hline
MLP    & No neighbor & 0.0657 & 0.0634 & 5.9057 & 4.2169 & 0.0225  & 0.0264  & 2.2156  & 1.6916  & 0.0391  & 0.0478 & 4.6646  & 3.7121 \\ \hline
LSTM   & Optimized   & 0.0453 & 0.0517 & 3.6015 & 3.0878 & 0.0107  & 0.0262  & 0.9938  & 1.7157  & 0.0189  & 0.0438 & 2.3895  & 3.5942 \\ \hline
LSTM   & Data        & 0.0338 & 0.0414 & 2.7206 & 2.4910 & 0.0070  & 0.0118  & 0.6251  & 0.6803  & 0.0180  & 0.0460 & 2.1391  & 3.7375 \\ \hline
LSTM   & No neighbor & 0.0360 & 0.0425 & 2.8522 & 2.5619 & -0.0009 & 0.0027  & -0.0770 & 0.1536  & 0.0166  & 0.0449 & 1.9563  & 3.6240 \\ \hline

GBRT & No neighbor  &     0.0727 &       0.0746 &      11.8015 &         6.1850 &     0.0639 &       0.0763 &      11.2264 &         6.4979 &     0.0589 &       0.0489 &       7.1202 &         4.6718 \\ \hline
Linear & Optimized   & 0.0451 & 0.0524 & 3.2813 & 3.0374 & 0.0374  & 0.0499  & 3.6260  & 3.4670  & 0.0252  & 0.0197 & 3.3796  & 1.6104 \\ \hline
Lasso  & No neighbor & 0.0418 & 0.0477 & 4.3591 & 3.6496 & -0.0083 & -0.0262 & -1.1474 & -2.1270 & -0.0013 & 0.0244 & -0.1903 & 2.5165 \\ \hline
Ridge  & No neighbor & 0.0454 & 0.0528 & 3.3240 & 3.0684 & 0.0206  & 0.0291  & 1.7709  & 1.8791  & 0.0255  & 0.0310 & 4.1090  & 3.1694 \\ \hline
SFM & &0.0334 & 0.04 & 2.8564 & 2.6317 & -0.0083 & -0.0078 & -0.86 & -0.5632 & -0.0409 & 0.0075 & -3.7163 & 0.6063\\ \hline
Alpha & & 0.0049 & 0.0061 & 0.9505 & 0.7321 & 0.0052 & 0.0018 & 1.1437 & 0.2035 & 0.0016 & 0.006 & 0.394 & 0.8429\\ \hline
\end{tabular}
\end{adjustbox}
\caption{800,adj, by year}
\end{table}

\begin{figure}[!htb]
\minipage{0.32\textwidth}
  \includegraphics[width=\linewidth]{figures/LI800adj.png}
\endminipage\hfill
\minipage{0.32\textwidth}
  \includegraphics[width=\linewidth]{figures/LS800radj.png}
\endminipage\hfill
\minipage{0.32\textwidth}%
  \includegraphics[width=\linewidth]{figures/LSW800adj.png}
\endminipage
\caption{Universe 800, adj return}
\end{figure}

\begin{figure}[!htb]
\minipage{0.32\textwidth}
  \includegraphics[width=\linewidth]{figures/LI3000adj.png}
\endminipage\hfill
\minipage{0.32\textwidth}
  \includegraphics[width=\linewidth]{figures/LS3000radj.png}
\endminipage\hfill
\minipage{0.32\textwidth}%
  \includegraphics[width=\linewidth]{figures/LSW3000adj.png}
\endminipage
\caption{Universe 3000, adj return}
\end{figure}


\begin{figure}[!htb]
\minipage{0.32\textwidth}
  \includegraphics[width=\linewidth]{figures/LI800raw.png}
\endminipage\hfill
\minipage{0.32\textwidth}
  \includegraphics[width=\linewidth]{figures/LS800raw.png}
\endminipage\hfill
\minipage{0.32\textwidth}%
  \includegraphics[width=\linewidth]{figures/LSW800raw.png}
\endminipage
\caption{Universe 800, raw return}
\end{figure}
\begin{figure}[!htb]
\minipage{0.32\textwidth}
  \includegraphics[width=\linewidth]{figures/LI3000raw.png}
\endminipage\hfill
\minipage{0.32\textwidth}
  \includegraphics[width=\linewidth]{figures/LS3000raw.png}
\endminipage\hfill
\minipage{0.32\textwidth}%
  \includegraphics[width=\linewidth]{figures/LSW3000raw.png}
\endminipage
\caption{Universe 3000, raw return}
\end{figure}

\begin{table}[ht!]
  %\caption{The comparison between algorithms}
  \centering
  \label{tbl:excel-table}
  \includegraphics[width=0.5\linewidth]{figures/table_compare2.pdf}
\caption{Explain why different settings may need different models.}
\vspace{-0.5cm}
\label{fig:compare1}
\end{table}
\begin{figure}[ht!] 
    \centering
    \vspace{-0.4cm}
    \includegraphics[width=0.7\textwidth]{figures/algorithm/graph_for_algorithm1_crop.pdf} 
    %\label{fig:by:table} 
  \vspace{-0.6cm}
  \caption{Translating the stock embedding problem into a regression problem: The original $\mx \in [-1,1]$ is partitioned into $\ell=10$ uniform subsets while variables $\mu_1,\dots,\mu_{10}$ are assigned to $g(\cdot)$ for each subset.}
  \label{fig:partition1}
  \vspace{-0.2cm}
\end{figure}


\begin{figure}[htbp]
\centering
\includegraphics[scale=0.45]{figures/algorithm/graph_for_algorithm2_combine.pdf}
\caption{Framework for linear boosting algorithm. (Left) Workflow for one linear base learner. (Right) Boosting process. \qq{Why we only pick 6 terms in total.}}
\label{fig:linear_boost_algorithm1}
\end{figure}
\begin{figure*}[t!] 
  %\centerline
    {\includegraphics[width=1.0\textwidth]{figures/table_1_1/partition/table_1_crop.pdf} }
  \vspace{-0.6cm}
  \caption{Improving forecasting power by the stock latent space model {\color{red} check the model name}.}
  \label{partitionfix1}
  \vspace{-0.3cm}
\end{figure*}

\begin{table}[ht!]
\centering

\begin{tabular}{l|l|l}
\hline
Method    & \multicolumn{2}{l}{Explanation}                      \\ \hline
Boosting  & \multicolumn{2}{l}{Linear boosting (ours)}           \\ \hline
Partition & \multicolumn{2}{l}{Partitioning algorithm (ours)}    \\ \hline
MLP       & \multicolumn{2}{l}{Multiple layer perceptron (ours)} \\ \hline
GBRT      & \multicolumn{2}{l}{Gradient Boost Regression Tree}   \\ \hline
\end{tabular}
\caption{Explanation of methods}
\end{table}
\iffalse

\subsubsection{Hyper parameters}

We summarize the hyperparameters for all models as follows:

\myparab{Hyper parameters for generating $\hat K$}

\emph{$\hat K$ from Data driven approach:} the $k$ for low rank approximation: [10, 20, 50]

\emph{Hyper $\hat K$:} [Barra distance, Barra inner product, Barra distance  + news, Barra inner product + news] 

\myparab{Hyper parameters for generating $g$}

\emph{Hyper parameters in $g$-EST Algorithm}

Number of subsets: [10, 20, 30, 40, 50]

\emph{Hyper parameters in Linear Boosting}

Number of Base Learners: [50, 100, 200]

Learning rate: [0.05, 0.1, 0.2]



\emph{Shared parameters for deep learning related models}

Batch size: [128, 256, 512]

The number of  epoch: 15 and we save model weights every epoch and run testing every two epoch.

Test years: [2016, 2017, 2018]  

Learning rate: [0.01, 0.001]

Dropout rate: [0.1, 0.3, 0.5, 0.8]

Universe: [\emph{Universe 800}, \emph{Full universe}]

$\beta$ Initialization:  [0.2, 0.5, 0.8]

Regularizer: [0,1,2], 

Regulation type: [0, 1, 2] where 0 means no regularization, 1 means Lasso, and 2 is Ridge regression.

Regulation rate: [0.001, 0.01, 0.1, 0.5, 1]

\emph{Hyper parameters in MLP}

Number of Dense Layers: [2, 3]

\emph{Hyper parameters in LSTM}

Number of dates: [2, 3, 5, 10, 21]

Recurrent Dropout:[0.2, 0.3, 0.5]

Equity forecasting models still heavily rely on hand-crafted features (the so-called ``factors'' in the empirical asset pricing literature~\cite{feng2019taming}. Superior performance of many sophisticated models may simply be explained by the higher quality factors these models used. Thus, we need to carefully perform an ``attribution analysis'' to accurately estimate the ``added value'' of a new statistical model. \MC{do we mean added value of a feature or set of features to a model? Or added value of a model itself? I though we meant performance attribution to individual features/signals.} 

\qq{add the definitions of corr and tstat}

\myparab{Significance test.} Recall that $\my_t \in \reals^d$ is a vector of response and $\hat \my_t \in \reals^d$ is the forecast of a model to be evaluated. We first need to examine whether the signals are correlated with the responses, i.e., for each $t$ we run the regression model $\my_t = \beta_t \hat \my_t + \epsilon$ and test whether we can reject the null hypothesis that the series $\beta_t = 0$ for all $t$. Note that the noises in the regression model is serially correlated so we use Newey-West~\cite{newey1986simple} estimator to adjust serial correlation issues. 
Consider, for example, a coin-tossing game, in which we make one dollar if our prediction of a coin toss is correct and loss one dollar otherwise. When our forecast has 51\% accuracy, we are guaranteed to generate positive return in long run (by standard concentration results). But testing whether our forecast has better than 51\% needs to be tested against many trials because, for example, when there are only 100 tosses, with $\approx 40\%$ probability a random forecast has a $\geq 51\%$ accuracy rate.  


\myparab{Infrastructure contribution.} Our major contribution is a new forecasting model that delivers superior prediction power by identifying latent links between stocks. Verifying our claim requires extensive and robust evaluation, which is remarkably difficult to be done by using only open resources. For example, most recent results~\cite{zhang2017stock,wang2019alphastock,hu2018listening} do not report how data are pre-processed, the logic of back-testing, and they report different sets of statistics. It becomes impossible to make any comparisons between models. This brings frustration to both practitioners, researchers, and reviewers. We provide the first open source evaluation framework for equity models with a goal to ensure models developed on our framework are reproducible, comparable to each other, and extensively evaluated. Our framework includes a major portion of (best effort) replicates of models appeared in recent premier machine learning/data mining conferences. 
%\MC{We can come back to this at the very end}.

%\MC{Can add a link to code, if avbl at the end. Data is hard to make available, but what about some of the actual  embeddings data? People in NLP release embeddings of the words, for example, but it's one embedding only, here we have it by time, but perhaps we make available montly embeddings, for example?}



%\MC{Just FYI:  Good point about data leakage, see for example the discussion here
%\url{https://papers.ssrn.com/sol3/papers.cfm?abstract_id=3486363}}

%\MC{ \textit{ See their Section  2.4 Data partition methods. 
%An ANN needs to be trained on a training set (in-sample) and then tested on a test set (out-of-sample). There exist several ways to partition a data set into such a training and test set. The first way is chronologically. That is, the early data constitutes the training set, and the late data constitutes the test set. Table 1 indicates that most of the papers follow this approach. However, some studies violate this time structure in the data by choosing a different way to partition the data. Violations can be introduced by randomly partitioning the data into a training and a test set or by using a so-called ‘odd-even split.’Random partitioning breaks the time structure and introduces information leakage between the training set and the test set. When an ANN is trained on a training set constructed in such a way, the error on the test set underestimates the generalisation error of the ANN. Yao et al. [2000] and our companion paper Ruf and Wang [2019] provide more discussion on this point.}  }

%\MC{ and they show in this paper \url{https://arxiv.org/pdf/2004.08891v1.pdf} that "random per- mutations of the in-sample and out-of-sample sets lead to a remarkable overestimation of the relative performance". Would be good to reference this example, and stress how important it is to obery the temporal ordering while splitting into test and train..
%}
\fi

==> simulator.tex <==

\section{Simulator}
Beyond simple statistical information, we built a simulator to better evaluate our model's performance in real market.\\
Why we need a simulator:

\myparab{1. Slippage.} In a real trading market, we may encounter slippage. For example, we change the stocks position at the open time of market in our model. If the price of the stock we want to buy goes up at this moment, then we can not make the transaction happen at the price we assumed, which makes the performance that we saw in long-short not reliable.

\myparab{2. liquidity risk.} We also need to consider the liquidity when we are going to buy stocks. We can not achieve the target position if there is no enough liquidity in the stock market. For example, we want to increase our position on one stock by 10,000 shares while there are only 1,000 shares traded in the market. Then we can not achieve our target.

\myparab{3. Transaction fee.} We also need to consider the transaction fee generated by changing the positions of stocks. 

